Coo: Consistency Check for Transactional Databases

In modern databases, transaction processing technology provides ACID (Atomicity, Consistency, Isolation, Durability) features. Consistency refers to the correctness of databases and is a crucial property for many applications, such as financial and banking services. However, there exist typical challenges for consistency. Theoretically, the current two definitions of consistency express quite different meanings, which are causal and sometimes controversial. Practically, it is notorious to check the consistency of databases, especially in terms of the verification cost. This paper proposes Coo, a framework to check the consistency of databases. Specifically, Coo has the following advancements. First, Coo proposes partial order pair (POP) graph, which has a better expressiveness on transaction conflicts in a schedule by considering stateful information like Commit and Abort. By POP graph with no cycle, Coo defines consistency completely. Secondly, Coo can construct inconsistent test cases based on POP cycles. These test cases can be used to check the consistency of databases in accurate (all types of anomalies), user-friendly (SQL-based test), and cost-effective (one-time checking in a few minutes) ways. We evaluate Coo with eleven databases, both centralized and distributed, under all supported isolation levels. The evaluation shows that databases did not completely follow the ANSI SQL standard (e.g., Oracle claimed to be serializable but appeared in some inconsistent cases), and have different implementation methods and behaviors for concurrent controls (e.g., PostgreSQL, MySQL, and SQL Server performed quite differently at Repeatable Read level). Coo aids to comprehend the gap between coarse levels, finding more detailed and complete inconsistent behaviors.

==> sections/new_model.tex <==
\section{Consistency model}\label{sec:anoamly_model}
This section introduces a new consistency model that can correlate all data anomalies. Specifically, we proposed \textit{Partial Order Pair (POP) Graph}, which considers not only object-oriented but also state-expressed operations, in contrast to traditional conflict graph which models only object-oriented operations.
% Traditional conflict dependencies $\{W_iW_j, W_iR_j, R_iW_j\}$ are operations of two transactions on the same object, without any the state information, i.e., commit and rollback. However, the state-expressed operations may also affect the object states. We consider these stateful information in our model. Specifically, we refine the edges of the traditional conflict graph into conflict dependencies with transaction states, called \textit{Partial Order Pair (POP)}. We call the redefined graph as \textit{Partial Order Pair Graph (POP graph)}. We later will prove that data anomalies can be completely represented by POP cycles, as both object-oriented and state-expressed operations are considered.

\subsection{Definition of Partial Order Pair Graph}\label{sec:Definition_pop_graph}

% This part extends the conflict graph so that we can redefine all data anomalies, thus correlating all anomalies to inconsistency. 
% Previous data anomalies defined by cases have struggled to characterize the nature of the problem, resulting in the ongoing reporting of new anomalies. 
% To solve this problem, we first formally define the POP in the following.
Adya's model introduced some non-cycle anomalies \cite{adya1999weak,DBLP:journals/pvldb/AlvaroK20} like Dirty Reads and Dirty write. The reason is that they did not consider state-expressed operations in their model, yet these operation sometimes maybe equivalent to a object-oriented operation. We strive to model all anomalies by a cycle by considering these state-expressed operations. We first formally define POPs as extended conflicts in the following.

\begin{definition}\textsc{\textbf{Partial Order Pair (POP).}}\label{def:pop}
Let $T_i$, $T_j$ be transactions in a Schedule $S$ and $T_i \neq T_j$.  A Partial Order Pair (POP) is the combination of object-oriented and state-expressed operations from $T_i$ and $T_j$ and satisfies:
\begin{itemize}
    \item both transactions operate on the same object;
    \item at least one operation affects the object version (a write or a rollback of a write).
\end{itemize}
\end{definition}

% POPs differ from standard conflict dependencies in that they take the stateful information (i.e., commit and abort) into account. In this way, the 3 conflicts can be expanded to 9 types of POPs.
\begin{lemma}\label{lemma:pop_types}
There exist at most 9 POPs in an arbitrary schedule, i.e.,$POP =  \{WW, WR, RW, WCW, WCR, RCW, RA, WC, WA\}$. 
\end{lemma}
\begin{proof}
The proof can be trivially achieved by enumerating all possible combinations of object-oriented and state-expressed operations.
Let $T_i, T_j$ be transactions in a Schedule $S$ and $p_i \in T_i$ with $q_j \in T_j $ being object-oriented operations that access the same object, $(p_i, q_j)\in \{W_iW_j, W_iR_j,R_iW_j\}$. The following is a list of all possible combinations.
\begin{itemize}
    \item[1.] $p_i-q_j$: Both transactions $T_i$ and $T_j$ are still active.
\end{itemize}
The transaction $T_i$ ends before $T_j$:
\begin{itemize}
    \item[2.] $p_i-C_i-q_j$: $T_i$ commits before $q_j$;
    \item[3.] $p_i-A_i-q_j$: $T_i$ aborts before $q_j$;
    \item[4.] $p_i-q_j-C_i$: $T_i$ commits after $q_j$ but ended before $T_j$;
    \item[5.] $p_i-q_j-A_i$: $T_i$ aborts after $q_j$ but ended before $T_j$;
\end{itemize}
The transaction $T_i$ ends after $T_j$:
\begin{itemize}
\item[6.] $p_i-q_j-C_j$: $T_j$ commits before $T_i$;
\item[7.] $p_i-q_j-A_j$: $T_j$ aborts before $T_i$.
\end{itemize} 
The operation $p_i$ will not influence the operation $q_j$ in combination $3$ due to the timely rollback of $T_i$. So does combination $7$. We acquire $15$ cases by substituting $\{W_iW_j, R_iW_j, W_iR_j\}$ into $(p_iq_j)$ of the remaining $5$ combinations.

Among them, $W_i W_j C_j$  and $W_i W_j$ both have the identical effect of modifying the accessing object by $W_j$, we group them together as POP $WW$. 
Similarly, we use POP $WR$ to represent $W_i R_j$ and $W_i R_j C_i$ and POP $RW$ to represent $R_i W_j$ and $R_i W_j C_j$.
Because read operations are unaffected by commit or abort, we put $R_i W_j A_i$ and $R_i W_j C_i$ into $RW$. Similarly, we put $W_i R_j C_j$ into $WR$.
% As a result, the above $9$ combination cases are divided into $3$ types of POPs.
% \begin{itemize}
%     \item $WW = W_i W_j[x] \leftarrow \{ W_i W_j, W_i W_j C_j\}$:  $T_j$ overwrites $T_i$'s write; %The version written by $T_i$ is overwritten by $T_j$ with a newer version, so that there may be inconsistent data status;
%     \item $WR = W_iR_j[x] \leftarrow \{ W_i R_j, W_i R_j C_j, W_i R_j C_i \}$: $T_j$ reads $T_i$'s write; %The version written by $T_i$ read by $T_j$;
%     \item $RW = R_i W_j[x]\leftarrow  \{ R_i W_j, R_i W_j C_j, R_i W_j C_i, R_i W_j A_i\}$: $T_i$ reads an old version, then $T_j$ writes a new version;%The version read by $T_i$, which is modified by $T_j$ to generate a new version, which may affect $T_i$ to read or modify the same variables;
% \end{itemize}
Three cases with committed of $T_i$, $W_i C_i R_j[x]$, $W_i C_i W_j[x]$, and $R_i C_i W_j[x]$, are specified as types $WCR$, $WCW$, and $RCW$, respectively.

Finally, we have three special combination cases, i.e., ${W_i R_j A_i}$, ${W_i W_j C_i}$, and ${W_i W_j A_i}$, that are more complex as they have two changing states. As for $W_i R_j A_i$, we have first changing state by $W_i R_j$ then second changing state by ${R_j A_i}$. $W_i R_j$ belongs to POP $WR$ and ${R_j A_i[x]}$ belongs to new POP $RA$. Likewise, ${W_i W_j C_i}$ has ${WW}$ and ${WC}$ POPs, and ${W_i W_j A_i}$ has ${WW}$ and ${WA}$ POPs.

In summary, these $15$ combination cases are grouped into 9 types POPs, i.e., $WW, WR, RW, WCW, WCR, RCW, RA, WC, WA$.
\end{proof}

For simplicity, this paper uses  group types for POPs, e.g.,  $WW$, $WR$, and $RW$ denote $W_iW_j[x]$, $W_iR_j[x]$, and $R_iW_j[x]$ POPs, respectively, unless otherwise specified for example when different objects need to be specified. Note that RA, WA, and WC are from the combination of a cycle, meaning RA, WA, and WC existed only when cycle already existed, and this cycle is a 2-transaction cycle on the single object. %For example, WA and WC are from the Dirty Write anomaly. 
Let $\mathcal{F}: POP(S) \rightarrow T(S) \times T(S)$ be the map between POPs and the transaction orders, e.g., $\mathcal{F}(W_i C_i R_j [x]) = (T_i, T_j)$.
In terms of POPs and their orders, we can define POP graphs.

\begin{definition}\textsc{\textbf{Partial Order Pair Graph (POP graph).}}\label{exmaple:cg_vs_popg}
  Let $S$ be a schedule. % and $s.transactions$ be a set of transactions belong to Schedule $S$. 
%   A graph $G(s)=(V,E)$ is called Partial Order Pair Graph, if vertices are transactions set  and edges are operations with partial order pairs, i.e.,
  A graph $G(S)=(V,E)$ is called Partial Order Pair Graph (POP graph), if vertices are transactions in $S$ and edges are orders in POPs derived from $S$, i.e (i) $V = T(S)$; (ii) $E = \mathcal{F}(POP(S))$.
\end{definition} 

Conflict and POP graphs are differences in the proposed purposes, edges, and expressiveness. Example 3 exemplifies a distinction between them.
% In general, POP graphs can express more on schedules.
% Table \ref{table:conflict_graph_comparison} illustrates differences between conflict and POP graphs. They are differences in the proposed purposes, edges, and expressiveness. In general, POP graphs can express more on schedules.
% \begin{table}[t]
% \caption{The comparison between conflict and POP cycles.}
% \small
% % \resizebox{1\linewidth}{!}{
% \input{tables/conflict_graph_comparison}
% % }
% \label{table:conflict_graph_comparison}
% \end{table}

\begin{example}\label{exp:pop}
Continuing Example \ref{exp:schedule}, we obtain objects $Obj$=$\{x,$ $y\}$, and operations
$Op[x]$=$\{R_1[x_0]R_3[x_0]W_2[x_1]C_2\}$ and
$Op[y]$= $\{W_1[y_1]R_3[y_1]R_1[y_1]A_1\}$ from $S_1$. Note that we don't put $A_1$ in $Op[x]$ as they don't have a write on object $x$ by $T_1$.
We derive POP from these operations, i.e. $\{R_1W_2[x],R_3W_2[x],$ $W_1R_3[y],$ $R_3A_1[y]\}$.

The Conflict graph and the POP graph for $S_1$ are shown in Figure \ref{fig:compare_ser_popg}. This time, by a POP graph, the Dirty Read is expressed by a cycle formed by $T_1$ and $T_3$. 
\begin{figure}[t]
    \centering
    \includegraphics[width= \linewidth]{figures/CG&POP.eps}
    \caption{Comparison of conflict and POP graph.}
    \label{fig:compare_ser_popg}
\end{figure}
\end{example}

\begin{lemma}
Arbitrary schedules can be represented by POP graphs. 
\end{lemma}
\begin{proof}
Given an arbitrary schedule $S$ with $Op(S)$ being the set of operations by transactions $\mathcal{T} = \{T_1, T_2, \dots, T_n\}$. First, we can derive sets of operations for variables from $S$, $\{OP[x]| x \in Obj(S)\}$. Then we can find all the combination cases in each object operation set $Op[x]$. Finally, we classify them into POPs referred to the proof of Lemma \ref{lemma:pop_types}. Through the above method, we can get the POP set $POP(S)$ corresponding to the schedule $S$. 

Then, by $\mathcal{F}$, we get the ordering between transactions based on POPs. We can model POP graphs using the transactions set and the dependent orders between transactions.
%Then we get the ordering between transactions based on POPs by $\mathcal{F}$. By the transactions set and the dependency orders between transactions, we can model the POP graphs. %Relation over transaction set $\mathcal{T}$ can be visualized through a POP graph in which the transaction of $\mathcal{T}$ form the nodes. The image set $\mathcal{F}(POP(S))$ describing the whole transactions orders in schedule $S$ takes as a directed edge. In particular, if $\mathcal{F}(POP(S))=\phi$, the POP graph only has 0-degree verities.
\end{proof}

% Due to the considering state-express operations on POPs, anomalies such as Dirty Read and Dirty Write are easy to represent by POP cycles.
% As seen in Figure \ref{fig:my_label}, $T 2$ reads the object $y$, causing a Dirty Read due to the abort operation of $T_1$, but no cycle in the conflict graph of schedule $S_1$(Left). In contrast, we can recognize $RA$ as a POP edge, forming a cycle for the Dirty Read anomaly(Right).

% The difference between POPs and traditional conflict dependencies is that the POPs considers the transaction state. For example. $R_i[x]A_j$ and $W_i[x]C_j$ are POPs as long as $A_j$ rollbacks a write and $C_j$ confirms a write, respectively. These new POPs can recognize more conflict dependency between transactions, making it more complete to express anomalies. 
% 
%Previous data anomaly definitions by cases are difficult to reflect the nature and new anomalies are frequently reported. Lacking state-express operations makes even Dirty Read or Dirty Write hard to be represented by the conflict graph. 
%For example, 
% In Example \ref{exp:schedule}, $T_2$ reads the object $y$ causing a Dirty Read due to the abort operation of $T_1$, but no cycle in the conflict graph of schedule $S_1$, as shown in Figure \ref{fig:compare_ser_popg}(a). 
% meaning serializable and consistent of the schedule, which conflicting our knowledge of the known Dirty Read anomaly. 
% In contrast, by our POP graph, we can recognize $RA$ as a conflict dependency, thus form a cycle for Dirty Read anomaly.


% For example, the previous dependency of $W_iR_j[x]$ can be split into $W_iC_iR_j[x]$ or $W_iR_j$ after adding states of two transactions. It makes the partial order  $W_iR_j[x]$ mean that no transaction commit or rollback operation between the two transactions. 
% We next discover all possible POPS in the following.


% \begin{proof}
% % The proof can be trivial achieved by enumerating all possible combination of object-oriented and state-expressed operations.
% % Let $T_i, T_j$ be transactions in a Schedule $S$ and $T_i \neq T_j$. Two object-oriented operations $p_i \in T_i$ and $q_j \in T_j $ access the same object and at least one of them is a write. If there is a state-expressed operation by one of the two transactions in a conflicting dependency, we only mark the first completed transaction, as the second one completed later. We show all the possible combinations as follows: %The state-expressed operation by another transaction is one of the three statuses of commit, abort, and still active.  Extensions of conflict dependencies are:
% % \begin{itemize}
% %     \item[1.] $p_i-q_j$: Both transactions $T_i$ and $T_j$ are still active.
% % \end{itemize}
% % The transaction $T_i$ ends before $T_j$:
% % \begin{itemize}
% %     \item[2.] $p_i-C_i-q_j$: $T_i$ commits before $q_j$;
% %     \item[3.] $p_i-A_i-q_j$: $T_i$ aborts before $q_j$;
% %     \item[4.] $p_i-q_j-C_i$: $T_i$ commits after $q_j$ but ended before $T_j$;
% %     \item[5.] $p_i-q_j-A_i$: $T_i$ aborts after $q_j$ but ended before $T_j$;
% % \end{itemize}
% % The transaction $T_i$ ends after $T_j$:
% %   \begin{itemize}
% %     \item[6.] $p_i-q_j-C_j$: $T_j$ commits before $T_i$;
% %     \item[7.] $p_i-q_j-A_j$: $T_j$ aborts before $T_i$.
% %   \end{itemize} 

% % In the combination $3$, due to the timely rollback of $T_i$, the operation $p_i$ will not affect the operation $q_j$. We remove this combination in our POP. So does the combination $7$. For the remaining cases, we substitute three conflict dependencies $p q\in \{W W,W R,R W\}$ into two operations, obtaining 15 instance cases.

% % Among them, $W_i W_j C_j$  and $W_i W_j$ has the same affect of changing the state of first transaction. We group them into one POP group called $WW$. Likewise, we let POP $WR$ represent the cases of $W_i R_j$, $W_i R_j C_j$ and let POP $RW$ represent $R_i W_j$, $R_i W_j C_j$.
% % The state-expressed operation of $R_i W_j C_i$ and $R_i W_j A_i$ in the $T_i$ did not affect the state of the $T_j$, making it equivalent to  $R_i W_j$. So we group them into POP $RW$.
% % Therefore, the above 9 combination instance cases are grouped into 3 types of POPs as follows:
% %   \begin{itemize}
% %     \item $WW = W_i W_j[x] \leftarrow \{ W_i W_j, W_i W_j C_j\}$:  $T_j$ overwrites $T_i$'s write; %The version written by $T_i$ is overwritten by $T_j$ with a newer version, so that there may be inconsistent data status;
% %     \item $WR = W_iR_j[x] \leftarrow \{ W_i R_j, W_i R_j C_j, W_i R_j C_i \}$: $T_j$ reads $T_i$'s write; %The version written by $T_i$ read by $T_j$;
% %     \item $RW = R_i W_j[x]\leftarrow  \{ R_i W_j, R_i W_j C_j, R_i W_j C_i, R_i W_j A_i\}$: $T_i$ reads an old version, then $T_j$ writes a new version;%The version read by $T_i$, which is modified by $T_j$ to generate a new version, which may affect $T_i$ to read or modify the same variables;
% %   \end{itemize}

% % Then there three cases with committed states for the first transaction, which are $W_i C_i R_j[x]$, $W_i C_i W_j[x]$, and $R_i C_i W_j[x] $ defined as types $WCR$,  $WCW$, and $RCW$, respectively. 

% % Next, we have three special combination cases, i.e., ${W_i R_j A_i}$, ${W_i W_j C_i}$, and ${W_i W_j A_i}$, that are more complex as they have two changing states. As for $W_i R_j A_i$, we have first changing state by $W_i R_j$ then second changing state by ${R_j A_i}$. $W_i R_j$ belongs to POP $W R$ and ${R_j A_i[x]}$ belongs to new POP $RA$. Likewise, ${W_i W_j C_i}$ has ${WW}$ and ${WC}$ POPs, and ${W_i W_j A_i}$ has ${WW}$ and ${WA}$ POPs.



% %   On the other hand, Split ${W_i R_j A_i} = {W_i R_j [x]} \vee {R_j A_i[x]} $ (Figure \ref{RA}),  ${W_i W_j C_i} = {W_i W_j [x]} \vee {W_j C_i[x]}$ (Figure \ref{WC}) and ${W_i W_j A_i} = {W_i W_j [x]} \vee {W_j A_i[x]}$(figure \ref{WA}). So cases $\{W_i R_j A_i, W_i W_j C_i, W_i W_j A_i \}$ can be abbreviated as $\{RA,  WC, WA\}$ respectively.
% %   \begin{figure}[ht!]
% %     \begin{subfigure}[t]{0.167\textwidth}
% %         \centering
% %         \includegraphics[width= 0.8\linewidth]{figures/RA.PNG}
% %         \caption{}
% %         % \caption{The partial order $R_j A_i$ constitutes a cycle.}
% %         \label{RA}
% %     \end{subfigure}%
% %     \begin{subfigure}[t]{0.167\textwidth}
% %         \centering
% %         \includegraphics[width= 0.8\linewidth]{figures/WC.PNG}
% %         \caption{}
% %         % \caption{The partial order $W_j C_i$ constitutes a cycle.}
% %         \label{WC}
% %     \end{subfigure}%
% %     \begin{subfigure}[t]{0.167\textwidth}
% %         \centering
% %         \includegraphics[width= 0.8\linewidth]{figures/WA.PNG}
% %         \caption{}
% %         % \caption{The partial order $W_j A_i$ constitutes a cycle.}
% %         \label{WA}
% %     \end{subfigure}%
% % \caption{The partial order (a) $R_j A_i$, (b) $W_j C_i$ or (c) $W_j A_i$ constitutes a cycle.}
% % \end{figure} 
% \end{proof}

% According to the definition of POPs, each element in POPs set maps to an order of two transactions. Let $\mathcal{F}: POPs\rightarrow T\times T$ be a function from the POPs set to the transaction orders, e.g., $\exists W_iA_j\in POPs$, $\mathcal{F}(W_iA_j) = (T_i, T_j)$. The image set $\mathcal{F}(POPs)$ means the whole transactions orders set are in POPs set. Let $\mathcal{F}^{-1}$ $(T_i, T_j)$ $= \{POP[x]$ $\in POPs: \mathcal{F}(POP[x]) = (T_i, T_j)\}$ be the inverse image.

% \begin{figure}[t]
% \centering
%     \subfigure[Conflict graph]{
%     \includegraphics[width= 0.45\linewidth]{figures/CG_2.png}}
%     % \hspace{.05in}
%     \subfigure[POP graph]{
%     \includegraphics[width= 0.45\linewidth]{figures/POPG_2.png}    
%     }
%     \caption{Comparison of the conflict graph and the POP graph  of the same schedule. Left: Traditional conflict graph, Right: Partial order pair graph.}
%     \label{fig:compare_ser_popg}
% \end{figure}
% \begin{example}
% Continuing Example \ref{exp:schedule}, Figure \ref{fig:compare_ser_popg} shows the graphic representations of Conflict graph and POP graph for $S_1$. 
% % The conflict graph and the POP graph of Schedule $S$ from example \ref{exp:pop} are shown in figure \ref{fig:compare_ser_POP graph}.
% The rollback of the $T_1$ makes the read of the $T_3$ to be incorrect, causing the Dirty Read anomaly between $T_1$ and $T_3$. However, traditional conflict graph without consider state-expressed operations cannot reflect this anomaly/cycle on the graphs. In contrast in POP graph, the Dirty Read is expressed by a cycle formed by $T_1$ and $T_3$. 
% \end{example}


\subsection{Definition of Consistency}\label{sec:definition_consistency}

With POP cycles, we now are ready to define data anomalies, then define consistency with no data anomaly. 
\begin{definition}\textsc{\textbf{Data Anomaly}.}\label{def:anomaly}
Data anomaly exists if the represented POP graph has a cycle.
\end{definition} 
Detecting conflict cycles on conflict graphs \cite{DBLP:conf/eurosys/YabandehF12} is a popular strategy for avoiding data anomalies.
The definition of data anomalies by POP graphs differs from the conflict graph one in three aspect. Firstly, POP model schedule instead of history. We later show some unfinished transactions can already form cycles. Secondly, cycles in the conflict graph cannot express all data anomalies. For example, Dirty Read in Example \ref{exmaple:cg_vs_popg} is an anomaly between $T_1$ and $T_3$, yet can not represented by conflict graph as it can not model state-expressed operations like abort. 
Thirdly, conflict graph can not distinguish some distinct anomalies with different schedules. For example, Read Skew (RW-WR) and Read Skew Committed (RW-WCR) are different anomalies by our model and behave differently in some databases. As shown in Table \ref{table:evaluation_test_case_read_skew}, PostgreSQL passes the test of Read Skew anomaly but takes Read Skew Committed as an anomaly in Read Committed isolation level. %However, conflict graph model these two anomalies as the same one. %However, Aday take the two anomalies as the same conflict cycle.


 
% The data anomaly we define by POP cycles could express all possible anomalies in any schedule as we consider not only object-oriented operations but also state-expressed operations. We also enumerate all possible combinations that could change data stats. 
The definition of data anomalies to cycles is read-time and stricter than the result consistency \cite{2002Concurrency}, where some may consider no anomaly if the result is consistent or serializable. For example, we consider Full-write ($W_i[x_0] W_j[x_1] W_i[x_2]$) in Table \ref{table:anomaly_classification} as a anomaly as its presented POP graph is a cycle. However, some systems executing it as scheduled may not raise any issue, as the final result is consistent to a serializable execution of $T_j$ and $T_i$ with the final result $x_2$. Yet, in our evaluation, we found all databases do not allow any write on a dirty write, resulting in abort or wait in $T_j$.

% \begin{corollary} \label{corollary:2-POPs}
%  A data anomaly has at least two transactions and two POPs. 
% \end{corollary}
% Since we define an anomaly as a POP cycles, such cycle must have at least two vertices and two edges.

\begin{definition}\textsc{\textbf{Inconsistency}}\label{def:InConsistency}
Schedule $S$ satisfies \textbf{Inconsistency} when the POP graph of $S$ has at least one data anomaly.
\end{definition}

\begin{definition}\textsc{\textbf{Consistency}}\label{def:Consistency}
%Schedule $S$ satisfies consistency when the POP graph of $S$ is acyclic.
Schedule $S$ satisfies consistency when there is no \textbf{Inconsistency} in the POP graph of $S$.
\end{definition}
We have defined data anomalies by POP cycles. We now define the consistency of no data anomaly, i.e., the represented graphs are acyclic. %This definition is stricter than result consistency which only check if the result is consistent with one of the serializable schedule. 
By this definition, consistency, no data anomalies, and acyclic POP graphs are equivalent. Likewise, inconsistency, existing data anomalies, and POP cycles are equivalent.
% \textcolor{red}{this is a definition, so no need to prove but need to clarify the assumption/prerequisite/condition}
% We specify the earliest cycle that appeared in the conflict graph to be studied.  And we use types of POPs to classify them. 

% The only operations that affect data states in a schedule are writes.  A consistent state requires at least  two transactions keep the consistency. Therefore, the total combination of operations between two transactions that can affect the data state is in POP set. If a schedule does not contain anomalies, we consider that the schedule maintains the consistency of the data.

% In other words, if there is no cycle in its POP graph,  the scheduling does not contain any anomaly. We think the schedule maintains the consistency of databases, w.r.t,

%   Consistency $\Leftrightarrow$ Directed acyclic graph $\Leftrightarrow$ No data anomalies  .
  
%   No Consistency $\Leftrightarrow$ Directed cycle $\Leftrightarrow$ Data anomalies  .

\input{sections/new_model_Pro2}

% \subsection{Classification of Data Anomalies}\label{sec:AnomalyClassification}
\subsection{Consistency Check Principle}\label{sec:AnomalyClassification}
This part introduce our consistency check method in theory and in practice. In theory, we show the soundness and completeness of the method. In practice, we classify data anomalies and show cases forms of data anomalies.
% The traditional definition of anomalies is based on Conflict graph \cite{adya2000generalized} that only has three kinds of conflict dependencies as edges. But it can not take Dirty Write, Dirty Read, and Intermediate Reads as cycle structures expressing in the POP graph. Now, we define a POP graph by nine kinds of POPs. The POP graph not only takes Dirty Read, Dirty Write, and Intermediate Reads as cycles but also considers all operation combinations with all possible objects.  Therefore, data anomalies based on POP cycles we define take in all cases of data anomaly. It tries to completely establish a one-to-one mapping of all data anomalies and graphs.

% TODO % yuxing
% Consider for an example a sorting algorithm A that receives as input a list of numbers. We say that A is sound if every time it returns a result that result is a sorted list. Likewise, we say that A is complete if guarantees to return a sorted list any time we give it a list of numbers.

% Elle’s inferences are sound: that is, any anomalies identified in an observation must be present in any corresponding Adya history.
% Consistency checker is sound: any anomaly identified in a schedule must be present in any corresponding history.

% if it reports an anomaly in an observation, that anomaly should exist in every interpretation of that observation.
We first discuss the soundness and completeness of our model. The consistency check is \textbf{sound}, if it reports an anomaly in a schedule, that anomaly should exist in every history of that schedule. 
The consistency check is \textbf{complete}, it reports an anomaly in a schedule, then it must find a POP cycle in the schedule. As a schedule is a prefix of history, the anomaly occurring in the schedule occurs in the corresponding history. So the soundness is correct. As we define the anomaly schedule exists a POP cycle, the completeness is also correct.

We then divide anomalies based on the primitive conflict dependencies, i.e., WR, WW, and RW, separating anomalies into three types, as follows:
\begin{itemize}
    \item \textbf{Read Anomaly Type (RAT)}, if the cycle has at least a $WR$ POP; % , i.e., for a cycle $G=\{V, E\}$ with $ \exists WR\in E$.
    \item \textbf{Write Anomaly Type (WAT)}, if the cycle does not have a $WR$ POP, but have at least a $WW$ POP; %, i.e.,for a cycle $G=\{V,E\}$ with $ (\forall WR \notin E)\wedge (\exists WW\in E) $.  
    \item \textbf{Intersect Anomaly Type (IAT)}, if the cycle does not have $WR$ and $WW$ POPs. %, i.e.,for a cycle $G=\{V,E\}$ with $ (\forall WW \notin E)\wedge (\forall WR \notin E) $.
\end{itemize}
We can also classify the anomalies/cycles based on number of transactions ($N_{T}$) and objects ($N_{obj}$), as follows:
\begin{itemize}
    \item \textbf{Single Data Anomaly (SDA)}, if $N_{T}=2$, $N_{obj}=1$;
    \item \textbf{Double Data Anomaly (DDA)}, if $N_{T}=2$, $N_{obj}=2$;
    \item \textbf{Multi-transaction Data Anomaly (MDA)}, otherwise.
\end{itemize}
By Lemma \ref{lemma:one_object_reduction}, SDAs contains all single-object anomalies. For expressiveness simplicity, DDAs only include 2 objects with 2 transaction. So, SDA and DDA are finite and one-to-one maping anomalies, while each anomaly in MDA stands for groups of anomalies, meaning MDAs are infinite with arbitrary $N_{T}$ and $N_{Obj}$. Since SDAs and DDAs are finite, complete, and enumerable, we will build all test cases based on them. While MDAs are infinite, we will build one typical and representative case for each group of them in our evaluation.

Table \ref{table:anomaly_classification} shows all data anomalies types and their classification. The anomaly names with BOLD font are 20+ new types of anomalies that have never been reported. Those reported in Step RAT and Step IAT are tiny portion of them. We do not limit other classifications with more transactions and objects for one-to-one mapping anomalies, yet we think this classification is sufficient to illustrate the core idea and evaluation, enabling us to check the consistency of RDBMs with a countable number of representative anomaly test cases.
% \textbf{Based on this, an infinite number of data anomalies can be transformed into a limited types of data anomalies.}
% This enables us to check the consistency of RDBMs with a limited number of test cases.

% \begin{theorem} \label{theorem2}
%   MDAs are infinite.
% \end{theorem}
% The cases in SDA and DDA are finite, one-to-one mapping, and complete by Theorems \ref{theorem:reduction} and \ref{theorem2}. 
% However, MDAs are a set of anomalies. And the number of variables can be infinite in a schedule, resulting infinite of POP cycles, thus infinite number of MDAs.

% We also classify the anomalies based on the different numbers of transactions and numbers of objects. We call it Single Data Anomaly (SDA) if anomalies cycles have an object ($N=1$) and two transactions ($n = 2$).  Lemma \ref{lemma:one_object_reduction} proves that a POP cycle accessing only one object can be reduced to a 2-transaction cycle. Therefore, SDAs contains all single-object anomalies. Theorem \ref{theorem:reduction} proves that a POP cycle with POPs accessing two objects ($N=2$) is at most constructed by 4-transaction. However, considering the complexity of the discussion and the occurrence probability in practice, we only classify the cycle with two transactions ($n = 2$) and two objects ($N=2$) as Double Data Anomaly (DDA). We classify the remaining cases as multi-transaction data anomaly (MDA) types. Therefore, the MDA class includes two objects with three- or four-transaction anomalies and multi-objects $N \geq 2$ with multi-transaction $n \geq 3$. 
% Table \ref{table:anomaly_classification} shows all data anomalies types and their classification. The anomaly names with BOLD font are 20+ new types of anomalies that have never been reported. Though some instances of Step RAT and Step IAT are reported, we claim that these anomalies could be produced differently with any numbers ($N \geq 2$) of objects.


So based on our classification, Read Skew ($R_1[x_0]W_2[x_1]W_2[y_1]$ $R_1[y_1]$) and Read Skew Committed ($R_1[x_0]W_2[x_1]W_2[y_1]C_2R_1[y_1]$) are in different categories. Read Skew with WR belongs to RAT, while Read Skew Committed without WR and WW belongs IAT.
% \begin{example}
% Given the schedule of anomaly Read Skew $S_3$ by two transactions and two objects:
% \begin{equation}
%     S_3 = R_1[x_0]~W_2[x_1]~W_2[y_1]~R_1[y_1])
% \end{equation}
% And the schedule of $S_4$ of anomaly Read Skew Committed in the following:
% \begin{equation}
%     S_4 = R_1[x_0]~W_2[x_1]~W_2[y_1]~C_2~R_1[y_1]
% \end{equation}
% Note these two anomalies are recognized by one conflict graph without consider state-expressed operations. Yet we consider these two anomalies as two individual even in two anomalies types. Read Skew is in RAT type as it has WR POP, while Read Skew Committed is in IAT type as it does not have WW and WR POPs.
% \end{example}


% \begin{proof}
% 
% In a schedule, the number of variables can be infinite. And MDA represents a POP cycle which could be also infinite.
%According to the Theorem \ref{them:reduction}, an infinite number of variables can be reduced to an edge with twice the number of variables, so the number of MDA is infinite.
% \end{proof}

\begin{corollary}
  If a schedule satisfies consistency, then the schedule does not have any data anomalies in Table \ref{table:anomaly_classification}. 
\end{corollary}

% \textcolor{red}{Read Skew and Read Skew Committed}
% \begin{example}
%   Suppose $x+y = 5$ is a database constraint between two objects $x$ and $y$. We show an example of a schedule $S_2$ with initial values $x = 3, y = 2$:
%   \begin{equation}
%       S_2 = R_1[x:=3] W_2[x:=2] W_2[y:=3] C_2 R_1[y:=3].
%   \end{equation}
%   Transaction $T_1$ reads $x$, and then the other transaction $T_2$ update $x$ and $y$ and commits. Transaction $T_2$ may see an inconsistent state if it reads $y$.
% \end{example}
% Our classification is efficient to illustrate POP cycles and data anomalies, yet we don't limit more detailed classification for MDAs.
% SDA contains all cycles with two transactions and one object. DDA contains all cycles with two transaction and two objects. MDA contains all cycles of other cases.
% We define anomalies by POP cycles to make it visualize and specific. Since we enumerate all combinations of operations that change the state of data, and we have proved schedules mapping to POP graphs in lemma 2, let anomalies we define include all anomalies in any schedule.

%\noindent \textbf{Distributed Data Anomalies.} \indent In databases,



% Two important points:
% Soundness is a weak guarantee. It does not promise that A will terminate.
% Soundness and Completeness are related concepts; infact they are the logical converse of each other. i.e. Soundness says that if an answer is returned that answer is true. Completeness says that an answer is true if it is returned.
% Consider for an example a sorting algorithm A that receives as input a list of numbers. We say that A is sound if every time it returns a result that result is a sorted list. Likewise, we say that A is complete if guarantees to return a sorted list any time we give it a list of numbers.



\subsection{Distributed Consistency} \label{sec:DistributedDataAnomalies}
%In databases, if distributed, the concurrent control may need extra validation (e.g., 2PC \cite{DBLP:conf/icdt/Raz95}) for transaction. 
We have shown that the consistency lacks standards and is non-trivial to verify, not to mention the distributed consistency.
Our model is also possible to validate distributed scenarios. We then define distributed data anomalies.
% Or, discuss it in Chapter 3

\begin{definition}\textsc{\textbf{Distributed Data Anomalies}}\label{definition:distributed_data_anomaly}
    A schedule exists a distributed data anomaly, if the represented POP graph is cyclic and it has at least two object storing at distributed partitions.
\end{definition} 
By our classification, a distributed data anomaly belongs to DDA or MDA, but not SDA.  Schedule $S$ satisfies \textbf{distributed consistency} if no distributed data anomaly exists in $S$. 
For evaluation, we deployed multiple ($\geq$2) servers or data partitions/nodes. We particularly designed the test cases to access the different objects from different partitions sometimes from different tables. The design is required by table partitioning and the data is expected to insert/update in different partitions/shards (e.g., PARTITION BY RANGE in SQL).

% \begin{definition}\textsc{\textbf{Distributed Inconsistency}}\label{def:DistributedInConsistency}
% Schedule $S$ satisfies distributed inconsistency when the POP graph of $S$ has at least one distributed data anomaly.
% \end{definition}

% \begin{definition}\textsc{\textbf{Distributed Consistency}}\label{def:DistributedConsistency}
% %Schedule $S$ satisfies consistency when the POP graph of $S$ is acyclic.
% Schedule $S$ satisfies distributed consistency when there is no distributed inconsistency in the POP graph of $S$.
% \end{definition}

%TODO % yuxing 弱化对死锁的定义和表达，将来另外成文

%definition of deadlock

% That is to say, a distributed data anomaly cannot be an SDA anomaly, but only a DDA or MDA anomaly.

% \subsection{Important Discussion}\label{sec:ImportantDiscussion}























%\input{sections/Theorem}

% \section{Predicate Anomalies}
% Consider predicate operations in a schedule, the read operation is divided into two categories. One type is a \textcolor{red}{physical} read $R_i[x_n]$, which describes the transaction $T_i$ read the object $x$ with version $n$. The other type is a predicate read operation $R_i^P[x_n]$, which describes that the object $x$ with version $n$ was in the set of objects fitting predicate logic $P$ by the transaction $T_i$, i.e, $R_i[x_n \in Vset(P)]$. 
% \textcolor{red}{put above}
% A \textbf{predicate} is a sentence that contains a finite number of variables and becomes a statement when specific objects are substituted for the variables. The \textbf{domain} of a predicate $Vset(P)$ is the set of all objects that may be substituting in place of the variables \cite{epp2010discrete}. \textcolor{red}{In logic, predicates can be obtained by removing some or all of the nouns $x$ or $x,y$ from a statement and be symbolized as $P(x)$ or $P(Objs)$. Always predicate is a  predicate symbol together with suitable predicate variables referred to as propositional functions or open sentences.} Predicate logic includes first-order logic, second-order logic and $n$-order logic. In first-order logic, a predicate can only refer to a single subject. First-order logic is also known as first-order predicate calculus or first-order functional calculus \cite{smullyan1995first}. A sentence in first-order logic is written in the form $P(x)$, where $P$ is the predicate and $x$ is the subject, represented as a variable.  \textcolor{red}{Second-order logic is a predicate logic of two predicate variables after simplie.} The same definition method is for $n$-order logic. We define that \textbf{atomic formula} for an $n$-tuple $P(x,y,\dots)$ where $P$ is any predicate of degree $n$ and $x,y,\dots$ are $n$ cannot be divided symbols (or variables).Smullyan and Raymond M \cite{janin1996expressive}proved that a $n$ order logic \textcolor{red}{can containing} only disjunction of sentence of the form: $P(x,y,\dots) = \wedge (or \vee) P_i(x_i) \wedge(or \vee) P_j(x_j,y_j) \dots \wedge (or \vee) P_z(x_z,y_z,\dots)$. Besides, a physical read operation can be regarded as the predicate read operation with the predicate variable happens to be the object ID. 
% In order to reflect the affection between write and read operations, we extend senses of versions of the object which adding insertion and deletion versions.
%   \begin{itemize}
%     \item The object $x$ has an initial version $x_{init}$ called unborn version. When transaction $T_i$ creates an object that will ever exist in the system through writing operation, we denote $W_i[x_0]$. Of course, there is no read operation $R_i[x_{init}]$. 
%     \item The object $x$ has a visible version $x_n(n=0,1,2,\dots)$ when a transaction updates an object to generate its new version. We use $R_i[x_n]$ to describe a transaction read a version of an object that is in the set.
%     \item The object $x$ has a dead version $x_{dead}$ when the transaction deletes an object $x$. We use $W_i[x_{dead}]$ to describe this situation. Also, there is no read operation $R_i[x_{dead}]$.
%   \end{itemize}

% \textcolor{red}{how do these different order logic related to the latter work?}




%   Based on the definition of versions of an object, there are four cases of reading and writing operations under the predicate logic.
%   \begin{itemize}
%     \item The version of the object $x_n$ is in the predicate domain set $Vset(P)$ by the predicated-based read operation, which denoted $R_i[x_n \in Vset(P)]$.
%     \item  The version of the object $x_n$ is not in the predicate domain set $Vset(P)$ by the predicate-based read operation, which denoted $R_i[x_n \notin Vset(P)]$.
%     \item The version of the object $x_n$ is in the predicate domain set $Vset(P)$ by the predicate-based write operation, which denoted $W_i[x_n \in Vset(P)]$.
%     \item The version of the object $x_n$ is not in the predicate domain set $Vset(P)$ by the predicate-based write operation, which denoted $W_i[x_n \notin Vset(P)]$.
%   \end{itemize}
%   We write $W_i[x_n]$ indicated writing a value $x_n$ that is irrelevant to whether or not in the predicate domain set $Vset(P)$.

%   According to the extended definition of object versions, \textcolor{red}{$W_i[x_0 \in Vset(P)]$} indicates that the transaction $T_i$ inserts the new object exactly in the predicate set. And  \textcolor{red}{$W_i[x_{dead} \in Vset(P)]$} indicates that the transaction $T_i$ deleted the object exactly in the predicate set.
  
%   We separate Read-Write dependency and Write-Read dependency to several cases by whether the object read in predicate-based domains. We divide (\textcolor{red}{how?}) the conflict dependencies into entity conflicts and predicate conflicts:
% \begin{itemize}
%     \item []$\begin{aligned}
%   \text{Entity Conflicts} = &\{ W_i[x_n] W_j[x_{n+1}], \\ 
%   & R_i[x_n \in Vset(P)]W_j[x_{n+1} \in Vset(P)],\\
%   & W_i[x_n \in Vset(P)]R_j[x_n \in Vset(P)]\} ;
% \end{aligned}
% $
% \item []$\begin{aligned}
%   \text{Predicate Conflicts} = &\{ R_i[x_n \in Vset(P)]W_j[x_{n+1} \notin Vset(P)], \\ 
%   &  R_i[x_n \notin Vset(P)]W_j[x_{n+1} \in Vset(P)],\\
%   & W_i[x_n \notin Vset(P)]R_j[x_n \notin Vset(P)]\} .
% \end{aligned}
% $
% \end{itemize}
% Based on the above discussion, We can still symbolize the conflict dependencies as \textcolor{red}{$conf = \{ W_iW_j,W_iR_j,R_iW_j\}$}. 

% \textcolor{red}{Adding transaction state to the expanded conflicting dependencies can get 9 types of partial order pairs in section \ref{sec:model}}. And the expanded conflict dependencies also one-to-one map a partial order pairs graph.

% \textcolor{red}{provide a detailed purpose before example, why these examples?}
% \begin{example}
%   If 
% $$
% \begin{aligned}
%   s = &W_1[x_0 \in Vset(P)]W_2[x_1 \notin Vset(P)]W_2[y_1 \in Vset(P)] \\
%   &W_3[y_2 \in Vset(P)]R_1[x_1 \notin Vset(P)]R_1[y_2 \in Vset(P)]C_1C_2
% \end{aligned}
% $$
% where $T_1$ and $T_2$ are committed, \textcolor{red}{and $T_3$ still active}.

% The transaction $T_1$ inserts an object $x$ in predicate domain set $Vset(P)$, but the transaction $T_2$ updates it and \textcolor{red}{move it out}. The transaction $T_3$ updates the object $y$ and the transaction $T_1$ read it.

% We have 
% $$ 
% \begin{aligned}
% \text{Entity conflicts} = &\{W_1 W_2[x],W_2W_3[y],\\
%                          &W_3[y_2 \in Vset(P)]R_1[y_2 \in Vset(P)]\}.
% \end{aligned}
% $$
% $$
% \text{Predicate conflict} = \{W_2[x_1 \notin Vset(P)]R_1[x_1 \notin Vset(P)]\}.
% $$

% \end{example}

% \begin{example}
%   A schedule has two predicate logics and $Vset(P_1)\bigcap Vset(P_2)=\phi$,  i.e.,
%   $$
%   \begin{aligned}
%     s = &W_1[x_0 \in Vset(P_1)]W_2[x_1 \notin Vset(P_2)]W_2[y_1 \in Vset(P_2)] \\
%     &W_3[y_2 \in Vset(P_1)]R_1[x_1 \notin Vset(P_2)]R_1[y_1 \in Vset(P_1)]C_1C_2.
%   \end{aligned}
%   $$
%   Firstly, we rewrite the schedule with visible read under non-predicate logic
%   $$
%   S_{1} = W_1[x_0]W_2[x_1]W_2[y_1]W_3[y_2]R_1[y_1].
%   $$
%   We have the entity conflicts set
%   $$
%   \text{Entity conflict} = \{W_1 W_2[x],W_2W_3[y],W_3R_1[y]\}.
%   $$

%   The only invisible read operation is $R_1[x_1 \notin Vset(P_2)]$. We choice operations with the predicate $P_2$
%   $$
%   \text{Predicate conflict} = \{W_2[x_1 \notin Vset(P_2)]R_1[x_1 \notin Vset(P_2)]\}.
%   $$
% \end{example}
% So the conflict graph is shown as fig.\ref{fig1}.
% \begin{figure}[h]
%   \centering
%   \includegraphics[width= 0.7\linewidth]{figures/fig1.PNG}
%   \caption{Conflict graphs of \textcolor{red}{example 2.}}
%   \label{fig1}
% \end{figure}

% It also keeps the corresponding relationship between data anomalies and partial order pairs graphs. When read and write operations in the table as predicate conflict dependencies, it can represent predicate anomalies. 

% \begin{example}
%   Phantom anomaly will be like predicate-based non-repeatable read in table \ref{table:conflict_graph_comparison}. It has two combination methods,
%   \begin{itemize}
%       \item $R_i[x \notin Vset(P)]\dots W_j[x \in Vset(P)]\dots R_i[x \in Vset(P)]$, i.e., 
%       $$R_i[x \in Vset(P)]W_j[x \in Vset(P)]-W_j[x \in Vset(P)] R_i[x \in Vset(P)]$$.
%       \item $R_i[x \in Vset(P)]\dots W_j[x \notin Vset(P)] \dots R_i[x \notin Vset(P)]$, i.e.,
%       $$R_i[x \in Vset(P)]W_j[x \notin Vset(P)]-W_j[x \in Vset(P)] R_i[x \notin Vset(P)]$$.
%   \end{itemize}
% \end{example}

% \begin{example}
%   Predicate-based write skew in table \ref{table:conflict_graph_comparison} has 9 methods of combination. 
%   $$R[x \in Vset(P)]W[x \in Vset(P)]-R[y \in Vset(P)]W[y \in Vset(P)].$$ It is an entity anomalies.
%   $$R[x \in Vset(P)]W[x \notin Vset(P)]-R[y \in Vset(P)]W[y \in Vset(P)]$$
%   $$R[x \notin Vset(P)]W[x \in Vset(P)]-R[y \in Vset(P)]W[y \in Vset(P)]$$
  
%   $$R[x \in Vset(P)]W[x \in Vset(P)]-R[y \notin Vset(P)]W[y \in Vset(P)]$$
%   $$R[x \in Vset(P)]W[x \notin Vset(P)]-R[y \notin Vset(P)]W[y \in Vset(P)]$$
%   $$R[x \notin Vset(P)]W[x \in Vset(P)]-R[y \notin Vset(P)]W[y \in Vset(P)]$$
  
%   $$R[x \in Vset(P)]W[x \in Vset(P)]-R[y \in Vset(P)]W[y \notin Vset(P)]$$
%   $$R[x \in Vset(P)]W[x \notin Vset(P)]-R[y \in Vset(P)]W[y \notin Vset(P)]$$
%   $$R[x \notin Vset(P)]W[x \in Vset(P)]-R[y \in Vset(P)]W[y \notin Vset(P)].$$
%   The rest of 8 combinations is predicate anomalies.
%   Entity-dependent and predicate-dependent may compose an anomalies cycle, which we regard as predicate anomalies. 
% \end{example}

% According to the previous discussion, Table \ref{table:conflict_graph_comparison} with predicate operations anomalies with a labeled star(*) can be expressed as including all data anomalies. 



==> sections/preliminary.tex <==
\section{Preliminary}\label{sec:preliminary}
This section provides the preliminary of knowledge that will be used and extended in the following section. We consider storing data objects $Obj=\{x,y,...\}$ in a concurrent system. The data object is an abstract concept, and the definition leaves some leeway in other systems. Transactions interact with the objects by issuing read and write operations. We divide operations in a database into two types: object-oriented operations and state-expressed operations. \textbf{Object-oriented operations} are operations on objects by reading or writing. Let $Op_i$ describe the possible invocations set: reading or writing an object by transaction $T_i$.  \textbf{State-expressed operations} are operations to express states of transactions, consisting of committed (C) and abort (A). \textbf{Transaction} is a sequence of object-oriented operations and a state-expressed operation at the end. If there is no state-expressed operation at the end, the transaction is still active. A state-expressed operation indicates the end of the transaction. We use subscripts to express transactions of operations. For example, $Op_i[x_n]$ is $x$-oriented operations by transaction $T_i$; $C_i$ and $A_j$ are the committed and abort operations and by transaction $T_i$ and transaction $T_j$, respectively.

% \begin{definition}\textsc{\textbf{Schedules}}\cite{DBLP:books/mk/WeikumV2002}. \label{def:Schedule}
% Let $\mathcal{T} = \{T_1, T_2, \dots, T_n \}$ be a (finite) set of transactions, where each $T_i \in \mathcal{T}$ has the form $T_i = (Op_i, <_i)$, with $Op_i$ denoting the set of operations of $T_i$ and $<_i$ denoting their ordering, $1\leq i \leq n$.
% A history for $\mathcal{T}$ is a pair $S = (Op(S), <_s)$ such that:
% \begin{itemize}
%     \item[a.] $Op(S)\subseteq \cap_{i=1}^n Op_i \cap_{i=1}^m \{A_i, C_i\}$ and $\cap_{i=1}^n Op_i \subseteq Op(S)$, i.e., $S$ consists of the union of the operations (object-oriented operations) from the given transactions plus a termination operation (state-expressed operations) for each $T_i \in \mathcal{T}$;
%     \item[b.] $\left(\forall i, 1\leq i \leq m\right) C_i\in Op(S) \Leftrightarrow A_i \notin Op(S)$, i.e., for each transaction, there is either a commit or an abort in $S$, but not both;
%     \item[c.] $\cap_{i=1}^n <_i \subseteq <_s$, i.e., all transaction orders are contained in the order given by $S$;
%     \item[d.] $\left(\forall i, 1\leq i \leq m\right)\left(\forall p\in Op_i\right) p<_s A_i$ or $p<_s C_i$, i.e., the Commit or Abort operation always appears as the last step of a transaction.
%     \item[e.] every pair of operations $p,q \in Op(S)$ from distinct transactions that accesses the same object and has at least one write operation among them is ordered in $S$ in such a way that either $p<_s q$ or $q<_s p$. 
% \end{itemize}
% A schedule is a prefix of a history.
% \end{definition}

\begin{definition}\textsc{\textbf{Schedules}} \cite{DBLP:books/mk/WeikumV2002}. \label{def:Schedule}
Let $\mathcal{T} = \{T_1, T_2, \dots, T_n \}$ be a (finite) set of transactions. A schedule $S$ is a list of operations (object-oriented or state-expressed) from the set of transactions $\mathcal{T}$ in database. Let $Op(S)$ be the operations set of the schedule $S$, and $<_s$ denote orderings such that:
\begin{itemize}
    \item[a.] $Op(S)\subseteq \cap_{i=1}^n Op_i \cap_{i=1}^m \{A_i, C_i\}$ and $\cap_{i=1}^n Op_i \subseteq Op(S), m \leq n$, i.e., $S$ consists of the union of the operations (object-oriented operations) from the given transactions plus a termination operation (state-expressed operations) for each $T_i \in \mathcal{T}$;
    \item[b.] $\left(\forall i, 1\leq i \leq m\right) C_i\in Op(S) \Leftrightarrow A_i \notin Op(S)$, i.e., for each transaction, there is either a commit or an abort in $S$, but not both;
    \item[c.] $(\forall p,q \in Op(S))p <_s q$ denotes the step $p$ in the schedule $S$ occurs before another step $q$ in the same schedule;
    \item[d.] $\left(\forall i, 1\leq i \leq m\right)\left(\forall p\in Op_i\right) p<_s A_i$ or $p<_s C_i$, i.e., the Commit or Abort operation always appears as the last step of a transaction.
    \item[e.] A transaction is still active if the Commit or Abort operation does not exist.
\end{itemize}
\end{definition}

\begin{example}\label{exp:schedule} We show an example of a schedule $S_1$ in the following:
\begin{equation}
S_1 = R_1[x_0]~R_3[x_0]~W_2[x_1]~W_1[y_1]~R_3[y_1]~R_1[y_1]~A_1~C_2.
\end{equation}
which involves three transactions, where $T_1 = R_1[x]W_1[y]R_1[y]A_1$, $T_2 = W_2[x]C_2$, and $T_3 = R_3[x]R_3[y]$ are failed (rollback), committed, and active transactions respectively.
The set of operations is $Op(S)=\{R_1[x], R_3[x], W_2[x], W_1[y], R_3[y], R_1[y]\}$. Any two operations in the operation set are in the order of $<_s$, e.g., $W_1[y] <_s R_3[y]$

% Consider the transaction set $\mathcal{T}=\{ T_1, T_2, T_3\}$, where
% $$T_1 = R_1[x]W_1[y]R_1[y]A_1, T_2 = W_2[x]C_2, T_3 = R_3[x]R_3[y]$$.
% We have schedule
% $$
% s = R_1[x]R_3[x]W_2[x]W_1[y]R_3[y]R_1[y]A_1C_2.
% $$
\end{example}

\begin{definition}\label{def:EdgeType} \textsc{\textbf{Conflict Dependency}\cite{adya2000generalized}.}
  Let $T_i, T_j$ be transactions in a schedule $S$, $T_i \neq T_j$. There exists a conflict dependency if two object-oriented operations $p_i\in T_i$ and $q_i \in T_j$ access the same object and at least one of them is a write, i.e.,
  $conf_{ij}[x] \in \{W_i W_j[x] , W_i R_j[x] , R_i W_j[x] \}$.
\end{definition}
Let $conf(S)$ denote all the conflict dependency in a schedule $S$, and it can be expressed as follows:
\begin{equation}
    conf(S)=\{conf_{ij}[x]|\forall x\in T_i.Obj \cap T_j.Obj \wedge T_i \neq T_j\}.
\end{equation}

\begin{example}\label{exp:conflict_dependency} Continuing Example \ref{exp:schedule}, all the conflict dependencies of $S_1$ are
\begin{equation}
conf(S_1)= \{R_1W_2[x], R_3W_2[x], W_1R_3[y]\}.
\end{equation}

\end{example}

\begin{definition}\textsc{\textbf{Conflict Graph}\cite{2002Concurrency}.}
  Let $S$ be a schedule, The conflict graph $G(S)=(V,E)$ of $S$, is defined by
  \begin{itemize}
    \item $V = T(S)$;
    \item $(T_i T_j) \in E \Leftrightarrow T_i \neq T_j \wedge \left(p_i \in T_i\right)\left(q_j \in T_j\right)(p_i q_j) \in conf(S)$.
  \end{itemize}
\end{definition}

Conflict graph is used to test if a schedule is serializable. Intuitively, an acyclic conflict graph indicates a serializable schedule, thus the consistent execution and final state. Figure \ref{fig:compare_ser_popg}(a) depicts the graphic representation of $S_1$.

% \begin{example}\label{exp:conflict_dependency} Continuing Example \ref{exp:schedule}, all the conflict dependencies of $s_1$ are:\textcolor{red}{example of conflict graph}
% \end{example}


% It is difficult to make connections between traditional conflict graphs and data anomalies. Intuitively, the existence of cycles in the conflict graph should illustrate having data anomalies in schedules. But even simple anomalies such as dirty reads and dirty writes are difficult to show in traditional conflict graphs by cycles as they did not express state-expressed operations. In example \ref{exp:schedule}, the transaction $T_2$ reads the object $y$ causing a dirty read due to the abort operation of $T_1$, but no cycle in the conflict graph of schedule $s$. To address this, we will redefine the edges in conflict graphs, establishing a one-to-one mapping between conflict graphs and data anomalies. %So that the abstract data anomalies can be intuitively represented in the conflict graph. 



==> tables/CCNewIsoAgorithms.tex <==

\begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c}
\toprule
\hline
\multicolumn{2}{c|}{Type of cycle}  &  \multicolumn{3}{c|}{RAT}         &  \multicolumn{3}{c|}{WAT}             & \multicolumn{9}{c}{IAT}     \\\hline
\multicolumn{2}{c|}{Target POP} &  \multicolumn{3}{c|}{WR}      &  \multicolumn{3}{c|}{WW}          & \multicolumn{3}{c|}{ \dots RW \dots }      &   \multicolumn{3}{c|}{ \dots RW  \dots WCR \dots }   &  \multicolumn{3}{c}{ \dots RW \dots WCW \dots }    \\\hline

\multicolumn{2}{c|}{-}  &  SDA        &DDA& MDA&  SDA           &DDA& MDA &  SDA        &DDA& MDA     &  SDA        &DDA& MDA   &  SDA        &DDA& MDA    \\\hline


CC protocol &   Levels &  &  &     &  &  &     &  &  &     & &  &     & &  &     \\\hline
\multirow{4}{*}{DLI}
             & NRW    & RC+SI+2PL-W & RC+SI+2PL-W & RC+SI+2PL-W    & RC+SI+2PL-W & RC+SI+2PL-W & RC+SI+2PL-W    & - & - & -     & - & - & -   & - & - & -  \\\cline{2-17}
             & NA     & ditto/CC-SDA & ditto/CC-DDA & ditto/CC-NS    & ditto/CC-SDA & ditto/CC-DDA & CC-NS     & CC-NS & CC-NS & CC-NS     & CC-NS & CC-NS & CC-NS     & CC-NS & CC-NS & CC-NS    \\\hline

\multirow{4}{*}{2PL+MVCC}
             & NRW    & RC+SI & RC+SI & RC+SI    & ditto & ditto & ditto    & - & - & -     & - & - & -   & - & - & -  \\\cline{2-17}
             & NA     & RC+SI & RC+SI & RC+SI    & ditto & ditto & ditto    & 2PL & 2PL & 2PL    & 2PL & 2PL & 2PL    & 2PL & 2PL & 2PL  \\\hline

\multirow{4}{*}{TO}
             & NRW    & TO-R/RC+2PL-P & TO-R/RC+2PL-P & TO-R/RC+2PL-P    & ditto & ditto & ditto    & - & - & -     & - & - & -   & - & - & -  \\\cline{2-17}
             & NA     & ditto & ditto & ditto    & ditto & ditto & ditto     & TO+2PL-P & TO+2PL-P & TP+2PL-P     & TO+2PL-P & TO+2PL-P & TP+2PL-P     & TO+2PL-P & TO+2PL-P & TP+2PL-P    \\\hline

\multirow{4}{*}{TO+MVCC}
             & NRW    & TO-R/RC+SI & TO-R/RC+SI & TO-R/RC+SI    & ditto & ditto & ditto    & - & - & -     & - & - & -   & - & - & -  \\\cline{2-17}
             & NA     & ditto & ditto & ditto    & ditto & ditto & ditto     & TO+SI & TO+SI & TP+SI     & TO+SI & TO+SI & TP+SI     & TO+SI & TO+SI & TP+SI    \\\hline

\multirow{4}{*}{OCC+MVCC}
             & NRW    & TO-R/RC+SI & TO-R/RC+SI & TO-R/RC+SI    & ditto & ditto & ditto    & - & - & -     & - & - & -   & - & - & -  \\\cline{2-17}
             & NA     & ditto & ditto & ditto    & ditto & ditto & ditto     & TO+SI & TO+SI & TP+SI     & TO+SI & TO+SI & TP+SI     & TO+SI & TO+SI & TP+SI    \\\hline

\multirow{4}{*}{SSI}
             & NRW    & RC+SI & RC+SI & RC+SI    & ditto & ditto & ditto    & - & - & -     & - & - & -   & - & - & -  \\\cline{2-17}
             & NA     & ditto & ditto & ditto    & ditto & ditto & ditto     & CC-SSI & CC-SSI & CC-SSI     & Undo & Undo & Undo     & Undo & Undo & Undo    \\\hline

\multirow{4}{*}{WSI}
             & NRW    & RC+SI & RC+SI & RC+SI    & ditto & ditto & ditto    & - & - & -     & - & - & -   & - & - & -  \\\cline{2-17}
             & NA     & ditto & ditto & ditto    & ditto & ditto & ditto     & CC-WSI & CC-WSI & CC-WSI     & CC-WSI & CC-WSI & CC-WSI     & CC-WSI & CC-WSI & CC-WSI    \\\hline

\bottomrule
\end{tabular}


==> tables/CCRules.tex <==
\setlength\extrarowheight{1.5pt}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}

\begin{tabular}{|l|l|l|l|}
\hline
\textbf{No}   & \textbf{Rules} & \textbf{Content} & \textbf{Notes} \\ \hline
1  & CC       &  Cycle check algorithm                  & known rules \\ \hline
2  & CC-SDA   &  Cycle check on two vertex and two edges(for SDA)      & we \\ \hline
3  & CC-DDA   &  Cycle check on two vertex and two edges(for DDA)      & we \\ \hline
4  & CC-WAT   &  Cycle check on two edges only for WAT  & we \\ \hline
5  & CC-NS    &  Cycle check on more then N(N $ \geq $ 3) skips and rollback one transaction  & we \\ \hline
6  & RC       &  Read Committed                         & known rules \\ \hline
7  & SI       &  Snapshot Reads to eliminate Phantom data anomaly & known rules \\ \hline
8  & 2PL      &  Locking protocol(2PL/SS2PL)            & known rules \\ \hline
9  & 2PL-W    &  Apply write lock only(only eliminate WW conflict relation) & known rules \\ \hline
10 & 2PL-R    &  Apply Read lock(2PL for Serializable)  & known rules \\ \hline
11 & 2PL-RW   &  Apply read and write lock(2PL for Serializable), it equals to 2PL-R & known rules \\ \hline
12 & 2PL-WO   &  Apply write lock only and sort write locks to avoid deadlock   & known rules \\ \hline
13 & 2PL-WNW  &  Apply write lock with No Wait strategy(deadlock can not occur) & known rules \\ \hline
14 & 2PL-WWD  &  Apply write lock with Wait Die strategy(deadlock may occur) & known rules \\ \hline
15 & 2PL-CC   &  Apply write lock and merge CC          & we \\ \hline
16 & 2PL-P    &  Locking protocol for predicate operation(predicate lock)         & known rules \\ \hline
17 & CC-SW    &  SSI or WSI                             & known rules \\ \hline
18 & CC-SSI   &  SSI algorithm                          & known rules \\ \hline
19 & CC-WSI   &  WSI algorithm                          & known rules \\ \hline
20 & TO       &  TO algorithm(for read and write operation)                    & known rules \\ \hline
21 & TO-R     &  TO algorithm for read operation                               & known rules \\ \hline
22 & TO-NW    &  TO algorithm with No Wait strategy(deadlock can not occur)    & known rules \\ \hline
23 & TO-WD    &  TO algorithm with Wait Die strategy(deadlock may occur)       & known rules  \\ \hline
24 & TO-CC    &  TO algorithm merge cycle check                                & we \\ \hline
25 & TO-DTA   &  TO algorithm(Dynamic timestamp allocate)                      & known rules \\ \hline
26 & OCC      &  OCC algorithm (reduce conflict duration)                      & known rules \\ \hline
27 & OCC-NW   &  OCC algorithm with No Wait strategy(deadlock can not occur)   & known rules \\ \hline
28 & OCC-WD   &  OCC algorithm with Wait Die strategy(deadlock can not occur)  & known rules \\ \hline
29 & OCC-CC   &  OCC algorithm merge cycle check  & we \\ \hline
\end{tabular}

% 19 It can effectively reduce the rollback rate of write conflicts

==> tables/algorithmAnalysis.tex <==
\setlength\extrarowheight{1.5pt}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}

\begin{tabular}{|c|c|l|l|l|}
\hline
\multicolumn{2}{|c|}{\textbf{Types   of Anomalies}} & \multicolumn{1}{c|}{\textbf{Cycle Check Algorithm}}  & \multicolumn{1}{c|}{\textbf{Rule-based Algorithm}}                                                        & 
\multicolumn{1}{c|}{\textbf{Notes}}  
\\ \hline
\multirow{3}{*}{RAT}      & SDA & CC-NS    & RC: Read Committed  & Table \ref{table:anomaly_statistics} shows SDA has 83.10\%, so we should use the rule to avoid SDA \\ \cline{2-5} 
                          & DDA & CC-NS    & RC                  & Table \ref{table:anomaly_statistics} shows DDA has 16.12\%, so we should use the rule to avoid DDA \\ \cline{2-5} 
                          & MDA & CC: Cycle check    & RC           & - \\ \hline
\multirow{3}{*}{WAT}      & SDA & CC-NS    & 2PL: two-phase locking protocol  & 2PL is a rule \\ \cline{2-5} 
                          & DDA & CC-NS    & 2PL           & ditto \\ \cline{2-5} 
                          & MDA & CC        & 2PL or CC-NS    & CC-NS: Cycle check on more then three edges and rollback one transaction \\  \hline
\multirow{3}{*}{IAT}      & SDA & CC-NS    & 2PL or CC-NS    & - \\ \cline{2-5} 
                          & DDA & CC-NS    & 2PL or CC-NS    & - \\ \cline{2-5} 
                          & MDA & CC        & 2PL or CC-NS     & -   \\ \hline
\end{tabular}

==> tables/algorithmAnalysisByAllDAs.tex <==
\setlength\extrarowheight{1.5pt}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}

\begin{tabular}{|c|c|l|l|l|}
\hline
\multicolumn{2}{|c|}{\textbf{Types   of Anomalies}}  & Anomalies  & \multicolumn{1}{c|}{\textbf{Cycle Check Algorithm}}  & \multicolumn{1}{c|}{\textbf{Rule-based Algorithm}}
\\ \hline
\multirow{14}{*}{RAT}     & SDA            & Dirty   Read                             & CC-SDA   & RC  \\ \cline{2-5} 
                          & SDA            & Non-repeatable Read                      & CC-SDA   & RC  \\ \cline{2-5}  
                          & SDA            & Intermediate Read                        & CC-SDA   & RC   \\ \cline{2-5}  
                          & SDA            & \textbf{Intermediate Read Committed}     & CC-SDA   & RC   \\ \cline{2-5}  
                          & SDA            & \textbf{Lost Self Update}                & CC-SDA   & RC   \\ \cline{2-5}         
                          & DDA            & \textbf{Write-Read   Skew}               & CC-DDA   & RC   \\ \cline{2-5} 
                          & DDA            & \textbf{Write-Read   Skew Committed}     & CC-DDA   & RC   \\ \cline{2-5} 
                          & DDA            & \textbf{Double-Write Skew 1}             & CC-DDA   & RC   \\ \cline{2-5} 
                          & DDA            & \textbf{Double-Write Skew 1 Committed}   & CC-DDA   & RC   \\ \cline{2-5} 
                          & DDA            & \textbf{Double-Write Skew 2}             & CC-DDA   & RC   \\ \cline{2-5} 
                          & DDA            & Read   Skew                              & CC-DDA   & RC   \\ \cline{2-5} 
                          & DDA            & \textbf{Read Skew 2}                     & CC-DDA   & RC   \\ \cline{2-5} 
                          & DDA            & \textbf{Read Skew 2 Committed}           & CC-DDA   & RC   \\ \cline{2-5} 
                          & MDA            & \textbf{Step RAT}                        & CC       & RC   \\ \hline
\multirow{11}{*}{WAT}     & SDA            & Dirty   Write                            & CC-SDA   & 2PL   \\ \cline{2-5}  
                          & SDA            & \textbf{Full-Write}                      & CC-SDA   & 2PL   \\ \cline{2-5}  
                          & SDA            & \textbf{Full-Write Committed}            & CC-SDA   & 2PL   \\ \cline{2-5} 
                          & SDA            & Lost   Update                            & CC-SDA   & 2PL   \\ \cline{2-5} 
                          & SDA            & \textbf{Lost Self Update Committed}      & CC-SDA   & 2PL   \\ \cline{2-5} 
                          & DDA            & \textbf{Double-Write   Skew 2 Committed} & CC-DDA   & 2PL   \\ \cline{2-5} 
                          & DDA            & \textbf{Full-Write   Skew}               & CC-DDA   & 2PL   \\ \cline{2-5} 
                          & DDA            & \textbf{Full-Write   Skew Committed}     & CC-DDA   & 2PL   \\ \cline{2-5} 
                          & DDA            & \textbf{Read-Write   Skew 1}             & CC-DDA   & 2PL   \\ \cline{2-5} 
                          & DDA            & \textbf{Read-Write   Skew 2}             & CC-DDA   & 2PL   \\ \cline{2-5} 
                          & MDA            & \textbf{Step   WAT}                      & CC       & 2PL or CC-NS   \\ \hline
\multirow{6}{*}{IAT}      & SDA            & \textbf{Non-repeatable   Read Committed}       & CC-SDA            & 2PL or CC-SDA or CC-WSI    \\ \cline{2-5} 
                          & SDA            & \textbf{Lost   Update Committed}               & CC-SDA            & 2PL or CC-SDA or CC-WSI    \\ \cline{2-5} 
                          & DDA            & \textbf{Read   Skew Committed}                 & CC-DDA            & 2PL or CC-DDA or CC-WSI    \\ \cline{2-5}  
                          & DDA            & \textbf{Read-Write   Skew 1 Committed}         & CC-DDA            & 2PL or CC-DDA or CC-WSI    \\ \cline{2-5}  
                          & DDA            & Write   Skew                                   & CC-DDA            & 2PL or CC-DDA or CC-SSI or CC-WSI    \\ \cline{2-5}  
                          & MDA            & \textbf{Step   IAT}                            & CC       & 2PL or CC-NS     \\ \hline
\end{tabular}

==> tables/cc_algorithm_isolation_level.tex <==

\begin{tabular}{c|c|c|c|c|c|c|c|c}
\toprule
\hline
\multicolumn{2}{c|}{Type of cycle}  &  \multicolumn{2}{c|}{RAT}         &  \multicolumn{2}{c|}{WAT}             & \multicolumn{3}{c}{IAT}     \\\hline
\multicolumn{2}{c|}{Target POP} &  \multicolumn{2}{c|}{WR}      &  \multicolumn{2}{c|}{WW}          & \multicolumn{1}{c|}{ \dots RW \dots }      &   \multicolumn{1}{c|}{ \dots RW  \dots WCR \dots }   &  \multicolumn{1}{c}{ \dots RW \dots WCW \dots }    \\\hline

\multicolumn{2}{c|}{-}  & SDA/DDA & MDA    & SDA/DDA & MDA     & SDA/DDA/MDA         & SDA/DDA/MDA    & SDA/DDA/MDA    \\\hline


CC protocol &   Levels & &   & &   & & &      \\\hline
\multirow{4}{*}{2PL}
             & RU    & - & -    & 2PL-W & 2PL-W     & - & - & -       \\\cline{2-9}
             & RC    & RC& RC      & {$\uparrow$}  & {$\uparrow$}  & - & - & -   \\\cline{2-9}
             & RR    & RC+2PL-P & RC+2PL-P    & {$\uparrow$} & {$\uparrow$}     & - & - & -  \\\cline{2-9}
             & S     & {$\uparrow$} & {$\uparrow$}    & {$\uparrow$} & {$\uparrow$}     & 2PL+2PL-R & 2PL+2PL-R     & 2PL+2PL-R    \\\hline

\multirow{4}{*}{2PL+MVCC}
             & RU    & - & -    & 2PL-W & 2PL-W     & - & - & -   \\\cline{2-9}
             & RC    & RC & RC      & {$\uparrow$} & {$\uparrow$}     & - & - & -   \\\cline{2-9}
             & RR    & RC+SI& RC+SI & {$\uparrow$} & {$\uparrow$}    & - & - & -  \\\cline{2-9}
             & S     & RC+SI & RC+SI    & {$\uparrow$} & {$\uparrow$}    & 2PL & 2PL & 2PL  \\\hline

\multirow{4}{*}{TO}
             & RU    & - & -    & TO-NW & TO-NW     & - & - & -   \\\cline{2-9}
             & RC    & TO-R/RC & TO-R/RC      & {$\uparrow$} & {$\uparrow$}     & - & - & -   \\\cline{2-9}
             & RR    & TO-R/RC+2PL-P & TO-R/RC+2PL-P    & {$\uparrow$} & {$\uparrow$}    & - & - & -  \\\cline{2-9}
             & S     & {$\uparrow$} & {$\uparrow$}    & {$\uparrow$} & {$\uparrow$}    & TO+2PL-P & TO+2PL-P & TP+2PL-P    \\\hline

\multirow{4}{*}{TO+MVCC}
             & RU    & - & -    & TO-NW & TO-NW     & - & - & -   \\\cline{2-9}
             & RC    & TO-R/RC & TO-R/RC      & {$\uparrow$} & {$\uparrow$}     & - & - & -   \\\cline{2-9}
             & RR    & TO-R/RC+SI & TO-R/RC+SI    & {$\uparrow$} & {$\uparrow$}   & - & - & -  \\\cline{2-9}
             & S     & {$\uparrow$}   & {$\uparrow$} & {$\uparrow$} & {$\uparrow$}     & TO+SI & TO+SI     & TO+SI    \\\hline

\multirow{4}{*}{OCC+MVCC}
             & RU    & - & -    & TO-NW & TO-NW     & - & -     & -   \\\cline{2-9}
             & RC    & TO-R/RC & TO-R/RC      & {$\uparrow$} & {$\uparrow$}    & - & -     & -   \\\cline{2-9}
             & RR    & TO-R/RC+SI & TO-R/RC+SI    & {$\uparrow$} & {$\uparrow$}    & - & -     & -  \\\cline{2-9}
             & S     & {$\uparrow$} & {$\uparrow$}    & {$\uparrow$} & {$\uparrow$}     & TO+SI & TO+SI     & TO+SI    \\\hline

\multirow{4}{*}{SSI+2PL/TO}
             & RU    & - & -    & 2PL-W & 2PL-W     & - & - & -   \\\cline{2-9}
             & RC    & RC & RC     & {$\uparrow$} & {$\uparrow$}    & - & - & -   \\\cline{2-9}
             & RR    & RC+SI & RC+SI    & {$\uparrow$} & {$\uparrow$}    & - & \textcolor{red}{SI} & -  \\\cline{2-9}
             & S     & {$\uparrow$} & {$\uparrow$}    & {$\uparrow$} & {$\uparrow$}     & CC-SSI  & {$\uparrow$}  & \textcolor{red}{Undo}    \\\hline

\multirow{4}{*}{WSI+2PL/TO}
             & RU    & - & -    & 2PL-W & 2PL-W     & - & - & -   \\\cline{2-9}
             & RC    & RC & RC     & {$\uparrow$} & {$\uparrow$}    & - & - & -   \\\cline{2-9}
             & RR    & RC+SI & RC+SI    & {$\uparrow$} & {$\uparrow$}    & - & \textcolor{red}{SI} & -  \\\cline{2-9}
             & S     & {$\uparrow$} & {$\uparrow$}    & {$\uparrow$} & {$\uparrow$}     & CC-WSI    & {$\uparrow$}  & CC-WSI    \\\hline

\multirow{2}{*}{\textcolor{red}{\textbf{we}}}
             & NRW    & RC+SI+2PL-W & RC+SI+2PL-W    & RC+SI+2PL-W & RC+SI+2PL-W    & - & - & -  \\\cline{2-9}
             & NA     & {$\uparrow$} or \textcolor{red}{CC-SDA/CC-DDA} & {$\uparrow$} or \textcolor{red}{CC-NS}    & {$\uparrow$} or \textcolor{red}{CC-SDA/CC-DDA}  & {$\uparrow$} or \textcolor{red}{CC-NS}     & \textcolor{red}{CC-NS} & \textcolor{red}{CC-NS} & \textcolor{red}{CC-NS}    \\\hline
\bottomrule
\end{tabular}


==> tables/concurrency_model.tex <==
\begin{tabular}{llllllll}
\toprule
\hline
CC algorithm             & RR & WR      & WW & RW & WCR & WCW & total    \\\hline
2PL          & 2  & 0       &  0  & 0   & 2   & 2   & 6/12  \\\hline
2PL+MVCC     & 2  & 2  & 0  & 1  & 2   & 2   & 8/12  \\\hline
TO           & 2  & 1       & 1  & 1  & 2   & 2   & 9/12  \\\hline
TO+MVCC      & 2  & 2       & 1  & 2  & 2   & 2   & 11/12 \\\hline
OCC+ MVCC    & 2  & 2       & 0   & 2  & 2   & 2   & 10/12 \\\hline

OCC+TO+MVCC  & 2  & 2       & 1  & 2  & 2   & 2   & 11/12 \\\hline
SILO+TO+OCC  & 2  & 1       & 0   & 0   & 2   & 2   & 7/12  \\\hline
SSI+MVCC     & 2  & 2       & 0  & 2  & 2   & 2   & 10/12 \\\hline
% OCC+SSI+MVCC & 2  & 2       & 0   & 2  & 2   & 2   & 10/12 \\\hline
OCC+WSI+MVCC & 2  & 2        & 2 & 0   & 2   & 2   & 10/12  \\\hline
\bottomrule
\end{tabular}

==> tables/conflict_graph_comparison.tex <==
\begin{tabular}{p{1.5cm}|p{3cm}|p{3cm}}
\toprule
\hline
    
 &
 Conflict graph
 &
 POP graph
  \\ \hline




Purpose & Model conflict serialization &  Model all data anomalies   \\ \hline 
\#Edge type & 3 conflicts (WW,WR,RW) &  9 POPs (in Lemma \ref{lemma:pop_types})   \\ \hline 
Data structure & Directed graphs &  Directed graphs   \\ \hline 

Expressive ness & Limited to describe data anomalies, can not describe Dirty Write, Dirty Read, and Intermediate Read & Can express all POPs, so Coo can define all data anomalies    \\ \hline 

Added value & Correlate to conflict serializable schedule, but not to specific data anomalies & Correlate directed cycles, data anomalies, and consistency together  \\ \hline 
\bottomrule

\end{tabular}

==> tables/evaluation_anomaly_statistics.tex <==


\begin{tabular}{c|c|c|c}
\toprule
\hline
    Class               & Sub- &               Anomaly name                                    &  Perc                             \\ \hline
\multirow{10}{*}{RAT}  & SDA & Dirty Read                       & 16.68\% \\ %& \multirow{9}{*}{33.79 \%} \\
                   & SDA & Intermediate Read                & 5.90\%                             \\
                   & SDA & Lost Self Update              & 5.49\%                             \\
                   & SDA & Non-repeatable Read                     & 5.33\%                             \\
                   & DDA &  Read Skew 2                & 1.85\%                             \\
                   & DDA & Write-read Skew                      & 1.59\%                             \\
                   & DDA & Read Skew                        & 1.52\%                            \\
                   & MDA & Step RAT                         & 0.67\%                            \\
                   & DDA & Write-read Skew Committed      & 0.26\%                             \\
                   & DDA & Double-write Skew 1 Committed & 0.26\%                             \\\hline
\multirow{12}{*}{WAT} & SDA & Dirty Write                      & 36.13\% \\% & \multirow{14}{*}{62.45 \%} \\
                   & SDA & Full-write                       & 6.71\%                            \\
                   & SDA & Lost Update                      & 5.31\%                             \\
                   & DDA & Read-write Skew 2             & 1.76\%                             \\
                   & DDA & Double-write Skew 1            & 1.58\%                             \\
                   & DDA & Read-write Skew 1               & 1.53\%                             \\
                   & DDA & Full-write Skew                 & 1.51\%                             \\
                   & DDA & Double-write Skew 2            & 1.51\%                             \\
                   & DDA & Full-write Skew Committed      & 0.23\%                             \\
                   & DDA & Double-write Skew 2 Committed & 0.23\%                             \\
                   & MDA & Step WAT                         & 0.09\%                             \\
                   & SDA & Lost Self Update Committed   & 0.04\%                             \\\hline
\multirow{6}{*}{IAT}  & DDA & Write Skew                       & 1.79\%  \\ %& \multirow{6}{*}{3.76 \%} \\
                   & SDA & Non-repeatable Read Committed  & 0.74\%                            \\
                   & SDA & Lost Update Committed           & 0.74\%                             \\
                   & DDA & Read-write Skew 1 Committed   & 0.23\%                             \\
                   & DDA & Read Skew Committed             & 0.23\%                             \\
                   & MDA & Step IAT                         & 0.02\%      \\\hline
\bottomrule                      
\end{tabular}




% \begin{tabular}{c|c|c|c}
% \toprule
% \hline
%     Class               & Sub- &               Anomaly name                                    &  Perc                             \\ \hline
% \multirow{9}{*}{RAT}  & SDA & Dirty Read                       & 16.68\% \\ %& \multirow{9}{*}{33.79 \%} \\
%                   & SDA & Intermediate Read                & 5.86\%                             \\
%                   & SDA & Non-repeatable Read             & 5.34\%                             \\
%                   & DDA & Read Skew 2                     & 1.86\%                             \\
%                   & DDA & Write-Read Skew                 & 1.59\%                             \\
%                   & DDA & Read Skew                        & 1.53\%                             \\
%                   & MDA & Step RAT                         & 0.41\%                            \\
%                   & DDA & Write-Read Skew Committed      & 0.26\%                             \\
%                   & DDA & Double-Write Skew 1 Committed & 0.26\%                             \\\hline
% \multirow{14}{*}{WAT} & SDA & Dirty Write                      & 36.13\% \\% & \multirow{14}{*}{62.45 \%} \\
%                   & SDA & Full-Write                       & 11.28\%                            \\
%                   & SDA & Lost Update                      & 5.31\%                             \\
%                   & DDA & Read-Write Skew 2             & 1.76\%                             \\
%                   & DDA & Double-Write Skew 1            & 1.58\%                             \\
%                   & DDA & Read-Write Skew 1               & 1.53\%                             \\
%                   & DDA & Full-Write Skew                 & 1.51\%                             \\
%                   & DDA & Double-Write Skew 2            & 1.51\%                             \\
%                   & SDA & Full-Write Committed            & 0.74\%                             \\
%                   & MDA & Step WAT                         & 0.35\%                             \\
%                   & SDA & Lost Self Update               & 0.23\%                             \\
%                   & DDA & Full-Write Skew Committed      & 0.23\%                             \\
%                   & DDA & Double-Write Skew 2 Committed & 0.23\%                             \\
%                   & SDA & Lost Self Update Committed   & 0.04\%                             \\\hline
% \multirow{6}{*}{IAT}  & DDA & Write Skew                       & 1.79\%  \\ %& \multirow{6}{*}{3.76 \%} \\
%                   & SDA & Non-repeatable Read Committed  & 0.74\%                            \\
%                   & SDA & Lost Update Committed           & 0.74\%                             \\
%                   & DDA & Read-Write Skew 1 Committed   & 0.23\%                             \\
%                   & DDA & Read Skew Committed             & 0.23\%                             \\
%                   & MDA & Step IAT                         & 0.02\%      \\\hline
% \bottomrule                      
% \end{tabular}

==> tables/evaluation_anomaly_statistics_edge.tex <==


\begin{tabular}{c|c|c|c|c|c|c|c|c}
\toprule
\hline
Edge        & RW	& WR	&   WW	&  WA	&  RA	&   WC	& WCR	&  WCW    \\ \hline
History & 23.14\% & 22.01\% & 21.98\%	& 10.18\%	& 10.18\%	& 10.18\%	& 1.17\%	& 1.16\%		 \\\hline
Cycles & 18.90\% & 25.88\% & 32.45\%	& 6.52\%	& 6.10\%	& 7.23\%	& 1.50\%	& 1.41\%		 \\\hline

% RW	& 23.14\%		 \\\hline
% WR	& 22.01\%		 \\\hline
% WW	& 21.98\%		 \\\hline
% WA	& 10.18\%		 \\\hline
% RA	& 10.18\%		 \\\hline
% WC	& 10.18\%		 \\\hline
% WCR	& 1.17\%		 \\\hline
% WCW	& 1.16\%		 \\\hline

\bottomrule                      
\end{tabular}

==> tables/evaluation_anomaly_statistics_sub.tex <==

\begin{tabular}{c|c|c|c|c}
\toprule
\hline
                   & SDA &  DDA   &  MDA         &     Sum                      \\ \hline
RAT	& 33.41\%	&   5.51\%	& 	0.67\%	& 	39.59\% \\\hline
WAT	& 48.20\%	& 	8.36\%	& 	0.09\%	& 	56.65\% \\\hline
IAT	& 1.48\%	& 	2.25\%	& 	0.02\%	& 	3.76\% \\\hline
Sum	& 83.10\%	& 	16.12\%	& 	0.78\%	& 	 \\\hline

\bottomrule                      
\end{tabular}


% \begin{tabular}{c|c|c|c|c}
% \toprule
% \hline
%                   & SDA &  DDA   &  MDA         &     Sum                      \\ \hline
% RAT	& 27.88\%	&   5.51\%	& 	0.41\%	& 	33.79\% \\\hline
% WAT	& 53.74\%	& 	8.36\%	& 	0.35\%	& 	62.45\% \\\hline
% IAT	& 1.48\%	& 	2.25\%	& 	0.02\%	& 	3.76\% \\\hline
% Sum	& 83.10\%	& 	16.12\%	& 	0.78\%	& 	 \\\hline

% \bottomrule                      
% \end{tabular}

==> tables/evaluation_databases_intro.tex <==
\begin{tabular}{c|c|c|c|c|c|c|c|c}
\toprule
\hline

\rotatebox[origin=c]{270}{Isolation Levels} & \rotatebox[origin=c]{270}{MongoDB 4.4.4} &  \multicolumn{1}{c|}{ \rotatebox[origin=c]{270}{OceanBase (Oracle)}}       &       \normalfont{\rotatebox[origin=c]{270}{CockroachDB}} & \multicolumn{1}{c|}{\rotatebox[origin=c]{270}{TIDB}} & \multicolumn{1}{c|}{\rotatebox[origin=c]{270}{PostgreSQL}} & \multicolumn{1}{c|}{\rotatebox[origin=c]{270}{Oracle}} & \multicolumn{1}{c|}{\rotatebox[origin=c]{270}{SQL Server (Pessimistic)}} & \multicolumn{1}{c}{\rotatebox[origin=c]{270}{MySQL}}                     \\ \hline
SER	& x	&   o	& $\star$	& 	x  & o & o & o & o\\\hline
SI	& $\star$	&   x	& x	& 	o  & x & x & o & x\\\hline
RR	& x	&   o	& x	& 	o  & o & x & o & $\star$ \\\hline
RC	& x	&   $\star$	& x	& 	$\star$  & $\star$ & $\star$ & o & o\\\hline
RU	& x	&   x	& x	& 	x  & o & x & $\star$ & o\\\hline
% Core CC	& 2PL	&   TO-MVCC	& WSI	& 	2PL  & 	TO-MVCC & 	MVCC+2PL & 2PL & 	2PL+MVCC\\\hline
DLD	& No	&   No	& Yes	& 	Yes  & 	Yes & 	Yes & Yes & 	Yes\\\hline

\bottomrule                      
\end{tabular}



==> tables/evaluation_dynamic_rollback.tex <==
% \begin{tabular}{c|c|c|c|c|c|c}
% \toprule
% \hline
%   Workload &
%   OCC &
%   MaaT &
%   MVTO &
%   TO &
%   Wait$\_$die &
%   No$\_$wait \\ \hline


%  y1  & 0.09\% & 	0.03\% & 	0.01\% & 	0.01\% & 	0.02\% & 	0.02\% \\ \cline{2-7} 

%  y2  & 0.00\% & 	0.00\% & 	0.00\% & 	0.00\% & 	0.00\% & 	0.00\% \\ \cline{2-7} 

%  y3  & 0.04\% & 	0.01\% & 	0.00\% & 	0.00\% & 	0.01\% & 	0.01\% \\ \cline{2-7} 

%  y4  & 14.86\% & 	68.81\% & 	11.54\% & 	9.56\% & 	13.28\% & 	14.56\% \\ \hline 

%  t1  & 11.19\% & 	9.33\% & 	0.05\% & 	0.03\% & 	4.63\% & 	4.41\% \\ \cline{2-7}  

%  t2  & 5.10\% & 	4.04\% & 	0.19\% & 	0.18\% & 	4.39\% & 	4.71\% \\ \cline{2-7} 

%  t3  & 12.69\% & 	11.89\% & 	1.21\% & 	1.54\% & 	11.61\% & 	12.02\% \\ \hline 

% \bottomrule


% \end{tabular}

\begin{tabular}{c|c|c|c|c|c|c}
\toprule
\hline
  Workload &
  OCC &
  MaaT &
  MVTO &
  TO &
  SSI &
  No$\_$wait \\ \hline


 y1  & 0.09\% & 	0.03\% & 	0.01\% & 	0.01\% & 	0.05\% & 	0.02\% \\ \cline{2-7} 

 y2  & 0.00\% & 	0.00\% & 	0.00\% & 	0.00\% & 	0.00\% & 	0.00\% \\ \cline{2-7} 

 y3  & 0.04\% & 	0.01\% & 	0.00\% & 	0.00\% & 	0.01\% & 	0.01\% \\ \cline{2-7} 

 y4  & 14.86\% & 	68.81\% & 	11.54\% & 	9.56\% & 	47.51\% & 	14.56\% \\ \hline 

 t1  & 11.19\% & 	9.33\% & 	0.05\% & 	0.03\% & 	4.98\% & 	4.41\% \\ \cline{2-7}  

 t2  & 5.10\% & 	4.04\% & 	0.19\% & 	0.18\% & 	5.28\% & 	4.71\% \\ \cline{2-7} 

 t3  & 12.69\% & 	11.89\% & 	1.21\% & 	1.54\% & 	5.07\% & 	12.02\% \\ \hline 

\bottomrule


\end{tabular}

==> tables/evaluation_read_skew_example.tex <==

\begin{tabular}{c|p{0.7in}|c|c|p{0.7in}|c}
\toprule
\hline
\multicolumn{6}{c}{Preparation}\\\hline
1 & \multicolumn{5}{l}{DROP TABLE IF EXISTS t1}\\\hline
2 & \multicolumn{5}{l}{CREATE TABLE t1 (k INT PRIMARY KEY, v INT)}\\\hline
3 & \multicolumn{5}{l}{INSERT INTO t1 VALUES (0, 0)}\\\hline
4 & \multicolumn{5}{l}{INSERT INTO t1 VALUES (1, 0)}\\\hline
\bottomrule 
\cellcolor{gray!30} A & \multicolumn{5}{c}{\textbf{Generator:} Read Skew ($R_1[x_0]W_2[y_1]W_2[x_1]R_1[y_1]$)}\\\hline
Q & \multicolumn{1}{c|}{Session 1: $T_1$-SQL} & \multicolumn{2}{c|}{Operations} & \multicolumn{1}{c|}{Session 2: $T_2$-SQL} & Result\\\hline
1 & Begin & & & & -\\\hline
\multirow{2}{*}{2} & SELECT * FROM t1  & \multirow{2}{*}{$R_1[x_0]$} \tikzmark{a1}   & & & \multirow{2}{*}{(0,0)} \\
 &  WHERE k=0 &  & & & \\\hline
3 & & & & Begin & - \\\hline

\multirow{2}{*}{4} & & & \tikzmark{d1} \multirow{2}{*}{$W_2[y_1]$}  & UPDATE t1 SET v=1 & \multirow{2}{*}{-} \\\
 & & & & WHERE k=1 &  \\\hline

\multirow{2}{*}{5} & & & \tikzmark{b1}\multirow{2}{*}{$W_2[x_1]$}   & UPDATE t1 SET v=1  & \multirow{2}{*}{-} \\
 & & & & WHERE k=0 & \\\hline
\multirow{2}{*}{6} & SELECT * FROM t1 & \sout{$R_1[y_1]$} & & & \cellcolor{violet!20}Snapshot  \\
 & WHERE k=1 & $R_1[y_0]$ \tikzmark{c1}  & & & \cellcolor{violet!20} (1,0) \\\hline
7 & & & $C_2$ &  \cellcolor{violet!20}  Commit & -\\\hline
8 & Commit & $C_1$ & & & -\\\hline
\multicolumn{6}{c}{\cellcolor{green!16} \textbf{Checker:} Pass (\textbf{P}) with consistency} \\\hline
\bottomrule  

\cellcolor{gray!30} B & \multicolumn{5}{c}{\textbf{Generator:} Read Skew Committed ($R_1[x_0]W_2[y_1]W_2[x_1]C_2R_1[y_1]$)}\\\hline
Q & \multicolumn{1}{c|}{Session 1: $T_1$-SQL} & \multicolumn{2}{c|}{Operations} & \multicolumn{1}{c|}{Session 2: $T_2$-SQL} & Result\\\hline
1 & Begin & & & & -\\\hline
\multirow{2}{*}{2} & SELECT * FROM t1  & \multirow{2}{*}{$R_1[x_0]$} \tikzmark{a2} & & & \multirow{2}{*}{(0,0)}\\
 &  WHERE k=0 &  & & & \\\hline
3 & & & & Begin & - \\\hline
\multirow{2}{*}{4} & & & \tikzmark{c2} \multirow{2}{*}{$W_2[y_1]$} & UPDATE t1 SET v=1 & \multirow{2}{*}{-} \\\
 & & & & WHERE k=1 &  \\\hline

\multirow{2}{*}{5} & & & \tikzmark{b2} \multirow{2}{*}{$W_2[x_1]$} & UPDATE t1 SET v=1  & \multirow{2}{*}{-} \\
 & & & & WHERE k=0 & \\\hline
6 & & & $C_2$ & \cellcolor{violet!20} Commit & -\\\hline

\multirow{2}{*}{7} & SELECT * FROM t1 & \multirow{2}{*}{$R_1[y_1]$} \tikzmark{d2} & & & \cellcolor{violet!20}MV+RC \\
 & WHERE k=1 & & & & \cellcolor{violet!20} (1,1) \\\hline
8 & Commit & $C_1$ & & & -\\\hline
\multicolumn{6}{c}{\cellcolor{yellow!30} \textbf{Checker:} Anomaly (\textbf{A}) detected} \\\hline
\bottomrule  

\hline
% \multicolumn{6}{c}{Preparation}\\\hline
% 1 & \multicolumn{5}{l}{DROP TABLE IF EXISTS t1}\\\hline
% 2 & \multicolumn{5}{l}{CREATE TABLE t1 (k INT PRIMARY KEY, v INT)}\\\hline
% 3 & \multicolumn{5}{l}{INSERT INTO t1 VALUES (0, 0)}\\\hline
% 4 & \multicolumn{5}{l}{INSERT INTO t1 VALUES (1, 0)}\\\hline
% \bottomrule 
\cellcolor{gray!30} C & \multicolumn{5}{c}{\textbf{Generator:} Lost Update Committed ($R_1[x_0]W_2[x_1]W_1C_2[x_2]$)}\\\hline
Q & \multicolumn{1}{c|}{Session 1: $T_1$-SQL} & \multicolumn{2}{c|}{Operations} & \multicolumn{1}{c|}{Session 2: $T_2$-SQL} & Result\\\hline
1 & Begin & & & & -\\\hline
\multirow{2}{*}{2} & SELECT * FROM t1  & \multirow{2}{*}{$R_1[x_0]$} \tikzmark{aa1}   & & & \multirow{2}{*}{(0,0)} \\
 &  WHERE k=0 &  & & & \\\hline
3 & & & & Begin & - \\\hline

\multirow{2}{*}{4} & & & \tikzmark{bb1}\multirow{2}{*}{$W_2[x_1]$}   & UPDATE t1 SET v=1  & \multirow{2}{*}{-} \\
 & & & & WHERE k=0 & \\\hline
 
5 & & & $C_2$ & \cellcolor{violet!20} Commit & -\\\hline

\multirow{2}{*}{6} &  UPDATE t1 SET v=1 & \multirow{2}{*}{$W_1[y_1]$} \tikzmark{cc1} & & & \cellcolor{violet!20}Abort by\\
 & WHERE k=0 &   & & &  \cellcolor{violet!20}rules\\\hline
% 7 & & & $C_2$ &  \cellcolor{green!16} Commit & -\\\hline
% 8 & Commit & $C_1$ & & & -\\\hline
\multicolumn{6}{c}{\cellcolor{cyan!30} \textbf{Checker:} Rollback (\textbf{R}) by rules (2-RW found)} \\\hline
\bottomrule  

\begin{comment}
\cellcolor{gray!30} D & \multicolumn{5}{c}{\textbf{Generator:} Full-write Skew ($W_1[x_1]W_2[y_1]W_2[x_2]W_1[y_2]$)}\\\hline
Q & \multicolumn{1}{c|}{Session 1: $T_1$-SQL} & \multicolumn{2}{c|}{Operations} & \multicolumn{1}{c|}{Session 2: $T_2$-SQL} & Result\\\hline
1 & Begin & & & & -\\\hline

\multirow{2}{*}{2} &  UPDATE t1 SET v=1  & \multirow{2}{*}{$W_1[x_1]$} \tikzmark{aa2} & & & \multirow{2}{*}{-} \\
 &  WHERE k=0 &  & & & \\\hline
3 & & & & Begin & - \\\hline
\multirow{2}{*}{4} & & & \tikzmark{cc2} \multirow{2}{*}{$W_2[y_1]$} & UPDATE t1 SET v=2 & \multirow{2}{*}{-} \\\
 & & & & WHERE k=1 &  \\\hline

\multirow{2}{*}{5} & & & \tikzmark{bb2} \multirow{2}{*}{$W_2[x_2]$} & UPDATE t1 SET v=2  & \multirow{2}{*}{2PL Wait} \\
 & & & & WHERE k=0 & \\\hline
\multirow{2}{*}{6} &  UPDATE t1 SET v=1 & \multirow{2}{*}{$W_1[y_2]$} \tikzmark{dd2} & & & \cellcolor{violet!20} Abort by  \\
 & WHERE k=1 & & & & \cellcolor{violet!20} deadlock \\\hline
\multicolumn{6}{c}{\cellcolor{red!30} \textbf{Checker:} Deadlock (\textbf{D}) detected} \\\hline
\end{comment}



 \cellcolor{gray!30}                       & \multicolumn{4}{c}{  \textbf{Generator:} Step WAT} \\  
 \cellcolor{gray!30} \multirow{-2}{*}{  D }&   \multicolumn{4}{c}{  $W_1[x_1]W_2[y_1]W_3[z_1]W_3[y_2]W_2[x_2]W_1[z_2]$ }  \\ \hline

Q & \multicolumn{1}{c|}{Session 1: $T_1$-SQL} & \multicolumn{1}{c|}{Session 2: $T_2$-SQL} & \multicolumn{1}{c|}{Session 3: $T_3$-SQL} & Result\\\hline
1 & Begin & &  & -\\\hline

\multirow{2}{*}{2} &  UPDATE t1 SET v=1  & Begin & & \multirow{2}{*}{-} \\
 &  WHERE k=0 ($W_1[x_1]$) \tikzmark{xx1} &  & &  \\\hline
 
\multirow{2}{*}{3} & & UPDATE t1 SET v=1 & Begin & \multirow{2}{*}{-} \\\
 & & WHERE k=1 ($W_2[y_1]$) \tikzmark{yy1} & &    \\\hline
 
\multirow{2}{*}{4} & & \tikzmark{xx2} UPDATE t1 SET v=1 & UPDATE t1 SET v=2 & \multirow{2}{*}{-} \\\
 & & WHERE k=0 ($W_2[x_2]$) & WHERE k=2 ($W_3[z_1]$) \tikzmark{zz1} &    \\\hline
 
 \multirow{2}{*}{5} & & & UPDATE t1 SET v=2 & \multirow{2}{*}{-} \\\
 & &  & \tikzmark{yy2} WHERE k=1 ($W_3[y_2]$)  &  \\\hline
 
\multirow{2}{*}{6} & UPDATE t1 SET v=2 & & & \cellcolor{violet!20} 2PL Wait \\
 & WHERE k=2 ($W_1[z_2]$) \tikzmark{zz2} & & & \cellcolor{violet!20} deadlock \\\hline

\multicolumn{5}{c}{\cellcolor{red!30} \textbf{Checker:} Deadlock (\textbf{D}) detected} \\\hline
\bottomrule  
\end{tabular}


\begin{tikzpicture}[overlay, remember picture, shorten >=.5pt, shorten <=.5pt, transform canvas={yshift=.25\baselineskip}]
    \draw [magenta!70,->] ({pic cs:a1}) -- node [pos=0.45,above] {RW} ({pic cs:b1});
    \draw [magenta!70,->] ({pic cs:c1}) -- ({pic cs:d1})  node [pos=0.45,below] {RW};

    % \draw [->] ([yshift=.75pt]{pic cs:c}) -- ({pic cs:d});
    % \draw [->] ({pic cs:a}) [bend right] to ({pic cs:b});
    % \draw [->] ({pic cs:c}) [bend right] to  ({pic cs:d});
    \draw [magenta!70,->] ({pic cs:a2}) -- node [pos=0.45,above] {RW} ({pic cs:b2});
    \draw [magenta!70,->] ({pic cs:c2}) -- ({pic cs:d2})  node [pos=0.45,below] {WCR};
    
        \draw [magenta!70,->] ({pic cs:aa1}) -- node [pos=0.45,above] {RW} ({pic cs:bb1});
    \draw [magenta!70,->] ({pic cs:bb1}) -- ({pic cs:cc1})  node [pos=0.45,below] {WCW};

    % \draw [->] ([yshift=.75pt]{pic cs:c}) -- ({pic cs:d});
    % \draw [->] ({pic cs:a}) [bend right] to ({pic cs:b});
    % \draw [->] ({pic cs:c}) [bend right] to  ({pic cs:d});
%    \draw [magenta!70,->] ({pic cs:aa2}) -- node [pos=0.45,above] {WW} ({pic cs:bb2});
%    \draw [magenta!70,->] ({pic cs:cc2}) -- ({pic cs:dd2})  node [pos=0.45,below] {WW};
    
    \draw [magenta!70,->] ({pic cs:xx1}) -- node [pos=0.45,above] {WW} ({pic cs:xx2});
    \draw [magenta!70,->] ({pic cs:yy1}) -- ({pic cs:yy2})  node [pos=0.45,below] {yy2};
    \draw [magenta!70,->] ({pic cs:zz1}) -- node [pos=0.45,above] {WW} ({pic cs:zz2});
    
  \end{tikzpicture}

==> tables/evaluation_snapshot_strategies.tex <==
\begin{tabular}{c|p{0.45in}|p{0.45in}|p{0.45in}|p{0.45in}}
\toprule
\hline

% \rotatebox[origin=c]{270}{Databases} & \rotatebox[origin=c]{270}{Serializable} &  \multicolumn{1}{c|}{ \rotatebox[origin=c]{270}{Repeatable Read}}       &       \normalfont{\rotatebox[origin=c]{270}{Read Committed}} & \multicolumn{1}{c|}{\rotatebox[origin=c]{270}{Read Uncommitted}}       \\ \hline
Databases & SER & RR     &   RC & RU      \\ \hline


MySQL	& yes	&   yes, first read	& no & no \\\hline

SQL server & no	&  no	&  no  & no  \\\hline
TiDB	& /	&   yes	& no & /  \\\hline
Oracle	& yes 	&   /	& no & /  \\\hline
OceanBase	& yes 	&   yes	& no & /  \\\hline
PostgreSQL	& yes 	&   yes	& no & no \\\hline
CockroachDB	& no 	&   / & / & / \\\hline
MongoDB(SS)	&  	&   yes & / & / \\\hline
\bottomrule                      
\end{tabular}



==> tables/evaluation_static_rollback.tex <==
% \begin{tabular}{c|c|c|c|c|c|c|c}


% \toprule
% \hline
%  &
%   \multicolumn{1}{c|}{\textbf{ALL}} &
%   \multicolumn{1}{c|}{\textbf{OCC}} &
%   \multicolumn{1}{c|}{\textbf{MaaT}} &
%   \multicolumn{1}{c|}{\textbf{MVTO}} &
%   \multicolumn{1}{c|}{\textbf{TO}} &
%   \multicolumn{1}{c|}{\textbf{Wait$\_$die}} &
%   \multicolumn{1}{c}{\textbf{No$\_$wait}} \\ \hline
%  &
%   TRR &
%   FRR &
%   FRR &
%   FRR &
%   FRR &
%   FRR &
%   FRR \\ \hline
% \textbf{$\mathcal{H}$ (2,2,6)} & 1.41\%  & 3.32\% & 6.87\% & 16.47\% & 16.64\% & 21.31\% & 32.80\% \\ \hline
% \textbf{$\mathcal{H}$ (2,3,6)} & 2.17\%  & 3.02\% & 5.78\% & 11.99\% & 13.78\% & 19.43\% & 27.05\% \\ \hline
% \textbf{$\mathcal{H}$ (2,4,6)} & 1.72\%  & 2.26\% & 5.06\% & 10.22\% & 12.90\% & 18.59\% & 25.87\% \\ \hline
% \textbf{$\mathcal{H}$ (3,2,6)} & 2.27\%  & 2.85\% & 5.31\% & 11.90\% & 11.37\% & 17.85\% & 25.91\% \\ \hline
% \textbf{$\mathcal{H}$ (3,4,6)} & 1.43\%  & 1.97\% & 4.87\% & 8.32\%  & 10.98\% & 16.98\% & 21.36\% \\ \hline
% \bottomrule
% \end{tabular}

% \textbf{S (2,2,6)} & 1.41\% & 1.92\% & 3.32\% & 6.87\% & 16.47\% & 16.64\% & 21.31\% & 32.80\% \\ \hline
% \textbf{S (2,3,6)} & 2.17\% & 1.06\% & 3.02\% & 5.78\% & 11.99\% & 13.78\% & 19.43\% & 27.05\% \\ \hline
% \textbf{S (2,4,6)} & 1.72\% & 0.50\% & 2.26\% & 5.06\% & 10.22\% & 12.90\% & 18.59\% & 25.87\% \\ \hline
% \textbf{S (3,2,6)} & 2.27\% & 0.53\% & 2.85\% & 5.31\% & 11.90\% & 11.37\% & 17.85\% & 25.91\% \\ \hline
% \textbf{S (3,4,6)} & 1.43\% & 0.45\% & 1.97\% & 4.87\% & 8.32\%  & 10.98\% & 16.98\% & 21.36\% \\


\begin{tabular}{c|c|c|c|c|c|c|c}


\toprule
\hline
 &
  \multicolumn{1}{c|}{\textbf{ALL}} &
  \multicolumn{1}{c|}{\textbf{OCC}} &
  \multicolumn{1}{c|}{\textbf{MaaT}} &
  \multicolumn{1}{c|}{\textbf{MVTO}} &
  \multicolumn{1}{c|}{\textbf{TO}} &
  \multicolumn{1}{c|}{\textbf{SSI}} &
  \multicolumn{1}{c}{\textbf{No$\_$wait}} \\ \hline
 &
  TRR &
  FRR &
  FRR &
  FRR &
  FRR &
  FRR &
  FRR \\ \hline
\textbf{$\mathcal{H}$ (2,2,6)} & 69.82\%  & 3.48\% & 3.97\% & 1.53\% & 1.68\% & 1.72\% & 29.28\% \\ \hline
\textbf{$\mathcal{H}$ (3,2,6)} & 72.91\%  & 3.36\% & 3.94\% & 0.75\% & 0.87\% & 1.41\% & 25.20\% \\ \hline
\textbf{$\mathcal{H}$ (2,3,6)} & 52.09\%  & 7.71\% & 8.82\% & 3.29\% & 3.73\% & 3.53\% & 45.25\% \\ \hline
\textbf{$\mathcal{H}$ (2,4,6)} & 42.13\%  & 9.83\% & 11.37\% & 4.16\% & 4.80\% & 4.31\% & 52.16\% \\ \hline
\textbf{$\mathcal{H}$ (3,4,6)} & 46.40\%  & 21.86\% & 25.95\% & 4.36\%  & 6.01\% & 8.66\% & 45.46\% \\ \hline
\textbf{$\mathcal{H}$ (3,4,7)} & 58.36\%  & 20.17\% & 23.22\% & 5.28\%  & 6.45\% & 8.92\% & 38.26\% \\ \hline
\textbf{$\mathcal{H}$ (3,4,8)} & 69.65\%  &	16.71\%	& 18.73\% & 5.42\%	& 6.32\% & 7.98\% & 29.01\% \\ \hline
AVG & 58.77\%  &	11.87\%	& 13.71\% & 3.54\%	& 4.27\% & 5.22\% & 37.80\% \\ \hline
\bottomrule
\end{tabular}

% old data with no abort action in no_wait
% \textbf{$\mathcal{H}$ (2,2,6)} & 69.82\%  & 3.48\% & 3.97\% & 1.53\% & 1.68\% & 1.72\% & 0.90\% \\ \hline
% \textbf{$\mathcal{H}$ (3,2,6)} & 72.91\%  & 3.36\% & 3.94\% & 0.75\% & 0.87\% & 1.41\% & 6.88\% \\ \hline
% \textbf{$\mathcal{H}$ (2,3,6)} & 52.09\%  & 7.71\% & 8.82\% & 3.29\% & 3.73\% & 3.53\% & 2.66\% \\ \hline
% \textbf{$\mathcal{H}$ (2,4,6)} & 42.13\%  & 9.83\% & 11.37\% & 4.16\% & 4.80\% & 4.31\% & 30.19\% \\ \hline
% \textbf{$\mathcal{H}$ (3,4,6)} & 46.40\%  & 21.86\% & 25.95\% & 4.36\%  & 6.01\% & 8.66\% & 45.41\% \\ \hline
% \textbf{$\mathcal{H}$ (3,4,7)} & 58.36\%  & 20.17\% & 23.22\% & 5.28\%  & 6.45\% & 8.92\% & 38.26\% \\ \hline

% 	TRR	OCC	MAAT	 MVCC	TO	SSI	NO_WAIT
% #2-2-6	69.82%	3.48%	3.97%	1.53%	1.68%	1.72%	0.90%
% #2-3-6	52.09%	7.71%	8.82%	3.29%	3.73%	3.53%	2.66%
% #2-4-6	42.13%	9.83%	11.37%	4.16%	4.80%	4.31%	30.19%
% #3-2-6	72.91%	3.36%	3.94%	0.75%	0.87%	1.41%	6.88%
% #3-4-6	46.40%	21.86%	25.95%	4.36%	6.01%	8.66%	45.41%
% #3-4-7	58.36%	20.17%	23.22%	5.28%	6.45%	8.92%	38.26%


% \textbf{$\mathcal{H}$	(2,2,6)}	69.82%	3.48%	3.97%	1.53%	1.68%	1.72%	29.28%
% \textbf{$\mathcal{H}$	(3,2,6)}	72.91%	3.36%	3.94%	0.75%	0.87%	1.41%	25.20%
% \textbf{$\mathcal{H}$	(2,3,6)}	52.09%	7.71%	8.82%	3.29%	3.73%	3.53%	45.25%
% \textbf{$\mathcal{H}$	(2,4,6)}	42.13%	9.83%	11.37%	4.16%	4.80%	4.31%	52.16%
% \textbf{$\mathcal{H}$	(3,4,6)}	46.40%	21.86%	25.95%	4.36%	6.01%	8.66%	45.46%
% \textbf{$\mathcal{H}$	(3,4,7)}	58.36%	20.17%	23.22%	5.28%	6.45%	8.92%	38.26%
% \textbf{$\mathcal{H}$	(3,4,8)}	69.65%	16.71%	18.73%	5.42%	6.32%	7.98%	29.01%
% avg		58.77%	11.87%	13.71%	3.54%	4.27%	5.22%	37.80%


==> tables/evaluation_write_skew_example.tex <==
\begin{tabular}{c|p{0.7in}|c|c|p{0.7in}|c}
\toprule
\hline
% \multicolumn{6}{c}{Preparation}\\\hline
% 1 & \multicolumn{5}{l}{DROP TABLE IF EXISTS t1}\\\hline
% 2 & \multicolumn{5}{l}{CREATE TABLE t1 (k INT PRIMARY KEY, v INT)}\\\hline
% 3 & \multicolumn{5}{l}{INSERT INTO t1 VALUES (0, 0)}\\\hline
% 4 & \multicolumn{5}{l}{INSERT INTO t1 VALUES (1, 0)}\\\hline
% \bottomrule 
\multicolumn{6}{c}{\textbf{Generator:} Write Skew ($R_1[x_0]R_2[y_0]W_2[x_1]W_1[y_1]$)}\\\hline
Q & \multicolumn{1}{c|}{Session 1: $T_1$-SQL} & \multicolumn{2}{c|}{Operations} & \multicolumn{1}{c|}{Session 2: $T_2$-SQL} & Result\\\hline
1 & Begin & & & & -\\\hline
\multirow{2}{*}{2} & SELECT * FROM t1  & \multirow{2}{*}{$R_1[x_0]$} \tikzmark{aa1}   & & & \multirow{2}{*}{(0,0)} \\
 &  WHERE k=0 &  & & & \\\hline
3 & & & & Begin & - \\\hline

\multirow{2}{*}{4} & & & \tikzmark{dd1} \multirow{2}{*}{$R_2[y_0]$}  & SELECT * FROM t1 & \multirow{2}{*}{(1,0)} \\\
 & & & & WHERE k=1 &  \\\hline

\multirow{2}{*}{5} & & & \tikzmark{bb1}\multirow{2}{*}{$W_2[x_1]$}   & UPDATE t1 SET v=1  & \multirow{2}{*}{-} \\
 & & & & WHERE k=0 & \\\hline
\multirow{2}{*}{6} &  UPDATE t1 SET v=1 & \multirow{2}{*}{$W_1[y_1]$} \tikzmark{cc1} & & & \cellcolor{violet!20}Abort by\\
 & WHERE k=1 &   & & &  \cellcolor{violet!20}rules\\\hline
% 7 & & & $C_2$ &  \cellcolor{green!16} Commit & -\\\hline
% 8 & Commit & $C_1$ & & & -\\\hline
\multicolumn{6}{c}{\cellcolor{cyan!30} \textbf{Checker:} Rollback (\textbf{R}) by rules (2-RW found)} \\\hline
\bottomrule  

\multicolumn{6}{c}{\textbf{Generator:} Full-write Skew ($W_1[x_1]W_2[y_2]W_2[x_2]W_1[y_1]$)}\\\hline
Q & \multicolumn{1}{c|}{Session 1: $T_1$-SQL} & \multicolumn{2}{c|}{Operations} & \multicolumn{1}{c|}{Session 2: $T_2$-SQL} & Result\\\hline
1 & Begin & & & & -\\\hline

\multirow{2}{*}{2} &  UPDATE t1 SET v=1  & \multirow{2}{*}{$W_1[x_1]$} \tikzmark{aa2} & & & \multirow{2}{*}{-} \\
 &  WHERE k=0 &  & & & \\\hline
3 & & & & Begin & - \\\hline
\multirow{2}{*}{4} & & & \tikzmark{cc2} \multirow{2}{*}{$W_2[y_2]$} & UPDATE t1 SET v=2 & \multirow{2}{*}{-} \\\
 & & & & WHERE k=1 &  \\\hline

\multirow{2}{*}{5} & & & \tikzmark{bb2} \multirow{2}{*}{$W_2[x_2]$} & UPDATE t1 SET v=2  & \multirow{2}{*}{2PL Wait} \\
 & & & & WHERE k=0 & \\\hline
\multirow{2}{*}{6} &  UPDATE t1 SET v=1 & \multirow{2}{*}{$W_1[y_1]$} \tikzmark{dd2} & & & \cellcolor{violet!20} Abort by  \\
 & WHERE k=1 & & & & \cellcolor{violet!20} deadlock \\\hline
\multicolumn{6}{c}{\cellcolor{red!30} \textbf{Checker:} Deadlock (\textbf{D}) detected} \\\hline
\bottomrule  
\end{tabular}

\begin{tikzpicture}[overlay, remember picture, shorten >=.5pt, shorten <=.5pt, transform canvas={yshift=.25\baselineskip}]
    \draw [magenta!70,->] ({pic cs:aa1}) -- node [pos=0.45,above] {RW} ({pic cs:bb1});
    \draw [magenta!70,->] ({pic cs:dd1}) -- ({pic cs:cc1})  node [pos=0.45,below] {RW};

    % \draw [->] ([yshift=.75pt]{pic cs:c}) -- ({pic cs:d});
    % \draw [->] ({pic cs:a}) [bend right] to ({pic cs:b});
    % \draw [->] ({pic cs:c}) [bend right] to  ({pic cs:d});
    \draw [magenta!70,->] ({pic cs:aa2}) -- node [pos=0.45,above] {WW} ({pic cs:bb2});
    \draw [magenta!70,->] ({pic cs:cc2}) -- ({pic cs:dd2})  node [pos=0.45,below] {WW};
    
  \end{tikzpicture}

==> tables/isolation_level_performance.tex <==
% \begin{tabular}{c|cccc|ccc|ccc}
% \toprule \hline
% Workload    & SSI   & NRW    & RC & RU  & WAIT\_DIE & RC & RU & NO\_WAIT & RC & RU         \\\hline
% y1 & 445552  & 6.16\%   & 6.63\%  & 16.04\%    & 510021        & 2.28\%        & 13.73\%  & 478832       & 10.92\%      & 11.75\%  \\\hline
% y2 & 586457  & 1.88\%   & 7.18\%   & 9.04\%  & 464146        & 17.28\%       & 26.44\%  & 485169       & -8.41\%      & -5.50\%  \\\hline
% y3 & 553605  & -2.29\%  & 3.10\%   & 10.25\%   & 543264        & -2.53\%       & 15.35\%  & 482065       & 2.94\%       & -7.59\%  \\\hline
% y4 & 140474  & 531.19\% & 327.60\% & 706.78\%  & 113114        & 347.01\%      & 436.43\% & 117279       & 297.40\%     & 337.28\% \\\hline
% t1 & 374208  & 0.65\%   & 2.98\%  & 51.78\%   & 406490        & 7.36\%        & 28.57\%  & 408835       & 4.20\%       & 28.90\%  \\\hline
% t2 & 254915  & 0.22\%   & 1.53\%   & 32.33\%   & 266444        & 4.17\%        & 17.17\%  & 279314       & 4.08\%       & 13.54\% \\\hline
% t3 & 341092  & 0.86\%   & -1.47\%   & 37.75\%   & 151961        & 66.38\%        & 212.88\%  & 233255       & 60.04\%       & 173.88\% \\\hline

% \bottomrule
% \end{tabular}


\begin{tabular}{c|cccc|ccc|ccc}
\toprule \hline
Algorithm    &\multicolumn{4}{c|}{SSI}  &  \multicolumn{3}{c|}{WAIT\_DIE} &  \multicolumn{3}{c}{NO\_WAIT}       \\\hline
Workload    & S/NA   & NRW    & RC & RU  & S/NA  & RC & RU & S/NA  & RC & RU         \\\hline
y1 & 445552  & 6.16\%   & 6.63\%  & 16.04\%    & 510021        & 2.28\%        & 13.73\%  & 478832       & 10.92\%      & 11.75\%  \\\hline
y2 & 586457  & 1.88\%   & 7.18\%   & 9.04\%  & 464146        & 17.28\%       & 26.44\%  & 485169       & 4.44\%      & 1.93\%  \\\hline
y3 & 553605  & -2.29\%  & 3.10\%   & 10.25\%   & 543264        & -2.53\%       & 15.35\%  & 482065       & 0.59\%       & -1.16\%  \\\hline
y4 & 140474  & 531.19\% & 327.60\% & 706.78\%  & 113114        & 347.01\%      & 436.43\% & 117279       & 297.40\%     & 337.28\% \\\hline
t1 & 374208  & 0.65\%   & 2.98\%  & 51.78\%   & 406490        & 7.36\%        & 28.57\%  & 408835       & 4.20\%       & 28.90\%  \\\hline
t2 & 254915  & 0.22\%   & 1.53\%   & 32.33\%   & 266444        & 4.17\%        & 17.17\%  & 279314       & 4.08\%       & 13.54\% \\\hline
t3 & 341092  & 0.86\%   & -1.47\%   & 37.75\%   & 151961        & 66.38\%        & 212.88\%  & 233255       & 60.04\%       & 173.88\% \\\hline

\bottomrule
\end{tabular}





==> tables/new_isolation_level.tex <==
\begin{tabular}{lclcc}
\toprule
\hline
\multicolumn{2}{c}{Types   of Anomalies} & Anomaly name                                  & NRW                                  & NA                                   \\ \hline
% Class                & Sub-class    & Anomaly name                                  & NRW                                  & NA                                   \\ \hline
                       & SDA          & Dirty Read                                              & NP                         & NP                         \\ \cline{2-5} 
                       & SDA          & Non-repeatable Read                                     & NP                         & NP                         \\ \cline{2-5} 
                       & SDA          & Phantom                                                 & NP                         & NP                         \\ \cline{2-5}        
                       & SDA          & Intermediate Read                                       & NP                         & NP                         \\ \cline{2-5}
                       & SDA          & Intermediate Read Committed                                      & NP                         & NP                         \\ \cline{2-5}
                       & SDA          & Lost Self Update                & NP & NP \\ \cline{2-5}
                       & DDA          & Double-write Skew 2             & NP & NP \\ \cline{2-5}
                       & DDA          & Write-read Skew                               & NP                         & NP                         \\ \cline{2-5} 
                       & DDA          & Write-read Skew Committed                               & NP                         & NP                         \\ \cline{2-5} 
                       & DDA          & Double-write Skew 1                           & NP                         & NP                         \\ \cline{2-5}
                       & DDA          & Double-write Skew 1 Committed                           & NP                         & NP                         \\ \cline{2-5}
                       & DDA          & Write-read Skew                                         & NP                         & NP                         \\ \cline{2-5}                      
                       & DDA          & Read Skew                                               & NP                         & NP                         \\ \cline{2-5} 
                       & DDA          & Read Skew 2                                             & NP                         & NP                         \\ \cline{2-5} 
                       & DDA          & Read Skew 2 Committed                                   & NP                         & NP                         \\ \cline{2-5} 
\multirow{-10}{*}{RAT} & MDA                         & Step RAT                                                & NP                         & NP                         \\ \hline  
                       & SDA & Dirty Write                     & NP & NP \\ \cline{2-5} 
                       & SDA & Full-Write                      & NP & NP \\ \cline{2-5}
                       & SDA & Full-Write Committed            & NP & NP \\ \cline{2-5}                        
                       & SDA & Lost Update                     & NP & NP \\ \cline{2-5} 
                       & DDA & Double-write Skew 2   Committed & NP & NP \\ \cline{2-5}
                       & DDA & Full-write Skew                 & NP & NP \\ \cline{2-5} 
                       & DDA & Full-write Skew   Committed     & NP & NP \\ \cline{2-5}
                       & DDA & Read-write Skew 1               & NP & NP \\ \cline{2-5} 
                       & DDA & Read-write Skew 2               & NP & NP \\ \cline{2-5}                         
\multirow{-13}{*}{WAT} & MDA & Step WAT                        & NP & NP \\  \hline
                       & SDA                         & Non-repeatable Read Committed                           & P                      & NP                         \\ \cline{2-5} 
                       & SDA                         & Lost Update Committed                                   & P                             & NP                         \\ \cline{2-5} 
                       & DDA                         & Read Skew Committed                                     & P                             & NP                         \\ \cline{2-5} 
                       & DDA                         & Read-Write Skew 1 Committed                             & P                             & NP                         \\ \cline{2-5} 
                       & DDA                         & Write Skew                                              & P                             & NP                         \\ \cline{2-5} 
                       & DDA                         & Predicate-based Write Skew                              & P                             & NP                         \\ \cline{2-5} 
\multirow{-7}{*}{IAT}  & MDA                         & Step IAT                                                & P                             & NP                         \\  \hline
                       
                       \bottomrule
\end{tabular}

==> tables/predicate_anomalies.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}

\begin{tabular}{c|l|c|l|c}
\toprule
\hline
\textbf{Types of   Anomalies} & \multicolumn{1}{c|}{\textbf{Edges   Combanations}} & \textbf{Anomalies}                   & \multicolumn{1}{c|}{\textbf{Partially   ordered combination with predicate}}      & \multicolumn{1}{c}{\textbf{Classification}} \\ \hline
SDA                           & $W-W-W[x]$                                         & Full-write                           & $W-W-W[x]$                                                                        & E*                                 \\ \hline
\multirow{2}{*}{SDA}          & \multirow{2}{*}{$W-W-R[x]$}                        & \multirow{2}{*}{Lost Self Update}    & $W_i[x]-W_j[x \in   Vset(P)]-R_i[x \in Vset(P)]$                                  & E*                                 \\ \cline{4-5} 
                              &                                                    &                                      & $W_i[x]-W_j[x \notin Vset(P)]-R_i[x \notin Vset(P)]$                              & P*                              \\ \hline
\multirow{3}{*}{SDA}          & \multirow{3}{*}{$W-R-W[x]$}                        & \multirow{3}{*}{Intermediate Read}   & $W_i[x \in   Vset(P)]-R_j[x \in Vset(P)]-W_i[x \in Vset(P)]$                      & E*                                 \\ \cline{4-5} 
                              &                                                    &                                      & $W_i[x \in Vset(P)]-R_j[x \in Vset(P)]-W_i[x \notin Vset(P)]$                     & P*                              \\ \cline{4-5} 
                              &                                                    &                                      & $W_i[x \notin Vset(P)]-R_j[x \notin Vset(P)]-W_i[x \in Vset(P)]$                  & P*                              \\ \hline
\multirow{3}{*}{SDA}          & \multirow{3}{*}{$R-W-W[x]$}                        & \multirow{3}{*}{Lost Update}         & $R_i[x \in   Vset(P)]-W_j[x \in Vset(P)]-W_i[x]$                                  & E*                                 \\ \cline{4-5} 
                              &                                                    &                                      & $R_i[x \in Vset(P)]-W_j[x \notin Vset(P)]-W_i[x]$                                 & P*                              \\ \cline{4-5} 
                              &                                                    &                                      & $R_i[x \notin Vset(P)]-W_j[x \in Vset(P)]-W_i[x]$                                 & P*                              \\ \hline
\multirow{3}{*}{SDA}          & \multirow{3}{*}{$R-W-R[x]$}                        & \multirow{3}{*}{Non-repeatable Read} & $R_i[x \in   Vset(P)]-W_j[x \in Vset(P)]-R_i[x \in Vset(P)]$                      & E*                                 \\ \cline{4-5} 
                              &                                                    &                                      & $R_i[x \notin Vset(P)]-W_j[x \in Vset(P)]-R_i[x \in Vset(P)]$                     & P*                              \\ \cline{4-5} 
                              &                                                    &                                      & $R_i[x \in Vset(P)]-W_j[x \notin Vset(P)]-R_i[x \notin Vset(P)]$                  & P*                              \\ \hline
DDA                           & $WW[x]-WW[y]$                                      & Full-write   Skew                    & $WW[x]-WW[y]$                                                                     & E*                                 \\ \hline
\multirow{2}{*}{DDA}          & \multirow{2}{*}{$WW[x]-WR[y]$}                     & \multirow{2}{*}{Double-write Skew 2} & $WW[x]-W[y \in   Vset(P)]R[y \in Vset(P)]$                                        & E*                                 \\ \cline{4-5} 
                              &                                                    &                                      & $WW[x]-W[y \notin Vset(P)]R[y \notin Vset(P)]$                                    & P*                              \\ \hline
\multirow{3}{*}{DDA}          & \multirow{3}{*}{$WW[x]-RW[y]$}                     & \multirow{3}{*}{Read-Write Skew 2}   & $WW[x]-R[y \in   Vset(P)]W[y \in Vset(P)]$                                        & E*                                 \\ \cline{4-5} 
                              &                                                    &                                      & $WW[x]-R[y \notin Vset(P)]W[y \in Vset(P)]$                                       & P*                              \\ \cline{4-5} 
                              &                                                    &                                      & $WW[x]-R[y \in Vset(P)]W[y \notin Vset(P)]$                                       & P*                              \\ \hline
\multirow{2}{*}{DDA}          & \multirow{2}{*}{$WR[x]-WW[y]$}                     & \multirow{2}{*}{Double-Write Skew 1} & $W[x \in Vset(P)]R[x   \in Vset(P)]-WW[y]$                                        & E*                                 \\ \cline{4-5} 
                              &                                                    &                                      & $W[x \notin Vset(P)]R[x \notin Vset(P)]-WW[y]$                                    & P*                              \\ \hline
\multirow{4}{*}{DDA}          & \multirow{4}{*}{$WR[x]-WR[y]$}                     & \multirow{4}{*}{Write-Read Skew}     & $W[x \in Vset(P)]R[x   \in Vset(P)]-W[y \in Vset(P)]R[y \in Vset(P)]$             & E*                                 \\ \cline{4-5} 
                              &                                                    &                                      & $W[x \in Vset(P)]R[x \in Vset(P)]-W[y \notin Vset(P)]R[y \notin   Vset(P)]$       & P*                              \\ \cline{4-5} 
                              &                                                    &                                      & $W[x \notin Vset(P)]R[x \notin Vset(P)]-W[y \in Vset(P)]R[y \in   Vset(P)]$       & P*                              \\ \cline{4-5} 
                              &                                                    &                                      & $W[x \notin Vset(P)]R[x \notin Vset(P)]-W[y \notin Vset(P)]R[y \notin   Vset(P)]$ & P*                              \\ \hline
\multirow{6}{*}{DDA}          & \multirow{6}{*}{$WR[x]-RW[y]$}                     & \multirow{6}{*}{Read Skew 2}         & $W[x \in Vset(P)]R[x   \in Vset(P)]-R[y \in Vset(P)]W[y \in Vset(P)]$             & E*                                 \\ \cline{4-5} 
                              &                                                    &                                      & $W[x \in Vset(P)]R[x \in Vset(P)]-R[y \in Vset(P)]W[y \notin Vset(P)]$            & P*                              \\ \cline{4-5} 
                              &                                                    &                                      & $W[x \in Vset(P)]R[x \in Vset(P)]-R[y \notin Vset(P)]W[y \in Vset(P)]$            & P*                              \\ \cline{4-5} 
                              &                                                    &                                      & $W[x \notin Vset(P)]R[x \notin Vset(P)]-R[y \in Vset(P)]W[y \in   Vset(P)]$       & P*                              \\ \cline{4-5} 
                              &                                                    &                                      & $W[x \notin Vset(P)]R[x \notin Vset(P)]-R[y \in Vset(P)]W[y \notin   Vset(P)]$    & P*                              \\ \cline{4-5} 
                              &                                                    &                                      & $W[x \notin Vset(P)]R[x \notin Vset(P)]-R[y \notin Vset(P)]W[y \in   Vset(P)]$    & P*                              \\ \hline
\multirow{3}{*}{DDA}          & \multirow{3}{*}{$RW[x]-WW[y]$}                     & \multirow{3}{*}{Read-Write Skew 1}   & $R[x \in Vset(P)]W[x   \in Vset(P)]-WW[y]$                                        & E*                                 \\ \cline{4-5} 
                              &                                                    &                                      & $R[x \in Vset(P)]W[x \notin Vset(P)]-WW[y]$                                       & P*                              \\ \cline{4-5} 
                              &                                                    &                                      & $R[x \notin Vset(P)]W[x \in Vset(P)]-WW[y]$                                       & P*                              \\ \hline
\multirow{6}{*}{DDA}          & \multirow{6}{*}{$RW[x]-WR[y]$}                     & \multirow{6}{*}{Read Skew}           & $R[x \in Vset(P)]W[x   \in Vset(P)]-W[y \in Vset(P)]R[y \in Vset(P)]$             & E*                                 \\ \cline{4-5} 
                              &                                                    &                                      & $R[x \in Vset(P)]W[x \notin Vset(P)]-W[y \in Vset(P)]R[y \in Vset(P)]$            & P*                              \\ \cline{4-5} 
                              &                                                    &                                      & $R[x \notin Vset(P)]W[x \in Vset(P)]-W[y \in Vset(P)]R[y \in Vset(P)]$            & P*                              \\ \cline{4-5} 
                              &                                                    &                                      & $R[x \in Vset(P)]W[x \in Vset(P)]-W[y \notin Vset(P)]R[y \notin   Vset(P)]$       & P*                              \\ \cline{4-5} 
                              &                                                    &                                      & $R[x \in Vset(P)]W[x \notin Vset(P)]-W[y \notin Vset(P)]R[y \notin   Vset(P)]$    & P*                              \\ \cline{4-5} 
                              &                                                    &                                      & $R[x \notin Vset(P)]W[x \in Vset(P)]-W[y \notin Vset(P)]R[y \notin   Vset(P)]$    & P*                              \\ \hline
\multirow{9}{*}{DDA}          & \multirow{9}{*}{$RW[x]-RW[y]$}                     & \multirow{9}{*}{Write Skew}          & $R[x \in Vset(P)]W[x   \in Vset(P)]-R[y \in Vset(P)]W[y \in Vset(P)]$             & E*                                 \\ \cline{4-5} 
                              &                                                    &                                      & $R[x \in Vset(P)]W[x \notin Vset(P)]-R[y \in Vset(P)]W[y \in Vset(P)]$            & P*                              \\ \cline{4-5} 
                              &                                                    &                                      & $R[x \notin Vset(P)]W[x \in Vset(P)]-R[y \in Vset(P)]W[y \in Vset(P)]$            & P*                              \\ \cline{4-5} 
                              &                                                    &                                      & $R[x \in Vset(P)]W[x \in Vset(P)]-R[y \notin Vset(P)]W[y \in Vset(P)]$            & P*                              \\ \cline{4-5} 
                              &                                                    &                                      & $R[x \in Vset(P)]W[x \notin Vset(P)]-R[y \notin Vset(P)]W[y \in   Vset(P)]$       & P*                              \\ \cline{4-5} 
                              &                                                    &                                      & $R[x \notin Vset(P)]W[x \in Vset(P)]-R[y \notin Vset(P)]W[y \in   Vset(P)]$       & P*                              \\ \cline{4-5} 
                              &                                                    &                                      & $R[x \in Vset(P)]W[x \in Vset(P)]-R[y \in Vset(P)]W[y \notin Vset(P)]$            & P*                              \\ \cline{4-5} 
                              &                                                    &                                      & $R[x \in Vset(P)]W[x \notin Vset(P)]-R[y \in Vset(P)]W[y \notin   Vset(P)]$       & P*                              \\ \cline{4-5} 
                              &                                                    &                                      & $R[x \notin Vset(P)]W[x \in Vset(P)]-R[y \in Vset(P)]W[y \notin   Vset(P)]$       & P*                              \\ \hline
                               \bottomrule
\end{tabular}


==> tables/summary4anomaly-New.tex <==
\setlength{\tabcolsep}{4pt}
\setlength\extrarowheight{1.2pt}

\begin{tabular}{|p{0.1in}|p{0.1in}|p{1.95in}|p{0.1in}|p{0.1in}  | > {\bfseries}p{0.1in} |p{0.1in}|p{0.1in}|> {\bfseries} p{0.1in} |p{0.1in}|p{0.1in}| > {\bfseries}p{0.1in} |p{0.1in}|p{0.1in}|> {\bfseries}p{0.1in}|p{0.1in}|> {\bfseries}p{0.1in}|p{0.1in}|p{0.1in}|p{0.1in}|> {\bfseries}p{0.1in}|p{0.1in}|p{0.1in}|p{0.1in}|}
\toprule\hline
 \rotatebox[origin=c]{270}{The primary classification} & \multicolumn{2}{c|}{\rotatebox[origin=c]{270}{\begin{tabular}[c]{@{}c@{}}The Data Anomaly\\ Name\end{tabular}}} & \rotatebox[origin=c]{270}{Test case} & \rotatebox[origin=c]{270}{MongoDB 4.4.4} &  \multicolumn{3}{c|}{ \rotatebox[origin=c]{270}{OceanBase 2.2.50}}       &       \normalfont{\rotatebox[origin=c]{270}{CockroachDB v19.2.2}} & \multicolumn{2}{c|}{\rotatebox[origin=c]{270}{TIDB 4.0.5}} & \multicolumn{3}{c|}{\rotatebox[origin=c]{270}{PostgreSQL 12.4}} & \multicolumn{2}{c|}{\rotatebox[origin=c]{270}{Oracle 12.1.0.2.0}} & \multicolumn{4}{c|}{\rotatebox[origin=c]{270}{SQL Server 15.0}} & \multicolumn{4}{c|}{\rotatebox[origin=c]{270}{MySQL 8.0.20}}   \\ \hline

 & \multicolumn{2}{c|}{}     & &  \rotatebox[origin=c]{270}{Snapshot} &      \rotatebox[origin=c]{270}{ \textbf{Serializable}}        &      \rotatebox[origin=c]{270}{Repeatable Read}       &     \rotatebox[origin=c]{270}{Read committed}    &      \rotatebox[origin=c]{270}{ \textbf{Serializable}}   &        \rotatebox[origin=c]{270}{Repeatable Read/SI}      &        \rotatebox[origin=c]{270}{Read committed}     &     \rotatebox[origin=c]{270}{ \textbf{Serializable}}    &     \rotatebox[origin=c]{270}{Repeatable Read}   &   \rotatebox[origin=c]{270}{Read committed}     &       \rotatebox[origin=c]{270}{ \textbf{Serializable}}     &       \rotatebox[origin=c]{270}{Read committed}    &    \rotatebox[origin=c]{270}{ \textbf{Serializable}}  &    \rotatebox[origin=c]{270}{Repeatable Read}  &    \rotatebox[origin=c]{270}{Read committed}  &    \rotatebox[origin=c]{270}{Read Uncommitted} &     \rotatebox[origin=c]{270}{ \textbf{Serializable}} &    \rotatebox[origin=c]{270}{Repeatable Read}  &   \rotatebox[origin=c]{270}{Read committed}   &   \rotatebox[origin=c]{270}{Read Uncommitted}        \\ \hline
 

 
   \multirow{28}{*}{\rotatebox[origin=c]{270}{RAT(Read Anomaly Type)}}    & \multicolumn{2}{c|}{Dirty Read (Aborted Reads) (W1R2-R2A1)} & 1  &  \cellcolor{red} C &      \cellcolor{red} C        &       \cellcolor{red} C      &      \cellcolor{red} C   &   \cellcolor{green} D      &         \cellcolor{red} C     &          \cellcolor{red} C   &     \cellcolor{red} C    &     \cellcolor{red} C   &      \cellcolor{red} C  &       \cellcolor{red} C     &      \cellcolor{red} C     &   \cellcolor{green} D   &    \cellcolor{green} D  &     \cellcolor{green} D &  \cellcolor{yellow} A   &  \cellcolor{green} D    &     \cellcolor{red} C &    \cellcolor{red} C  &   \cellcolor{yellow} A       \\ \cline{2-24}

 &   \multicolumn{2}{c|}{Non-repeatable Read(R1W2-W2R1)}&  2   &\cellcolor{red} C &      \cellcolor{red} C        &       \cellcolor{red} C      &      \cellcolor{red} C   &   \cellcolor{red} C      &         \cellcolor{red} C     &          \cellcolor{red} C   &     \cellcolor{red} C    &     \cellcolor{red} C   &      \cellcolor{red} C  &       \cellcolor{red} C     &      \cellcolor{red} C     &   \cellcolor{green} D   &    \cellcolor{green} D  &     \cellcolor{green} D &  \cellcolor{yellow} A   &  \cellcolor{green} D    &     \cellcolor{red} C &    \cellcolor{red} C  &   \cellcolor{yellow} A      \\ \cline{2-24}
  
 &  \multicolumn{2}{c|}{Intermediate Reads(W1R2-R2W1) } &  3    & \cellcolor{red} C &      \cellcolor{red} C        &       \cellcolor{red} C      &      \cellcolor{red} C   &   \cellcolor{green} D      &         \cellcolor{red} C     &          \cellcolor{red} C   &     \cellcolor{red} C    &     \cellcolor{red} C   &      \cellcolor{red} C  &       \cellcolor{red} C     &      \cellcolor{red} C     &   \cellcolor{green} D   &    \cellcolor{green} D  &     \cellcolor{green} D &  \cellcolor{yellow} A   &  \cellcolor{green} D    &     \cellcolor{red} C &    \cellcolor{red} C  &   \cellcolor{yellow} A      \\ \cline{2-24}
 &  \multicolumn{2}{c|}{Intermediate Reads Committed(W1R2-R2C2W1) } &  4    & \cellcolor{red} C &      \cellcolor{red} C        &       \cellcolor{red} C      &      \cellcolor{red} C   &   \cellcolor{green} D      &         \cellcolor{red} C     &          \cellcolor{red} C   &     \cellcolor{red} C    &     \cellcolor{red} C   &      \cellcolor{red} C  &       \cellcolor{red} C     &      \cellcolor{red} C     &   \cellcolor{green} D   &    \cellcolor{green} D  &     \cellcolor{green} D &  \cellcolor{yellow} A   &  \cellcolor{green} D    &     \cellcolor{red} C &    \cellcolor{red} C  &   \cellcolor{yellow} A      \\ \cline{2-24}
  
& \multicolumn{2}{c|}{Lost self update(W1W2-W2R1)} & 5 &    \cellcolor{green} D  &      \cellcolor{green} D        &       \cellcolor{green} D      &      \cellcolor{green} D   &   \cellcolor{green} D      &         \cellcolor{green} D     &          \cellcolor{green} D   &     \cellcolor{green} D    &     \cellcolor{green} D   &      \cellcolor{green} D  &       \cellcolor{green} D     &      \cellcolor{green} D     &   \cellcolor{green} D   &    \cellcolor{green} D  &     \cellcolor{green} D &  \cellcolor{green} D   &  \cellcolor{green} D    &     \cellcolor{green} D &    \cellcolor{green} D  &   \cellcolor{green} D        \\ \cline{2-24}
 
 &  \multicolumn{2}{c|}{Phantom (R1(p)W2-W2R1(p))} &   6    & \cellcolor{red} C &      \cellcolor{red} C        &       \cellcolor{red} C      &      \cellcolor{red} C   &   \cellcolor{red} C      &         \cellcolor{red} C     &          \cellcolor{red} C   &     \cellcolor{red} C    &     \cellcolor{red} C   &      \cellcolor{red} C  &       \cellcolor{red} C     &      \cellcolor{red} C     &   \cellcolor{green} D   &    \cellcolor{green} D  &     \cellcolor{green} D &  \cellcolor{yellow} A   &  \cellcolor{green} D    &     \cellcolor{red} C &    \cellcolor{red} C  &   \cellcolor{yellow} A     \\ \cline{2-24}
 
 & \multicolumn{2}{c|}{Write-read Skew(W1R2-W2R1)} & 7    &   \cellcolor{yellow} A &      \cellcolor{yellow} A        &       \cellcolor{yellow} A      &      \cellcolor{yellow} A   &   \cellcolor{green} D      &         \cellcolor{yellow} A     &          \cellcolor{yellow} A   &     \cellcolor{green} D    &     \cellcolor{yellow} A   &      \cellcolor{yellow} A  &       \cellcolor{yellow} A     &      \cellcolor{red} C     &   \cellcolor{green} D   &    \cellcolor{green} D  &     \cellcolor{green} D &  \cellcolor{yellow} A   &  \cellcolor{green} D    &     \cellcolor{yellow} A &    \cellcolor{yellow} A  &   \cellcolor{yellow} A      \\ \cline{2-24}

 & \multicolumn{2}{c|}{Write-read Skew Committed(W1R2-W2C2R1)} &    8    & \cellcolor{yellow} A &      \cellcolor{green} D        &       \cellcolor{yellow} A      &      \cellcolor{red} C   &   \cellcolor{green} D      &         \cellcolor{yellow} A     &          \cellcolor{red} C   &     \cellcolor{green} D    &     \cellcolor{yellow} A   &      \cellcolor{red} C  &       \cellcolor{yellow} A     &      \cellcolor{red} C     &   \cellcolor{green} D   &    \cellcolor{green} D  &     \cellcolor{green} D &  \cellcolor{yellow} A   &  \cellcolor{green} D    &     \cellcolor{red} C &    \cellcolor{red} C  &   \cellcolor{yellow} A      \\ \cline{2-24}

 &  \multicolumn{2}{c|}{Double-write Skew 1(W1R2-W2W1)  }  & 9 &  \cellcolor{green} D &      \cellcolor{green} D        &       \cellcolor{green} D      &      \cellcolor{green} D   &   \cellcolor{green} D      &         \cellcolor{green} D     &          \cellcolor{green} D   &     \cellcolor{green} D    &     \cellcolor{green} D   &      \cellcolor{green} D  &       \cellcolor{green} D     &      \cellcolor{green} D     &   \cellcolor{green} D   &    \cellcolor{green} D  &     \cellcolor{green} D &  \cellcolor{green} D   &  \cellcolor{green} D    &     \cellcolor{green} D &    \cellcolor{green} D  &   \cellcolor{green} D         \\ \cline{2-24}
   
 & \multicolumn{2}{c|}{Double-write skew 1 Committed (W1R2-W2C2W1)} & 10    &   \cellcolor{green} D &      \cellcolor{green} D        &       \cellcolor{green} D      &      \cellcolor{red} C   &   \cellcolor{green} D      &         \cellcolor{red} C     &          \cellcolor{red} C   &     \cellcolor{green} D    &     \cellcolor{green} D   &      \cellcolor{red} C  &       \cellcolor{green} D     &      \cellcolor{red} C     &   \cellcolor{green} D   &    \cellcolor{green} D  &     \cellcolor{green} D &  \cellcolor{yellow} A   &  \cellcolor{green} D    &     \cellcolor{red} C &    \cellcolor{red} C  &   \cellcolor{yellow} A      \\ \cline{2-24}

 &  \multicolumn{2}{c|}{Double-write Skew 2(W1W2-W2R1)  }  & 11 &  \cellcolor{green} D &      \cellcolor{green} D        &       \cellcolor{green} D      &      \cellcolor{green} D   &   \cellcolor{green} D      &         \cellcolor{green} D     &          \cellcolor{green} D   &     \cellcolor{green} D    &     \cellcolor{green} D   &      \cellcolor{green} D  &       \cellcolor{green} D     &      \cellcolor{green} D     &   \cellcolor{green} D   &    \cellcolor{green} D  &     \cellcolor{green} D &  \cellcolor{green} D   &  \cellcolor{green} D    &     \cellcolor{green} D &    \cellcolor{green} D  &   \cellcolor{green} D         \\ \cline{2-24}
 
 & \multirow{13}{*}{ \rotatebox[origin=c]{270}{Read skew}} & \multicolumn{1}{c|}{Read Skew1 (R1W2-W2R1)} & 12 &   \cellcolor{red} C &      \cellcolor{red} C        &       \cellcolor{red} C      &      \cellcolor{yellow} A   &   \cellcolor{red} C      &         \cellcolor{red} C     &          \cellcolor{yellow} A   &     \cellcolor{red} C    &     \cellcolor{red} C   &      \cellcolor{yellow} A  &       \cellcolor{red} C     &      \cellcolor{yellow} A     &   \cellcolor{green} D   &    \cellcolor{green} D  &     \cellcolor{yellow} A &  \cellcolor{yellow} A   &  \cellcolor{green} D    &     \cellcolor{red} C &    \cellcolor{yellow} A  &   \cellcolor{yellow} A        \\ \cline{3-24}
 
 & & \multicolumn{1}{c|}{Read Skew2(W1R2-R2W1)}  & 13    &   \cellcolor{red} C &      \cellcolor{red} C        &       \cellcolor{red} C      &      \cellcolor{red} C   &   \cellcolor{red} C      &         \cellcolor{red} C     &          \cellcolor{red} C   &     \cellcolor{red} C    &     \cellcolor{red} C   &      \cellcolor{red} C  &       \cellcolor{red} C     &      \cellcolor{red} C     &   \cellcolor{green} D   &    \cellcolor{green} D  &     \cellcolor{green} D &  \cellcolor{yellow} A   &  \cellcolor{green} D    &     \cellcolor{red} C &    \cellcolor{red} C  &   \cellcolor{yellow} A                        \\ \cline{3-24}

 &  & \multicolumn{1}{c|}{Read Skew3} & 14    &   \cellcolor{red} C &      \cellcolor{red} C        &       \cellcolor{red} C      &      \cellcolor{red} C   &   \cellcolor{green} D      &         \cellcolor{red} C     &          \cellcolor{red} C   &     \cellcolor{red} C    &     \cellcolor{red} C   &      \cellcolor{red} C  &       \cellcolor{red} C     &      \cellcolor{red} C     &   \cellcolor{green} D   &    \cellcolor{green} D  &     \cellcolor{green} D &  \cellcolor{yellow} A   &  \cellcolor{green} D    &     \cellcolor{red} C &    \cellcolor{red} C  &   \cellcolor{yellow} A                       \\ \cline{3-24}

 &  & \multicolumn{1}{c|}{Read Skew(Fractured Reads)} & 15    &   \cellcolor{red} C &      \cellcolor{red} C        &       \cellcolor{red} C      &      \cellcolor{yellow} A   &   \cellcolor{red} C      &         \cellcolor{red} C     &          \cellcolor{yellow} A   &     \cellcolor{red} C    &     \cellcolor{red} C   &      \cellcolor{yellow} A  &       \cellcolor{red} C     &      \cellcolor{yellow} A     &   \cellcolor{green} D   &    \cellcolor{green} D  &     \cellcolor{yellow} A &  \cellcolor{yellow} A   &  \cellcolor{green} D    &     \cellcolor{red} C &    \cellcolor{yellow} A  &   \cellcolor{yellow} A                        \\ \cline{3-24}
 
 &  & \multicolumn{1}{c|}{Read Skew(Causality Violation Anomaly)} & 16   &     \cellcolor{red} C &      \cellcolor{red} C        &       \cellcolor{red} C      &      \cellcolor{yellow} A   &   \cellcolor{red} C      &         \cellcolor{red} C     &          \cellcolor{yellow} A   &     \cellcolor{red} C    &     \cellcolor{red} C   &      \cellcolor{yellow} A  &       \cellcolor{red} C     &      \cellcolor{yellow} A     &   \cellcolor{green} D   &    \cellcolor{green} D  &     \cellcolor{yellow} A &  \cellcolor{yellow} A   &  \cellcolor{green} D    &     \cellcolor{red} C &    \cellcolor{yellow} A  &   \cellcolor{yellow} A                      \\ \cline{3-24}

 &    & \multicolumn{1}{c|}{Read Skew(Serial Concurrent Phenomenon)} & 17  & \cellcolor{red} C &      \cellcolor{red} C        &       \cellcolor{red} C      &      \cellcolor{yellow} A   &   \cellcolor{red} C      &         \cellcolor{red} C     &          \cellcolor{yellow} A   &     \cellcolor{red} C    &     \cellcolor{red} C   &      \cellcolor{yellow} A  &       \cellcolor{red} C     &      \cellcolor{yellow} A     &   \cellcolor{green} D   &    \cellcolor{green} D  &     \cellcolor{yellow} A &  \cellcolor{yellow} A   &  \cellcolor{green} D    &     \cellcolor{red} C &    \cellcolor{yellow} A  &   \cellcolor{yellow} A                         \\ \cline{3-24}

 &    & \multicolumn{1}{c|}{Read Skew(Cross Phenomenon)} & 18  &  \cellcolor{red} C &      \cellcolor{red} C        &       \cellcolor{red} C      &      \cellcolor{yellow} A   &   \cellcolor{red} C      &         \cellcolor{red} C     &          \cellcolor{yellow} A   &     \cellcolor{red} C    &     \cellcolor{red} C   &      \cellcolor{yellow} A  &       \cellcolor{red} C     &      \cellcolor{yellow} A     &   \cellcolor{green} D   &    \cellcolor{green} D  &     \cellcolor{yellow} A &  \cellcolor{yellow} A   &  \cellcolor{green} D    &     \cellcolor{red} C &    \cellcolor{yellow} A  &   \cellcolor{yellow} A                        \\ \cline{3-24}

 &      & \multicolumn{1}{c|}{Read Skew(Cross Phantom)} & 19 & \cellcolor{green} D &      \cellcolor{red} C        &       \cellcolor{red} C      &      \cellcolor{yellow} A   &   \cellcolor{red} C      &         \cellcolor{red} C     &          \cellcolor{yellow} A   &     \cellcolor{red} C    &     \cellcolor{red} C   &      \cellcolor{yellow} A  &       \cellcolor{red} C     &      \cellcolor{yellow} A     &   \cellcolor{green} D   &    \cellcolor{yellow} A  &     \cellcolor{yellow} A &  \cellcolor{yellow} A   &  \cellcolor{green} D    &     \cellcolor{red} C &    \cellcolor{yellow} A  &   \cellcolor{yellow} A                        \\ \cline{3-24}

 &     & \multicolumn{1}{c|}{Read Skew(Long Fork Anomaly)} & 20 & \cellcolor{red} C &      \cellcolor{red} C        &       \cellcolor{red} C      &      \cellcolor{red} C   &   \cellcolor{green} D      &         \cellcolor{red} C     &          \cellcolor{red} C   &     \cellcolor{red} C    &     \cellcolor{red} C   &      \cellcolor{red} C  &       \cellcolor{red} C     &      \cellcolor{red} C     &   \cellcolor{green} D   &    \cellcolor{green} D  &     \cellcolor{green} D &  \cellcolor{yellow} A   &  \cellcolor{green} D    &     \cellcolor{red} C &    \cellcolor{red} C  &   \cellcolor{yellow} A                        \\ \cline{3-24}

 &     & \multicolumn{1}{c|}{Read Skew(Half-Predicate-Based Read Skew)} & 21 &  \cellcolor{red} C &      \cellcolor{yellow} A        &       \cellcolor{yellow} A      &      \cellcolor{yellow} A   &   \cellcolor{red} C      &         \cellcolor{red} C     &          \cellcolor{yellow} A   &     \cellcolor{red} C    &     \cellcolor{red} C   &      \cellcolor{yellow} A  &       \cellcolor{red} C     &      \cellcolor{yellow} A     &   \cellcolor{green} D   &    \cellcolor{yellow} A  &     \cellcolor{yellow} A &  \cellcolor{yellow} A   &  \cellcolor{green} D    &     \cellcolor{red} C &    \cellcolor{yellow} A  &   \cellcolor{yellow} A                        \\ \cline{3-24}

 &      & \multicolumn{1}{c|}{Read Skew(Total-Same-Predicate-Based Read Skew)} & 22 & \cellcolor{green} D &      \cellcolor{red} C        &       \cellcolor{red} C      &      \cellcolor{yellow} A   &   \cellcolor{red} C      &         \cellcolor{red} C     &          \cellcolor{yellow} A   &     \cellcolor{red} C    &     \cellcolor{red} C   &      \cellcolor{yellow} A  &       \cellcolor{red} C     &      \cellcolor{yellow} A     &   \cellcolor{green} D   &    \cellcolor{yellow} A  &     \cellcolor{yellow} A &  \cellcolor{yellow} A   &  \cellcolor{green} D    &     \cellcolor{red} C &    \cellcolor{yellow} A  &   \cellcolor{yellow} A                         \\ \cline{3-24}

 &     & \multicolumn{1}{c|}{Read Skew(Total-Diff-Predicate-Based Read Skew)} & 23  &  \cellcolor{green} D &      \cellcolor{yellow} A        &       \cellcolor{yellow} A      &      \cellcolor{yellow} A   &   \cellcolor{red} C      &         \cellcolor{red} C     &          \cellcolor{yellow} A   &     \cellcolor{red} C    &     \cellcolor{red} C   &      \cellcolor{yellow} A  &       \cellcolor{red} C     &      \cellcolor{yellow} A     &   \cellcolor{green} D   &    \cellcolor{yellow} A  &     \cellcolor{yellow} A &  \cellcolor{yellow} A   &  \cellcolor{green} D    &     \cellcolor{red} C &    \cellcolor{yellow} A  &   \cellcolor{yellow} A                        \\ \cline{3-24}

 &     & \centering Read Skew~~~~~(Total-Same-Predicate-Based Read Skew2) & 24 &   \cellcolor{red} C &      \cellcolor{red} C        &       \cellcolor{red} C      &      \cellcolor{yellow} A   &   \cellcolor{red} C      &         \cellcolor{red} C     &          \cellcolor{yellow} A   &     \cellcolor{red} C    &     \cellcolor{red} C   &      \cellcolor{yellow} A  &       \cellcolor{red} C     &      \cellcolor{yellow} A     &   \cellcolor{green} D   &    \cellcolor{green} D  &     \cellcolor{yellow} A &  \cellcolor{yellow} A   &  \cellcolor{green} D    &     \cellcolor{red} C &    \cellcolor{yellow} A  &   \cellcolor{yellow} A                        \\ \cline{2-24}

 &  \multirow{4}{*}{\rotatebox[origin=c]{270}{Step RAT}}    & \multicolumn{1}{c|}{Step RAT (WR $\ge$3)}  & 25 & \cellcolor{red} C &      \cellcolor{red} C        &       \cellcolor{red} C      &      \cellcolor{yellow} A   &   \cellcolor{red} C      &         \cellcolor{red} C     &          \cellcolor{yellow} A   &     \cellcolor{red} C    &     \cellcolor{red} C   &      \cellcolor{yellow} A  &       \cellcolor{red} C     &      \cellcolor{yellow} A     &   \cellcolor{green} D   &    \cellcolor{green} D  &     \cellcolor{yellow} A &  \cellcolor{yellow} A   &  \cellcolor{green} D    &     \cellcolor{red} C &    \cellcolor{yellow} A  &   \cellcolor{yellow} A    \\ \cline{3-24}

 &     & \multicolumn{1}{c|}{Step RAT(UnnamedAnomaly)} & 26 & \cellcolor{red} C &      \cellcolor{red} C        &       \cellcolor{red} C      &      \cellcolor{yellow} A   &   \cellcolor{red} C      &         \cellcolor{red} C     &          \cellcolor{yellow} A   &     \cellcolor{red} C    &     \cellcolor{red} C   &      \cellcolor{yellow} A  &       \cellcolor{red} C     &      \cellcolor{yellow} A     &   \cellcolor{green} D   &    \cellcolor{green} D  &     \cellcolor{yellow} A &  \cellcolor{yellow} A   &  \cellcolor{green} D    &     \cellcolor{red} C &    \cellcolor{yellow} A  &   \cellcolor{yellow} A                         \\ \cline{3-24}

 &      & \multicolumn{1}{c|}{Step RAT(RAT-Special)} & 27 & \cellcolor{yellow} A &      \cellcolor{yellow} A        &       \cellcolor{yellow} A      &      \cellcolor{yellow} A   &   \cellcolor{green} D      &         \cellcolor{yellow} A     &          \cellcolor{yellow} A   &     \cellcolor{green} D    &     \cellcolor{yellow} A   &      \cellcolor{yellow} A  &       \cellcolor{green} D     &      \cellcolor{yellow} A     &   \cellcolor{green} D   &    \cellcolor{green} D  &     \cellcolor{yellow} A &  \cellcolor{yellow} A   &  \cellcolor{green} D    &     \cellcolor{yellow} A &    \cellcolor{yellow} A  &   \cellcolor{yellow} A                        \\ \cline{3-24}

 &  & \multicolumn{1}{c|}{Step RAT(RAT-Special2)} & 28    & \cellcolor{yellow} A &      \cellcolor{yellow} A        &       \cellcolor{yellow} A      &      \cellcolor{yellow} A   &   \cellcolor{green} D      &         \cellcolor{yellow} A     &          \cellcolor{yellow} A   &     \cellcolor{green} D    &     \cellcolor{yellow} A   &      \cellcolor{yellow} A  &       \cellcolor{green} D     &      \cellcolor{yellow} A     &   \cellcolor{green} D   &    \cellcolor{green} D  &     \cellcolor{yellow} A &  \cellcolor{yellow} A   &  \cellcolor{green} D    &     \cellcolor{yellow} A &    \cellcolor{yellow} A  &   \cellcolor{yellow} A                         \\ \hline



 \multirow{11}{*}{\rotatebox[origin=c]{270}{WAT(Write Anomaly Type)}}   & \multicolumn{2}{c|}{Dirty Write(W1W2-W2C1 W1W2-W2A1)}  & 29 & \cellcolor{green} D   &      \cellcolor{green} D        &       \cellcolor{green} D      &      \cellcolor{green} D   &   \cellcolor{green} D      &         \cellcolor{green} D     &          \cellcolor{green} D   &     \cellcolor{green} D    &     \cellcolor{green} D   &      \cellcolor{green} D  &       \cellcolor{green} D     &      \cellcolor{green} D     &   \cellcolor{green} D   &    \cellcolor{green} D  &     \cellcolor{green} D &  \cellcolor{green} D   &  \cellcolor{green} D    &     \cellcolor{green} D &    \cellcolor{green} D  &   \cellcolor{green} D           \\ \cline{2-24}
  
 & \multicolumn{2}{c|}{Full-write(W1W2-W2W1)} & 30  &   \cellcolor{green} D &      \cellcolor{green} D        &       \cellcolor{green} D      &      \cellcolor{green} D   &   \cellcolor{green} D      &         \cellcolor{green} D     &          \cellcolor{green} D   &     \cellcolor{green} D    &     \cellcolor{green} D   &      \cellcolor{green} D  &       \cellcolor{green} D     &      \cellcolor{green} D     &   \cellcolor{green} D   &    \cellcolor{green} D  &     \cellcolor{green} D &  \cellcolor{green} D   &  \cellcolor{green} D    &     \cellcolor{green} D &    \cellcolor{green} D  &   \cellcolor{green} D         \\ \cline{2-24}
 
 & \multicolumn{2}{c|}{Full-write Committed(W1W2-W2C2W1)} & 31  &   \cellcolor{green} D &      \cellcolor{green} D        &       \cellcolor{green} D      &      \cellcolor{green} D   &   \cellcolor{green} D      &         \cellcolor{green} D     &          \cellcolor{green} D   &     \cellcolor{green} D    &     \cellcolor{green} D   &      \cellcolor{green} D  &       \cellcolor{green} D     &      \cellcolor{green} D     &   \cellcolor{green} D   &    \cellcolor{green} D  &     \cellcolor{green} D &  \cellcolor{green} D   &  \cellcolor{green} D    &     \cellcolor{green} D &    \cellcolor{green} D  &   \cellcolor{green} D         \\ \cline{2-24}
 
 &  \multicolumn{2}{c|}{Lost Update(R1W2-W2W1)} & 32  &  \cellcolor{green} D &      \cellcolor{green} D        &       \cellcolor{green} D      &      \cellcolor{green} D   &   \cellcolor{green} D      &         \cellcolor{green} D     &          \cellcolor{green} D   &     \cellcolor{green} D    &     \cellcolor{green} D   &      \cellcolor{green} D  &       \cellcolor{green} D     &      \cellcolor{green} D     &   \cellcolor{green} D   &    \cellcolor{green} D  &     \cellcolor{green} D &  \cellcolor{green} D   &  \cellcolor{green} D    &     \cellcolor{green} D &    \cellcolor{green} D  &   \cellcolor{green} D          \\ \cline{2-24}
  
 & \multicolumn{2}{c|}{Lost Self Update Committed(W1W2-W2C2R1)} & 33  &   \cellcolor{green} D &      \cellcolor{green} D        &       \cellcolor{green} D      &      \cellcolor{green} D   &   \cellcolor{green} D      &         \cellcolor{green} D     &          \cellcolor{green} D   &     \cellcolor{green} D    &     \cellcolor{green} D   &      \cellcolor{green} D  &       \cellcolor{green} D     &      \cellcolor{green} D     &   \cellcolor{green} D   &    \cellcolor{green} D  &     \cellcolor{green} D &  \cellcolor{green} D   &  \cellcolor{green} D    &     \cellcolor{green} D &    \cellcolor{green} D  &   \cellcolor{green} D         \\ \cline{2-24}
   
  &  \multicolumn{2}{c|}{Double-write Skew 2 Committed(W1W2-W2C2R1)  }  & 34 &  \cellcolor{green} D &      \cellcolor{green} D        &       \cellcolor{green} D      &      \cellcolor{green} D   &   \cellcolor{green} D      &         \cellcolor{green} D     &          \cellcolor{green} D   &     \cellcolor{green} D    &     \cellcolor{green} D   &      \cellcolor{green} D  &       \cellcolor{green} D     &      \cellcolor{green} D     &   \cellcolor{green} D   &    \cellcolor{green} D  &     \cellcolor{green} D &  \cellcolor{green} D   &  \cellcolor{green} D    &     \cellcolor{green} D &    \cellcolor{green} D  &   \cellcolor{green} D         \\ \cline{2-24}
 
 & \multicolumn{2}{c|}{Full-write Skew(W1W2-W2W1)} & 35  &   \cellcolor{green} D &      \cellcolor{green} D        &       \cellcolor{green} D      &      \cellcolor{green} D   &   \cellcolor{green} D      &         \cellcolor{green} D     &          \cellcolor{green} D   &     \cellcolor{green} D    &     \cellcolor{green} D   &      \cellcolor{green} D  &       \cellcolor{green} D     &      \cellcolor{green} D     &   \cellcolor{green} D   &    \cellcolor{green} D  &     \cellcolor{green} D &  \cellcolor{green} D   &  \cellcolor{green} D    &     \cellcolor{green} D &    \cellcolor{green} D  &   \cellcolor{green} D         \\ \cline{2-24}
 
 & \multicolumn{2}{c|}{Full-write Skew Committed(W1W2-W2C2W1)} & 36 &   \cellcolor{green} D &      \cellcolor{green} D        &       \cellcolor{green} D      &      \cellcolor{green} D   &   \cellcolor{green} D      &         \cellcolor{green} D     &          \cellcolor{green} D   &     \cellcolor{green} D    &     \cellcolor{green} D   &      \cellcolor{green} D  &       \cellcolor{green} D     &      \cellcolor{green} D     &   \cellcolor{green} D   &    \cellcolor{green} D  &     \cellcolor{green} D &  \cellcolor{green} D   &  \cellcolor{green} D    &     \cellcolor{green} D &    \cellcolor{green} D  &   \cellcolor{green} D         \\ \cline{2-24}

  & \multicolumn{2}{c|}{Read-write Skew 1(R1W2-W2W1)} & 37  &  \cellcolor{green} D &      \cellcolor{green} D        &       \cellcolor{green} D      &      \cellcolor{green} D   &   \cellcolor{green} D      &         \cellcolor{green} D     &          \cellcolor{green} D   &     \cellcolor{green} D    &     \cellcolor{green} D   &      \cellcolor{green} D  &       \cellcolor{green} D     &      \cellcolor{green} D     &   \cellcolor{green} D   &    \cellcolor{green} D  &     \cellcolor{green} D &  \cellcolor{green} D   &  \cellcolor{green} D    &     \cellcolor{green} D &    \cellcolor{green} D  &   \cellcolor{green} D          \\ \cline{2-24}

  & \multicolumn{2}{c|}{Read-write Skew 2(W1W2-R2W1/R2C2W1)} & 38  &  \cellcolor{green} D &      \cellcolor{green} D        &       \cellcolor{green} D      &      \cellcolor{green} D   &   \cellcolor{green} D      &         \cellcolor{green} D     &          \cellcolor{green} D   &     \cellcolor{green} D    &     \cellcolor{green} D   &      \cellcolor{green} D  &       \cellcolor{green} D     &      \cellcolor{green} D     &   \cellcolor{green} D   &    \cellcolor{green} D  &     \cellcolor{green} D &  \cellcolor{green} D   &  \cellcolor{green} D    &     \cellcolor{green} D &    \cellcolor{green} D  &   \cellcolor{green} D          \\ \cline{2-24}  
 
 &  \multicolumn{2}{c|}{Step WAT(WW$\ge$3)} & 39 & \cellcolor{green} D      &     \cellcolor{green} D        &       \cellcolor{green} D      &      \cellcolor{green} D   &   \cellcolor{green} D      &         \cellcolor{green} D     &          \cellcolor{green} D   &     \cellcolor{green} D    &     \cellcolor{green} D   &      \cellcolor{green} D  &       \cellcolor{green} D     &      \cellcolor{green} D     &   \cellcolor{green} D   &    \cellcolor{green} D  &     \cellcolor{green} D &  \cellcolor{green} D   &  \cellcolor{green} D    &     \cellcolor{green} D &    \cellcolor{green} D  &   \cellcolor{green} D     \\ \hline
 


 \multirow{15}{*}{\rotatebox[origin=c]{270}{IAT(Interactive Anomaly Type)}}    & \multicolumn{2}{c|}{Lost Update Committed (R1W2-W2C2W)} & 40 &  \cellcolor{green} D &      \cellcolor{green} D        &       \cellcolor{green} D      &      \cellcolor{yellow} A   &   \cellcolor{green} D      &         \cellcolor{yellow} A     &          \cellcolor{yellow} A   &     \cellcolor{green} D    &     \cellcolor{green} D   &      \cellcolor{yellow} A  &       \cellcolor{green} D     &      \cellcolor{yellow} A     &   \cellcolor{green} D   &    \cellcolor{green} D  &     \cellcolor{yellow} A &  \cellcolor{yellow} A   &  \cellcolor{green} D    &     \cellcolor{yellow} A &    \cellcolor{yellow} A  &   \cellcolor{yellow} A      \\ \cline{2-24}

 & \multicolumn{2}{c|}{Non-repeatable Read Committed(R1W2-W2C2R1)} &  41    &    \cellcolor{red} C &      \cellcolor{red} C        &       \cellcolor{red} C      &      \cellcolor{yellow} A   &   \cellcolor{red} C      &         \cellcolor{red} C     &          \cellcolor{yellow} A   &     \cellcolor{red} C    &     \cellcolor{red} C   &      \cellcolor{yellow} A  &       \cellcolor{red} C     &      \cellcolor{yellow} A     &   \cellcolor{green} D   &    \cellcolor{green} D  &     \cellcolor{yellow} A &  \cellcolor{yellow} A   &  \cellcolor{green} D    &     \cellcolor{red} C &    \cellcolor{yellow} A  &   \cellcolor{yellow} A     \\ \cline{2-24}

 &   \multicolumn{2}{c|}{Read Skew Committed(R1W2-W2R1)}  & 42 & \cellcolor{red} C &      \cellcolor{red} C        &       \cellcolor{red} C      &      \cellcolor{yellow} A   &   \cellcolor{red} C      &         \cellcolor{red} C     &          \cellcolor{yellow} A   &     \cellcolor{red} C    &     \cellcolor{red} C   &      \cellcolor{yellow} A  &       \cellcolor{red} C     &      \cellcolor{yellow} A     &   \cellcolor{green} D   &    \cellcolor{green} D  &     \cellcolor{yellow} A &  \cellcolor{yellow} A   &  \cellcolor{green} D    &     \cellcolor{red} C &    \cellcolor{yellow} A  &   \cellcolor{yellow} A      \\ \cline{2-24}

 &  \multicolumn{2}{c|}{Read-write Skew 1 Committed(R1W2-W2C2W1)} &  43    &  \cellcolor{green} D &      \cellcolor{green} D        &       \cellcolor{green} D      &      \cellcolor{yellow} A   &   \cellcolor{green} D      &         \cellcolor{yellow} A     &          \cellcolor{yellow} A   &     \cellcolor{green} D    &     \cellcolor{green} D   &      \cellcolor{yellow} A  &       \cellcolor{green} D     &      \cellcolor{yellow} A     &   \cellcolor{green} D   &    \cellcolor{green} D  &     \cellcolor{yellow} A &  \cellcolor{yellow} A   &  \cellcolor{green} D    &     \cellcolor{yellow} A &    \cellcolor{yellow} A  &   \cellcolor{yellow} A      \\ \cline{2-24}

 & \multirow{8}{*}{\rotatebox[origin=c]{270}{Write skew}} &  \multicolumn{1}{c|}{Write Skew (R1W2-R2W1)}  & 44    &  \cellcolor{yellow} A &      \cellcolor{yellow} A        &       \cellcolor{yellow} A      &      \cellcolor{yellow} A   &   \cellcolor{green} D      &         \cellcolor{yellow} A     &          \cellcolor{yellow} A   &     \cellcolor{green} D    &     \cellcolor{yellow} A   &      \cellcolor{yellow} A  &       \cellcolor{green} D     &      \cellcolor{yellow} A     &   \cellcolor{green} D   &    \cellcolor{green} D  &     \cellcolor{yellow} A &  \cellcolor{yellow} A   &  \cellcolor{green} D    &     \cellcolor{yellow} A &    \cellcolor{yellow} A  &   \cellcolor{yellow} A     \\ \cline{3-24}

 & &  \multicolumn{1}{c|}{Write Skew(Black and White)} &  45    & \cellcolor{yellow} A &      \cellcolor{yellow} A        &       \cellcolor{yellow} A      &      \cellcolor{yellow} A   &   \cellcolor{green} D      &         \cellcolor{yellow} A     &          \cellcolor{yellow} A   &     \cellcolor{green} D    &     \cellcolor{yellow} A   &      \cellcolor{yellow} A  &       \cellcolor{yellow} A     &      \cellcolor{yellow} A     &   \cellcolor{green} D   &    \cellcolor{green} D  &     \cellcolor{green} D &  \cellcolor{green} D   &  \cellcolor{green} D    &     \cellcolor{green} D &    \cellcolor{yellow} A  &   \cellcolor{yellow} A                        \\ \cline{3-24}

 &    & \multicolumn{1}{c|}{Write Skew(Intersecting Data)} & 46  &   \cellcolor{yellow} A &      \cellcolor{yellow} A        &       \cellcolor{yellow} A      &      \cellcolor{yellow} A   &   \cellcolor{green} D      &         \cellcolor{yellow} A     &          \cellcolor{yellow} A   &     \cellcolor{green} D    &     \cellcolor{yellow} A   &      \cellcolor{yellow} A  &       \cellcolor{green} D     &      \cellcolor{yellow} A     &   \cellcolor{green} D   &    \cellcolor{green} D  &     \cellcolor{green} D &  \cellcolor{red} C   &  \cellcolor{green} D    &     \cellcolor{yellow} A &    \cellcolor{yellow} A  &   \cellcolor{yellow} A                        \\ \cline{3-24}

 &   & \multicolumn{1}{c|}{Write Skew(Overdraft Protection)} & 47    &  \cellcolor{yellow} A &      \cellcolor{yellow} A        &       \cellcolor{yellow} A      &      \cellcolor{yellow} A   &   \cellcolor{green} D      &         \cellcolor{yellow} A     &          \cellcolor{yellow} A   &     \cellcolor{green} D    &     \cellcolor{yellow} A   &      \cellcolor{yellow} A  &       \cellcolor{green} D     &      \cellcolor{yellow} A     &   \cellcolor{green} D   &    \cellcolor{green} D  &     \cellcolor{yellow} A &  \cellcolor{yellow} A   &  \cellcolor{green} D    &     \cellcolor{yellow} A &    \cellcolor{yellow} A  &   \cellcolor{yellow} A                        \\ \cline{3-24}

 &     & \multicolumn{1}{c|}{Half-predicate-based Write Skew} & 48  & \cellcolor{yellow} A &      \cellcolor{yellow} A        &       \cellcolor{yellow} A      &      \cellcolor{yellow} A   &   \cellcolor{green} D      &         \cellcolor{yellow} A     &          \cellcolor{yellow} A   &     \cellcolor{green} D    &     \cellcolor{yellow} A   &      \cellcolor{yellow} A  &       \cellcolor{green} D     &      \cellcolor{yellow} A     &   \cellcolor{green} D   &    \cellcolor{green} D  &     \cellcolor{yellow} A &  \cellcolor{yellow} A   &  \cellcolor{green} D    &     \cellcolor{yellow} A &    \cellcolor{yellow} A  &   \cellcolor{yellow} A                        \\ \cline{3-24}

 &  & \multicolumn{1}{c|}{Total-same-predicate-based Write Skew} & 49   &   \cellcolor{yellow} A &      \cellcolor{yellow} A        &       \cellcolor{yellow} A      &      \cellcolor{yellow} A   &   \cellcolor{green} D      &         \cellcolor{yellow} A     &          \cellcolor{yellow} A   &     \cellcolor{green} D    &     \cellcolor{yellow} A   &      \cellcolor{yellow} A  &       \cellcolor{yellow} A     &      \cellcolor{yellow} A     &   \cellcolor{green} D   &    \cellcolor{yellow} A  &     \cellcolor{yellow} A &  \cellcolor{yellow} A   &  \cellcolor{green} D    &     \cellcolor{yellow} A &    \cellcolor{yellow} A  &   \cellcolor{yellow} A                        \\ \cline{3-24} 

 &  & \multicolumn{1}{c|}{Total-diff-predicate-based Write Skew} & 50    &   \cellcolor{yellow} A &      \cellcolor{yellow} A        &       \cellcolor{yellow} A      &      \cellcolor{yellow} A   &   \cellcolor{green} D      &         \cellcolor{yellow} A     &          \cellcolor{yellow} A   &     \cellcolor{green} D    &     \cellcolor{yellow} A   &      \cellcolor{yellow} A  &       \cellcolor{yellow} A     &      \cellcolor{yellow} A     &   \cellcolor{green} D   &    \cellcolor{yellow} A  &     \cellcolor{yellow} A &  \cellcolor{yellow} A   &  \cellcolor{green} D    &     \cellcolor{yellow} A &    \cellcolor{yellow} A  &   \cellcolor{yellow} A                        \\ \cline{3-24}

 &  & \multicolumn{1}{c|}{Write Skew(Read-only Transaction Anomaly)} & 51   &   \cellcolor{yellow} A &      \cellcolor{yellow} A        &       \cellcolor{yellow} A      &      \cellcolor{yellow} A   &   \cellcolor{green} D      &         \cellcolor{yellow} A     &          \cellcolor{yellow} A   &     \cellcolor{green} D    &     \cellcolor{yellow} A   &      \cellcolor{yellow} A  &       \cellcolor{green} D     &      \cellcolor{yellow} A     &   \cellcolor{green} D   &    \cellcolor{green} D  &     \cellcolor{yellow} A &  \cellcolor{yellow} A   &  \cellcolor{green} D    &     \cellcolor{yellow} A &    \cellcolor{yellow} A  &   \cellcolor{yellow} A                       \\ \cline{2-24}

 &   \multirow{3}{*}{\rotatebox[origin=c]{270}{Step IAT}}   & \multicolumn{1}{c|}{Step IAT(Primary Colors) (other$\ge$3)} & 52 &  \cellcolor{yellow} A &      \cellcolor{yellow} A        &       \cellcolor{yellow} A      &      \cellcolor{yellow} A   &   \cellcolor{green} D      &         \cellcolor{yellow} A     &          \cellcolor{yellow} A   &     \cellcolor{green} D    &     \cellcolor{yellow} A   &      \cellcolor{yellow} A  &       \cellcolor{yellow} A     &      \cellcolor{yellow} A     &   \cellcolor{green} D   &    \cellcolor{green} D  &     \cellcolor{green} D &  \cellcolor{green} D   &  \cellcolor{green} D    &     \cellcolor{green} D &    \cellcolor{yellow} A  &   \cellcolor{yellow} A      \\ \cline{3-24}

 &  & \multicolumn{1}{c|}{Step IAT(Sawtooth)} & 53   &   \cellcolor{yellow} A &      \cellcolor{yellow} A        &       \cellcolor{yellow} A      &      \cellcolor{yellow} A   &   \cellcolor{green} D      &         \cellcolor{yellow} A     &          \cellcolor{yellow} A   &     \cellcolor{green} D    &     \cellcolor{yellow} A   &      \cellcolor{yellow} A  &       \cellcolor{green} D     &      \cellcolor{yellow} A     &   \cellcolor{green} D   &    \cellcolor{green} D  &     \cellcolor{yellow} A &  \cellcolor{yellow} A   &  \cellcolor{green} D    &     \cellcolor{yellow} A &    \cellcolor{yellow} A  &   \cellcolor{yellow} A                        \\ \cline{3-24}

 &  & \multicolumn{1}{c|}{Step IAT(Predicate-based Sawtooth)} & 54   &   \cellcolor{yellow} A &      \cellcolor{yellow} A        &       \cellcolor{yellow} A      &      \cellcolor{yellow} A   &   \cellcolor{green} D      &         \cellcolor{yellow} A     &          \cellcolor{yellow} A   &     \cellcolor{green} D    &     \cellcolor{yellow} A   &      \cellcolor{yellow} A  &       \cellcolor{yellow} A     &      \cellcolor{yellow} A     &   \cellcolor{green} D   &    \cellcolor{yellow} A  &     \cellcolor{yellow} A &  \cellcolor{yellow} A   &  \cellcolor{green} D    &     \cellcolor{yellow} A &    \cellcolor{yellow} A  &   \cellcolor{yellow} A                        \\ \hline
\bottomrule
\end{tabular}


==> tables/summary4anomaly.tex <==
\setlength{\tabcolsep}{4pt}
\setlength\extrarowheight{1.2pt}

\begin{tabular}{|p{0.1in}|p{0.1in}|p{1.95in}|p{0.1in}|p{0.1in}  | > {\bfseries}p{0.1in} |p{0.1in}|p{0.1in}|> {\bfseries} p{0.1in} |p{0.1in}|p{0.1in}| > {\bfseries}p{0.1in} |p{0.1in}|p{0.1in}|> {\bfseries}p{0.1in}|p{0.1in}|> {\bfseries}p{0.1in}|p{0.1in}|p{0.1in}|p{0.1in}|> {\bfseries}p{0.1in}|p{0.1in}|p{0.1in}|p{0.1in}|}
\toprule\hline
 \rotatebox[origin=c]{270}{The primary classification} & \multicolumn{2}{c|}{\rotatebox[origin=c]{270}{\begin{tabular}[c]{@{}c@{}}The Data Anomaly\\ Name\end{tabular}}} & \rotatebox[origin=c]{270}{Test case} & \rotatebox[origin=c]{270}{MongoDB 4.4.4} &  \multicolumn{3}{c|}{ \rotatebox[origin=c]{270}{OceanBase 2.2.50}}       &       \normalfont{\rotatebox[origin=c]{270}{CockroachDB v19.2.2}} & \multicolumn{2}{c|}{\rotatebox[origin=c]{270}{TIDB 4.0.5}} & \multicolumn{3}{c|}{\rotatebox[origin=c]{270}{PostgreSQL 12.4}} & \multicolumn{2}{c|}{\rotatebox[origin=c]{270}{Oracle 12.1.0.2.0}} & \multicolumn{4}{c|}{\rotatebox[origin=c]{270}{SQL Server 15.0}} & \multicolumn{4}{c|}{\rotatebox[origin=c]{270}{MySQL 8.0.20}}   \\ \hline

 & \multicolumn{2}{c|}{}     & &  \rotatebox[origin=c]{270}{Snapshot} &      \rotatebox[origin=c]{270}{ \textbf{Serializable}}        &      \rotatebox[origin=c]{270}{Repeatable Read}       &     \rotatebox[origin=c]{270}{Read committed}    &      \rotatebox[origin=c]{270}{ \textbf{Serializable}}   &        \rotatebox[origin=c]{270}{Repeatable Read/SI}      &        \rotatebox[origin=c]{270}{Read committed}     &     \rotatebox[origin=c]{270}{ \textbf{Serializable}}    &     \rotatebox[origin=c]{270}{Repeatable Read}   &   \rotatebox[origin=c]{270}{Read committed}     &       \rotatebox[origin=c]{270}{ \textbf{Serializable}}     &       \rotatebox[origin=c]{270}{Read committed}    &    \rotatebox[origin=c]{270}{ \textbf{Serializable}}  &    \rotatebox[origin=c]{270}{Repeatable Read}  &    \rotatebox[origin=c]{270}{Read committed}  &    \rotatebox[origin=c]{270}{Read Uncommitted} &     \rotatebox[origin=c]{270}{ \textbf{Serializable}} &    \rotatebox[origin=c]{270}{Repeatable Read}  &   \rotatebox[origin=c]{270}{Read committed}   &   \rotatebox[origin=c]{270}{Read Uncommitted}        \\ \hline
 
 \multirow{13}{*}{\rotatebox[origin=c]{270}{WAT(Write Anomaly Type)}}  & \multicolumn{2}{c|}{Phantom Write (W1W2-W2R1)} & 1 &    \cellcolor{green} D  &      \cellcolor{green} D        &       \cellcolor{green} D      &      \cellcolor{green} D   &   \cellcolor{green} D      &         \cellcolor{green} D     &          \cellcolor{green} D   &     \cellcolor{green} D    &     \cellcolor{green} D   &      \cellcolor{green} D  &       \cellcolor{green} D     &      \cellcolor{green} D     &   \cellcolor{green} D   &    \cellcolor{green} D  &     \cellcolor{green} D &  \cellcolor{green} D   &  \cellcolor{green} D    &     \cellcolor{green} D &    \cellcolor{green} D  &   \cellcolor{green} D        \\ \cline{2-24}
 
 & \multicolumn{2}{c|}{Dirty Write (W1W2-W2C1 W1W2-W2A1)}  & 2 & \cellcolor{green} D   &      \cellcolor{green} D        &       \cellcolor{green} D      &      \cellcolor{green} D   &   \cellcolor{green} D      &         \cellcolor{green} D     &          \cellcolor{green} D   &     \cellcolor{green} D    &     \cellcolor{green} D   &      \cellcolor{green} D  &       \cellcolor{green} D     &      \cellcolor{green} D     &   \cellcolor{green} D   &    \cellcolor{green} D  &     \cellcolor{green} D &  \cellcolor{green} D   &  \cellcolor{green} D    &     \cellcolor{green} D &    \cellcolor{green} D  &   \cellcolor{green} D           \\ \cline{2-24}
 
 &\multicolumn{2}{c|}{Intermediate Write (W1W2-W2W1 W1W2-W2C2W1 )}  & 3 &  \cellcolor{green} D &      \cellcolor{green} D        &       \cellcolor{green} D      &      \cellcolor{green} D   &   \cellcolor{green} D      &         \cellcolor{green} D     &          \cellcolor{green} D   &     \cellcolor{green} D    &     \cellcolor{green} D   &      \cellcolor{green} D  &       \cellcolor{green} D     &      \cellcolor{green} D     &   \cellcolor{green} D   &    \cellcolor{green} D  &     \cellcolor{green} D &  \cellcolor{green} D   &  \cellcolor{green} D    &     \cellcolor{green} D &    \cellcolor{green} D  &   \cellcolor{green} D          \\ \cline{2-24}
 
 & \multicolumn{2}{c|}{Full-Write (W1W2-W2W1)} & 4  &   \cellcolor{green} D &      \cellcolor{green} D        &       \cellcolor{green} D      &      \cellcolor{green} D   &   \cellcolor{green} D      &         \cellcolor{green} D     &          \cellcolor{green} D   &     \cellcolor{green} D    &     \cellcolor{green} D   &      \cellcolor{green} D  &       \cellcolor{green} D     &      \cellcolor{green} D     &   \cellcolor{green} D   &    \cellcolor{green} D  &     \cellcolor{green} D &  \cellcolor{green} D   &  \cellcolor{green} D    &     \cellcolor{green} D &    \cellcolor{green} D  &   \cellcolor{green} D         \\ \cline{2-24}
 
 & \multicolumn{2}{c|}{Full-Write Committed(W1W2-W2C2W1)} & 5  &   \cellcolor{green} D &      \cellcolor{green} D        &       \cellcolor{green} D      &      \cellcolor{green} D   &   \cellcolor{green} D      &         \cellcolor{green} D     &          \cellcolor{green} D   &     \cellcolor{green} D    &     \cellcolor{green} D   &      \cellcolor{green} D  &       \cellcolor{green} D     &      \cellcolor{green} D     &   \cellcolor{green} D   &    \cellcolor{green} D  &     \cellcolor{green} D &  \cellcolor{green} D   &  \cellcolor{green} D    &     \cellcolor{green} D &    \cellcolor{green} D  &   \cellcolor{green} D         \\ \cline{2-24}
 
 & \multicolumn{2}{c|}{Lost Self Update (W1W2-W2R1 W1W2-W2C2R1)} & 6  &   \cellcolor{green} D &      \cellcolor{green} D        &       \cellcolor{green} D      &      \cellcolor{green} D   &   \cellcolor{green} D      &         \cellcolor{green} D     &          \cellcolor{green} D   &     \cellcolor{green} D    &     \cellcolor{green} D   &      \cellcolor{green} D  &       \cellcolor{green} D     &      \cellcolor{green} D     &   \cellcolor{green} D   &    \cellcolor{green} D  &     \cellcolor{green} D &  \cellcolor{green} D   &  \cellcolor{green} D    &     \cellcolor{green} D &    \cellcolor{green} D  &   \cellcolor{green} D         \\ \cline{2-24}
 
 &  \multicolumn{2}{c|}{Lost Update (R1W2-W2W1)} & 7  &  \cellcolor{green} D &      \cellcolor{green} D        &       \cellcolor{green} D      &      \cellcolor{green} D   &   \cellcolor{green} D      &         \cellcolor{green} D     &          \cellcolor{green} D   &     \cellcolor{green} D    &     \cellcolor{green} D   &      \cellcolor{green} D  &       \cellcolor{green} D     &      \cellcolor{green} D     &   \cellcolor{green} D   &    \cellcolor{green} D  &     \cellcolor{green} D &  \cellcolor{green} D   &  \cellcolor{green} D    &     \cellcolor{green} D &    \cellcolor{green} D  &   \cellcolor{green} D          \\ \cline{2-24}
 
 &  \multicolumn{2}{c|}{Double-Write Skew 1(W1R2-W2W1 W1W2-W2R1)  }  & 8 &  \cellcolor{green} D &      \cellcolor{green} D        &       \cellcolor{green} D      &      \cellcolor{green} D   &   \cellcolor{green} D      &         \cellcolor{green} D     &          \cellcolor{green} D   &     \cellcolor{green} D    &     \cellcolor{green} D   &      \cellcolor{green} D  &       \cellcolor{green} D     &      \cellcolor{green} D     &   \cellcolor{green} D   &    \cellcolor{green} D  &     \cellcolor{green} D &  \cellcolor{green} D   &  \cellcolor{green} D    &     \cellcolor{green} D &    \cellcolor{green} D  &   \cellcolor{green} D         \\ \cline{2-24}
 
  &  \multicolumn{2}{c|}{Double-Write Skew 1 Committed(W1W2-W2C2R1)  }  & 9 &  \cellcolor{green} D &      \cellcolor{green} D        &       \cellcolor{green} D      &      \cellcolor{green} D   &   \cellcolor{green} D      &         \cellcolor{green} D     &          \cellcolor{green} D   &     \cellcolor{green} D    &     \cellcolor{green} D   &      \cellcolor{green} D  &       \cellcolor{green} D     &      \cellcolor{green} D     &   \cellcolor{green} D   &    \cellcolor{green} D  &     \cellcolor{green} D &  \cellcolor{green} D   &  \cellcolor{green} D    &     \cellcolor{green} D &    \cellcolor{green} D  &   \cellcolor{green} D         \\ \cline{2-24}
 
 & \multicolumn{2}{c|}{Read-Write Skew 1$/$2 (R1W2-W2W1 W1W2-R2W1)} & 10  &  \cellcolor{green} D &      \cellcolor{green} D        &       \cellcolor{green} D      &      \cellcolor{green} D   &   \cellcolor{green} D      &         \cellcolor{green} D     &          \cellcolor{green} D   &     \cellcolor{green} D    &     \cellcolor{green} D   &      \cellcolor{green} D  &       \cellcolor{green} D     &      \cellcolor{green} D     &   \cellcolor{green} D   &    \cellcolor{green} D  &     \cellcolor{green} D &  \cellcolor{green} D   &  \cellcolor{green} D    &     \cellcolor{green} D &    \cellcolor{green} D  &   \cellcolor{green} D          \\ \cline{2-24}
 
 & \multicolumn{2}{c|}{Full-Write Skew(W1W2-W2W1)} & 11  &   \cellcolor{green} D &      \cellcolor{green} D        &       \cellcolor{green} D      &      \cellcolor{green} D   &   \cellcolor{green} D      &         \cellcolor{green} D     &          \cellcolor{green} D   &     \cellcolor{green} D    &     \cellcolor{green} D   &      \cellcolor{green} D  &       \cellcolor{green} D     &      \cellcolor{green} D     &   \cellcolor{green} D   &    \cellcolor{green} D  &     \cellcolor{green} D &  \cellcolor{green} D   &  \cellcolor{green} D    &     \cellcolor{green} D &    \cellcolor{green} D  &   \cellcolor{green} D         \\ \cline{2-24}
 
 & \multicolumn{2}{c|}{Full-Write Skew Committed(W1W2-W2C2W1)} & 12  &   \cellcolor{green} D &      \cellcolor{green} D        &       \cellcolor{green} D      &      \cellcolor{green} D   &   \cellcolor{green} D      &         \cellcolor{green} D     &          \cellcolor{green} D   &     \cellcolor{green} D    &     \cellcolor{green} D   &      \cellcolor{green} D  &       \cellcolor{green} D     &      \cellcolor{green} D     &   \cellcolor{green} D   &    \cellcolor{green} D  &     \cellcolor{green} D &  \cellcolor{green} D   &  \cellcolor{green} D    &     \cellcolor{green} D &    \cellcolor{green} D  &   \cellcolor{green} D         \\ \cline{2-24}
 
 &  \multicolumn{2}{c|}{Step WAT(WW$\ge$3)} & 13 & \cellcolor{green} D      &     \cellcolor{green} D        &       \cellcolor{green} D      &      \cellcolor{green} D   &   \cellcolor{green} D      &         \cellcolor{green} D     &          \cellcolor{green} D   &     \cellcolor{green} D    &     \cellcolor{green} D   &      \cellcolor{green} D  &       \cellcolor{green} D     &      \cellcolor{green} D     &   \cellcolor{green} D   &    \cellcolor{green} D  &     \cellcolor{green} D &  \cellcolor{green} D   &  \cellcolor{green} D    &     \cellcolor{green} D &    \cellcolor{green} D  &   \cellcolor{green} D     \\ \hline
 
  \multirow{24}{*}{\rotatebox[origin=c]{270}{RAT(Read Anomaly Type)}}    & \multicolumn{2}{c|}{Dirty Read (Aborted Reads) (W1R2-R2A1)} & 14  &  \cellcolor{red} C &      \cellcolor{red} C        &       \cellcolor{red} C      &      \cellcolor{red} C   &   \cellcolor{green} D      &         \cellcolor{red} C     &          \cellcolor{red} C   &     \cellcolor{red} C    &     \cellcolor{red} C   &      \cellcolor{red} C  &       \cellcolor{red} C     &      \cellcolor{red} C     &   \cellcolor{green} D   &    \cellcolor{green} D  &     \cellcolor{green} D &  \cellcolor{yellow} A   &  \cellcolor{green} D    &     \cellcolor{red} C &    \cellcolor{red} C  &   \cellcolor{yellow} A       \\ \cline{2-24}
 
 &  \multicolumn{2}{c|}{Intermediate Reads (W1R2-R2C2W1) } &  15    & \cellcolor{red} C &      \cellcolor{red} C        &       \cellcolor{red} C      &      \cellcolor{red} C   &   \cellcolor{green} D      &         \cellcolor{red} C     &          \cellcolor{red} C   &     \cellcolor{red} C    &     \cellcolor{red} C   &      \cellcolor{red} C  &       \cellcolor{red} C     &      \cellcolor{red} C     &   \cellcolor{green} D   &    \cellcolor{green} D  &     \cellcolor{green} D &  \cellcolor{yellow} A   &  \cellcolor{green} D    &     \cellcolor{red} C &    \cellcolor{red} C  &   \cellcolor{yellow} A      \\ \cline{2-24}
 
 &   \multicolumn{2}{c|}{Fuzzy$/$Non-Repeatable Read (R1W2-W2R1)}&  16    &\cellcolor{red} C &      \cellcolor{red} C        &       \cellcolor{red} C      &      \cellcolor{red} C   &   \cellcolor{red} C      &         \cellcolor{red} C     &          \cellcolor{red} C   &     \cellcolor{red} C    &     \cellcolor{red} C   &      \cellcolor{red} C  &       \cellcolor{red} C     &      \cellcolor{red} C     &   \cellcolor{green} D   &    \cellcolor{green} D  &     \cellcolor{green} D &  \cellcolor{yellow} A   &  \cellcolor{green} D    &     \cellcolor{red} C &    \cellcolor{red} C  &   \cellcolor{yellow} A      \\ \cline{2-24}
 
 &  \multicolumn{2}{c|}{Phantom (R1(p)W2-W2R1(p))} &   17    & \cellcolor{red} C &      \cellcolor{red} C        &       \cellcolor{red} C      &      \cellcolor{red} C   &   \cellcolor{red} C      &         \cellcolor{red} C     &          \cellcolor{red} C   &     \cellcolor{red} C    &     \cellcolor{red} C   &      \cellcolor{red} C  &       \cellcolor{red} C     &      \cellcolor{red} C     &   \cellcolor{green} D   &    \cellcolor{green} D  &     \cellcolor{green} D &  \cellcolor{yellow} A   &  \cellcolor{green} D    &     \cellcolor{red} C &    \cellcolor{red} C  &   \cellcolor{yellow} A     \\ \cline{2-24}
 
 & \multicolumn{2}{c|}{Write-Read Skew Committed (W1R2-W2C2R1)} &    18    & \cellcolor{yellow} A &      \cellcolor{green} D        &       \cellcolor{yellow} A      &      \cellcolor{red} C   &   \cellcolor{green} D      &         \cellcolor{yellow} A     &          \cellcolor{red} C   &     \cellcolor{green} D    &     \cellcolor{yellow} A   &      \cellcolor{red} C  &       \cellcolor{yellow} A     &      \cellcolor{red} C     &   \cellcolor{green} D   &    \cellcolor{green} D  &     \cellcolor{green} D &  \cellcolor{yellow} A   &  \cellcolor{green} D    &     \cellcolor{red} C &    \cellcolor{red} C  &   \cellcolor{yellow} A      \\ \cline{2-24}
 
 & \multicolumn{2}{c|}{Write-Read Skew (W1R2-W2R1)} & 19    &   \cellcolor{yellow} A &      \cellcolor{yellow} A        &       \cellcolor{yellow} A      &      \cellcolor{yellow} A   &   \cellcolor{green} D      &         \cellcolor{yellow} A     &          \cellcolor{yellow} A   &     \cellcolor{green} D    &     \cellcolor{yellow} A   &      \cellcolor{yellow} A  &       \cellcolor{yellow} A     &      \cellcolor{red} C     &   \cellcolor{green} D   &    \cellcolor{green} D  &     \cellcolor{green} D &  \cellcolor{yellow} A   &  \cellcolor{green} D    &     \cellcolor{yellow} A &    \cellcolor{yellow} A  &   \cellcolor{yellow} A      \\ \cline{2-24}
  
 & \multicolumn{2}{c|}{Double write skew 1 Committed (W1R2-W2C2W1)} & 20    &   \cellcolor{green} D &      \cellcolor{green} D        &       \cellcolor{green} D      &      \cellcolor{red} C   &   \cellcolor{green} D      &         \cellcolor{red} C     &          \cellcolor{red} C   &     \cellcolor{green} D    &     \cellcolor{green} D   &      \cellcolor{red} C  &       \cellcolor{green} D     &      \cellcolor{red} C     &   \cellcolor{green} D   &    \cellcolor{green} D  &     \cellcolor{green} D &  \cellcolor{yellow} A   &  \cellcolor{green} D    &     \cellcolor{red} C &    \cellcolor{red} C  &   \cellcolor{yellow} A      \\ \cline{2-24}
 
 & \multirow{13}{*}{ \rotatebox[origin=c]{270}{Read skew}} & \multicolumn{1}{c|}{Read Skew1 (R1W2-W2R1)} & 21 &   \cellcolor{red} C &      \cellcolor{red} C        &       \cellcolor{red} C      &      \cellcolor{yellow} A   &   \cellcolor{red} C      &         \cellcolor{red} C     &          \cellcolor{yellow} A   &     \cellcolor{red} C    &     \cellcolor{red} C   &      \cellcolor{yellow} A  &       \cellcolor{red} C     &      \cellcolor{yellow} A     &   \cellcolor{green} D   &    \cellcolor{green} D  &     \cellcolor{yellow} A &  \cellcolor{yellow} A   &  \cellcolor{green} D    &     \cellcolor{red} C &    \cellcolor{yellow} A  &   \cellcolor{yellow} A        \\ \cline{3-24}
 
 & & \multicolumn{1}{c|}{Read Skew2 (W1R2-R2W1)}  & 22    &   \cellcolor{red} C &      \cellcolor{red} C        &       \cellcolor{red} C      &      \cellcolor{red} C   &   \cellcolor{red} C      &         \cellcolor{red} C     &          \cellcolor{red} C   &     \cellcolor{red} C    &     \cellcolor{red} C   &      \cellcolor{red} C  &       \cellcolor{red} C     &      \cellcolor{red} C     &   \cellcolor{green} D   &    \cellcolor{green} D  &     \cellcolor{green} D &  \cellcolor{yellow} A   &  \cellcolor{green} D    &     \cellcolor{red} C &    \cellcolor{red} C  &   \cellcolor{yellow} A                        \\ \cline{3-24}

 &  & \multicolumn{1}{c|}{Read Skew3} & 23    &   \cellcolor{red} C &      \cellcolor{red} C        &       \cellcolor{red} C      &      \cellcolor{red} C   &   \cellcolor{green} D      &         \cellcolor{red} C     &          \cellcolor{red} C   &     \cellcolor{red} C    &     \cellcolor{red} C   &      \cellcolor{red} C  &       \cellcolor{red} C     &      \cellcolor{red} C     &   \cellcolor{green} D   &    \cellcolor{green} D  &     \cellcolor{green} D &  \cellcolor{yellow} A   &  \cellcolor{green} D    &     \cellcolor{red} C &    \cellcolor{red} C  &   \cellcolor{yellow} A                       \\ \cline{3-24}

 &  & \multicolumn{1}{c|}{Read Skew (Fractured Reads)} & 24    &   \cellcolor{red} C &      \cellcolor{red} C        &       \cellcolor{red} C      &      \cellcolor{yellow} A   &   \cellcolor{red} C      &         \cellcolor{red} C     &          \cellcolor{yellow} A   &     \cellcolor{red} C    &     \cellcolor{red} C   &      \cellcolor{yellow} A  &       \cellcolor{red} C     &      \cellcolor{yellow} A     &   \cellcolor{green} D   &    \cellcolor{green} D  &     \cellcolor{yellow} A &  \cellcolor{yellow} A   &  \cellcolor{green} D    &     \cellcolor{red} C &    \cellcolor{yellow} A  &   \cellcolor{yellow} A                        \\ \cline{3-24}
 
 &  & \multicolumn{1}{c|}{Read Skew (Causality Violation Anomaly)} & 25   &     \cellcolor{red} C &      \cellcolor{red} C        &       \cellcolor{red} C      &      \cellcolor{yellow} A   &   \cellcolor{red} C      &         \cellcolor{red} C     &          \cellcolor{yellow} A   &     \cellcolor{red} C    &     \cellcolor{red} C   &      \cellcolor{yellow} A  &       \cellcolor{red} C     &      \cellcolor{yellow} A     &   \cellcolor{green} D   &    \cellcolor{green} D  &     \cellcolor{yellow} A &  \cellcolor{yellow} A   &  \cellcolor{green} D    &     \cellcolor{red} C &    \cellcolor{yellow} A  &   \cellcolor{yellow} A                      \\ \cline{3-24}

 &    & \multicolumn{1}{c|}{Read Skew (Serial Concurrent Phenomenon)} & 26  & \cellcolor{red} C &      \cellcolor{red} C        &       \cellcolor{red} C      &      \cellcolor{yellow} A   &   \cellcolor{red} C      &         \cellcolor{red} C     &          \cellcolor{yellow} A   &     \cellcolor{red} C    &     \cellcolor{red} C   &      \cellcolor{yellow} A  &       \cellcolor{red} C     &      \cellcolor{yellow} A     &   \cellcolor{green} D   &    \cellcolor{green} D  &     \cellcolor{yellow} A &  \cellcolor{yellow} A   &  \cellcolor{green} D    &     \cellcolor{red} C &    \cellcolor{yellow} A  &   \cellcolor{yellow} A                         \\ \cline{3-24}

 &    & \multicolumn{1}{c|}{Read Skew (Cross Phenomenon)} & 27  &  \cellcolor{red} C &      \cellcolor{red} C        &       \cellcolor{red} C      &      \cellcolor{yellow} A   &   \cellcolor{red} C      &         \cellcolor{red} C     &          \cellcolor{yellow} A   &     \cellcolor{red} C    &     \cellcolor{red} C   &      \cellcolor{yellow} A  &       \cellcolor{red} C     &      \cellcolor{yellow} A     &   \cellcolor{green} D   &    \cellcolor{green} D  &     \cellcolor{yellow} A &  \cellcolor{yellow} A   &  \cellcolor{green} D    &     \cellcolor{red} C &    \cellcolor{yellow} A  &   \cellcolor{yellow} A                        \\ \cline{3-24}

 &      & \multicolumn{1}{c|}{Read Skew (Cross Phantom)} & 28 & \cellcolor{green} D &      \cellcolor{red} C        &       \cellcolor{red} C      &      \cellcolor{yellow} A   &   \cellcolor{red} C      &         \cellcolor{red} C     &          \cellcolor{yellow} A   &     \cellcolor{red} C    &     \cellcolor{red} C   &      \cellcolor{yellow} A  &       \cellcolor{red} C     &      \cellcolor{yellow} A     &   \cellcolor{green} D   &    \cellcolor{yellow} A  &     \cellcolor{yellow} A &  \cellcolor{yellow} A   &  \cellcolor{green} D    &     \cellcolor{red} C &    \cellcolor{yellow} A  &   \cellcolor{yellow} A                        \\ \cline{3-24}

 &     & \multicolumn{1}{c|}{Read Skew (Long Fork Anomaly)} & 29 & \cellcolor{red} C &      \cellcolor{red} C        &       \cellcolor{red} C      &      \cellcolor{red} C   &   \cellcolor{green} D      &         \cellcolor{red} C     &          \cellcolor{red} C   &     \cellcolor{red} C    &     \cellcolor{red} C   &      \cellcolor{red} C  &       \cellcolor{red} C     &      \cellcolor{red} C     &   \cellcolor{green} D   &    \cellcolor{green} D  &     \cellcolor{green} D &  \cellcolor{yellow} A   &  \cellcolor{green} D    &     \cellcolor{red} C &    \cellcolor{red} C  &   \cellcolor{yellow} A                        \\ \cline{3-24}

 &     & \multicolumn{1}{c|}{Read Skew (Half-Predicate-Based Read Skew)} & 30 &  \cellcolor{red} C &      \cellcolor{yellow} A        &       \cellcolor{yellow} A      &      \cellcolor{yellow} A   &   \cellcolor{red} C      &         \cellcolor{red} C     &          \cellcolor{yellow} A   &     \cellcolor{red} C    &     \cellcolor{red} C   &      \cellcolor{yellow} A  &       \cellcolor{red} C     &      \cellcolor{yellow} A     &   \cellcolor{green} D   &    \cellcolor{yellow} A  &     \cellcolor{yellow} A &  \cellcolor{yellow} A   &  \cellcolor{green} D    &     \cellcolor{red} C &    \cellcolor{yellow} A  &   \cellcolor{yellow} A                        \\ \cline{3-24}

 &      & \multicolumn{1}{c|}{Read Skew (Total-Same-Predicate-Based Read Skew)} & 31 & \cellcolor{green} D &      \cellcolor{red} C        &       \cellcolor{red} C      &      \cellcolor{yellow} A   &   \cellcolor{red} C      &         \cellcolor{red} C     &          \cellcolor{yellow} A   &     \cellcolor{red} C    &     \cellcolor{red} C   &      \cellcolor{yellow} A  &       \cellcolor{red} C     &      \cellcolor{yellow} A     &   \cellcolor{green} D   &    \cellcolor{yellow} A  &     \cellcolor{yellow} A &  \cellcolor{yellow} A   &  \cellcolor{green} D    &     \cellcolor{red} C &    \cellcolor{yellow} A  &   \cellcolor{yellow} A                         \\ \cline{3-24}

 &     & \multicolumn{1}{c|}{Read Skew (Total-Diff-Predicate-Based Read Skew)} & 32  &  \cellcolor{green} D &      \cellcolor{yellow} A        &       \cellcolor{yellow} A      &      \cellcolor{yellow} A   &   \cellcolor{red} C      &         \cellcolor{red} C     &          \cellcolor{yellow} A   &     \cellcolor{red} C    &     \cellcolor{red} C   &      \cellcolor{yellow} A  &       \cellcolor{red} C     &      \cellcolor{yellow} A     &   \cellcolor{green} D   &    \cellcolor{yellow} A  &     \cellcolor{yellow} A &  \cellcolor{yellow} A   &  \cellcolor{green} D    &     \cellcolor{red} C &    \cellcolor{yellow} A  &   \cellcolor{yellow} A                        \\ \cline{3-24}

 &     & \centering Read Skew~~~~~(Total-Same-Predicate-Based Read Skew2) & 33 &   \cellcolor{red} C &      \cellcolor{red} C        &       \cellcolor{red} C      &      \cellcolor{yellow} A   &   \cellcolor{red} C      &         \cellcolor{red} C     &          \cellcolor{yellow} A   &     \cellcolor{red} C    &     \cellcolor{red} C   &      \cellcolor{yellow} A  &       \cellcolor{red} C     &      \cellcolor{yellow} A     &   \cellcolor{green} D   &    \cellcolor{green} D  &     \cellcolor{yellow} A &  \cellcolor{yellow} A   &  \cellcolor{green} D    &     \cellcolor{red} C &    \cellcolor{yellow} A  &   \cellcolor{yellow} A                        \\ \cline{2-24}

 &  \multirow{4}{*}{\rotatebox[origin=c]{270}{Step RAT}}    & \multicolumn{1}{c|}{Step RAT (WR $\ge$3)}  & 34 & \cellcolor{red} C &      \cellcolor{red} C        &       \cellcolor{red} C      &      \cellcolor{yellow} A   &   \cellcolor{red} C      &         \cellcolor{red} C     &          \cellcolor{yellow} A   &     \cellcolor{red} C    &     \cellcolor{red} C   &      \cellcolor{yellow} A  &       \cellcolor{red} C     &      \cellcolor{yellow} A     &   \cellcolor{green} D   &    \cellcolor{green} D  &     \cellcolor{yellow} A &  \cellcolor{yellow} A   &  \cellcolor{green} D    &     \cellcolor{red} C &    \cellcolor{yellow} A  &   \cellcolor{yellow} A    \\ \cline{3-24}

 &     & \multicolumn{1}{c|}{Step RAT (UnnamedAnomaly)} & 35 & \cellcolor{red} C &      \cellcolor{red} C        &       \cellcolor{red} C      &      \cellcolor{yellow} A   &   \cellcolor{red} C      &         \cellcolor{red} C     &          \cellcolor{yellow} A   &     \cellcolor{red} C    &     \cellcolor{red} C   &      \cellcolor{yellow} A  &       \cellcolor{red} C     &      \cellcolor{yellow} A     &   \cellcolor{green} D   &    \cellcolor{green} D  &     \cellcolor{yellow} A &  \cellcolor{yellow} A   &  \cellcolor{green} D    &     \cellcolor{red} C &    \cellcolor{yellow} A  &   \cellcolor{yellow} A                         \\ \cline{3-24}

 &      & \multicolumn{1}{c|}{Step RAT (RAT-Special)} & 36 & \cellcolor{yellow} A &      \cellcolor{yellow} A        &       \cellcolor{yellow} A      &      \cellcolor{yellow} A   &   \cellcolor{green} D      &         \cellcolor{yellow} A     &          \cellcolor{yellow} A   &     \cellcolor{green} D    &     \cellcolor{yellow} A   &      \cellcolor{yellow} A  &       \cellcolor{green} D     &      \cellcolor{yellow} A     &   \cellcolor{green} D   &    \cellcolor{green} D  &     \cellcolor{yellow} A &  \cellcolor{yellow} A   &  \cellcolor{green} D    &     \cellcolor{yellow} A &    \cellcolor{yellow} A  &   \cellcolor{yellow} A                        \\ \cline{3-24}

 &  & \multicolumn{1}{c|}{Step RAT (RAT-Special2)} & 37    & \cellcolor{yellow} A &      \cellcolor{yellow} A        &       \cellcolor{yellow} A      &      \cellcolor{yellow} A   &   \cellcolor{green} D      &         \cellcolor{yellow} A     &          \cellcolor{yellow} A   &     \cellcolor{green} D    &     \cellcolor{yellow} A   &      \cellcolor{yellow} A  &       \cellcolor{green} D     &      \cellcolor{yellow} A     &   \cellcolor{green} D   &    \cellcolor{green} D  &     \cellcolor{yellow} A &  \cellcolor{yellow} A   &  \cellcolor{green} D    &     \cellcolor{yellow} A &    \cellcolor{yellow} A  &   \cellcolor{yellow} A                         \\ \hline

 \multirow{15}{*}{\rotatebox[origin=c]{270}{IAT(Interactive Anomaly Type)}}    & \multicolumn{2}{c|}{Lost Update Committed (R1W2-W2C2W)} & 38 &  \cellcolor{green} D &      \cellcolor{green} D        &       \cellcolor{green} D      &      \cellcolor{yellow} A   &   \cellcolor{green} D      &         \cellcolor{yellow} A     &          \cellcolor{yellow} A   &     \cellcolor{green} D    &     \cellcolor{green} D   &      \cellcolor{yellow} A  &       \cellcolor{green} D     &      \cellcolor{yellow} A     &   \cellcolor{green} D   &    \cellcolor{green} D  &     \cellcolor{yellow} A &  \cellcolor{yellow} A   &  \cellcolor{green} D    &     \cellcolor{yellow} A &    \cellcolor{yellow} A  &   \cellcolor{yellow} A      \\ \cline{2-24}

 & \multicolumn{2}{c|}{Fuzzy/Non-Repeatable Read Committed (R1W2-W2C2R1)} &  39    &    \cellcolor{red} C &      \cellcolor{red} C        &       \cellcolor{red} C      &      \cellcolor{yellow} A   &   \cellcolor{red} C      &         \cellcolor{red} C     &          \cellcolor{yellow} A   &     \cellcolor{red} C    &     \cellcolor{red} C   &      \cellcolor{yellow} A  &       \cellcolor{red} C     &      \cellcolor{yellow} A     &   \cellcolor{green} D   &    \cellcolor{green} D  &     \cellcolor{yellow} A &  \cellcolor{yellow} A   &  \cellcolor{green} D    &     \cellcolor{red} C &    \cellcolor{yellow} A  &   \cellcolor{yellow} A     \\ \cline{2-24}

 &   \multicolumn{2}{c|}{Read Skew Committed (R1W2-W2R1)}  & 40 & \cellcolor{red} C &      \cellcolor{red} C        &       \cellcolor{red} C      &      \cellcolor{yellow} A   &   \cellcolor{red} C      &         \cellcolor{red} C     &          \cellcolor{yellow} A   &     \cellcolor{red} C    &     \cellcolor{red} C   &      \cellcolor{yellow} A  &       \cellcolor{red} C     &      \cellcolor{yellow} A     &   \cellcolor{green} D   &    \cellcolor{green} D  &     \cellcolor{yellow} A &  \cellcolor{yellow} A   &  \cellcolor{green} D    &     \cellcolor{red} C &    \cellcolor{yellow} A  &   \cellcolor{yellow} A      \\ \cline{2-24}

 &  \multicolumn{2}{c|}{Read-Write Skew 1 Committed (R1W2-W2C2W1)} &  41    &  \cellcolor{green} D &      \cellcolor{green} D        &       \cellcolor{green} D      &      \cellcolor{yellow} A   &   \cellcolor{green} D      &         \cellcolor{yellow} A     &          \cellcolor{yellow} A   &     \cellcolor{green} D    &     \cellcolor{green} D   &      \cellcolor{yellow} A  &       \cellcolor{green} D     &      \cellcolor{yellow} A     &   \cellcolor{green} D   &    \cellcolor{green} D  &     \cellcolor{yellow} A &  \cellcolor{yellow} A   &  \cellcolor{green} D    &     \cellcolor{yellow} A &    \cellcolor{yellow} A  &   \cellcolor{yellow} A      \\ \cline{2-24}

 & \multirow{8}{*}{\rotatebox[origin=c]{270}{Write skew}} &  \multicolumn{1}{c|}{Write Skew (R1W2-R2W1)}  & 42    &  \cellcolor{yellow} A &      \cellcolor{yellow} A        &       \cellcolor{yellow} A      &      \cellcolor{yellow} A   &   \cellcolor{green} D      &         \cellcolor{yellow} A     &          \cellcolor{yellow} A   &     \cellcolor{green} D    &     \cellcolor{yellow} A   &      \cellcolor{yellow} A  &       \cellcolor{green} D     &      \cellcolor{yellow} A     &   \cellcolor{green} D   &    \cellcolor{green} D  &     \cellcolor{yellow} A &  \cellcolor{yellow} A   &  \cellcolor{green} D    &     \cellcolor{yellow} A &    \cellcolor{yellow} A  &   \cellcolor{yellow} A     \\ \cline{3-24}

 & &  \multicolumn{1}{c|}{Write Skew (Black and White)} &  43    & \cellcolor{yellow} A &      \cellcolor{yellow} A        &       \cellcolor{yellow} A      &      \cellcolor{yellow} A   &   \cellcolor{green} D      &         \cellcolor{yellow} A     &          \cellcolor{yellow} A   &     \cellcolor{green} D    &     \cellcolor{yellow} A   &      \cellcolor{yellow} A  &       \cellcolor{yellow} A     &      \cellcolor{yellow} A     &   \cellcolor{green} D   &    \cellcolor{green} D  &     \cellcolor{green} D &  \cellcolor{green} D   &  \cellcolor{green} D    &     \cellcolor{green} D &    \cellcolor{yellow} A  &   \cellcolor{yellow} A                        \\ \cline{3-24}

 &    & \multicolumn{1}{c|}{Write Skew (Intersecting Data)} & 44  &   \cellcolor{yellow} A &      \cellcolor{yellow} A        &       \cellcolor{yellow} A      &      \cellcolor{yellow} A   &   \cellcolor{green} D      &         \cellcolor{yellow} A     &          \cellcolor{yellow} A   &     \cellcolor{green} D    &     \cellcolor{yellow} A   &      \cellcolor{yellow} A  &       \cellcolor{green} D     &      \cellcolor{yellow} A     &   \cellcolor{green} D   &    \cellcolor{green} D  &     \cellcolor{green} D &  \cellcolor{red} C   &  \cellcolor{green} D    &     \cellcolor{yellow} A &    \cellcolor{yellow} A  &   \cellcolor{yellow} A                        \\ \cline{3-24}

 &   & \multicolumn{1}{c|}{Write Skew (Overdraft Protection)} & 45    &  \cellcolor{yellow} A &      \cellcolor{yellow} A        &       \cellcolor{yellow} A      &      \cellcolor{yellow} A   &   \cellcolor{green} D      &         \cellcolor{yellow} A     &          \cellcolor{yellow} A   &     \cellcolor{green} D    &     \cellcolor{yellow} A   &      \cellcolor{yellow} A  &       \cellcolor{green} D     &      \cellcolor{yellow} A     &   \cellcolor{green} D   &    \cellcolor{green} D  &     \cellcolor{yellow} A &  \cellcolor{yellow} A   &  \cellcolor{green} D    &     \cellcolor{yellow} A &    \cellcolor{yellow} A  &   \cellcolor{yellow} A                        \\ \cline{3-24}

 &     & \multicolumn{1}{c|}{Half-Predicate-Based Write Skew} & 46  & \cellcolor{yellow} A &      \cellcolor{yellow} A        &       \cellcolor{yellow} A      &      \cellcolor{yellow} A   &   \cellcolor{green} D      &         \cellcolor{yellow} A     &          \cellcolor{yellow} A   &     \cellcolor{green} D    &     \cellcolor{yellow} A   &      \cellcolor{yellow} A  &       \cellcolor{green} D     &      \cellcolor{yellow} A     &   \cellcolor{green} D   &    \cellcolor{green} D  &     \cellcolor{yellow} A &  \cellcolor{yellow} A   &  \cellcolor{green} D    &     \cellcolor{yellow} A &    \cellcolor{yellow} A  &   \cellcolor{yellow} A                        \\ \cline{3-24}

 &  & \multicolumn{1}{c|}{Total-Same-Predicate-Based Write Skew} & 47   &   \cellcolor{yellow} A &      \cellcolor{yellow} A        &       \cellcolor{yellow} A      &      \cellcolor{yellow} A   &   \cellcolor{green} D      &         \cellcolor{yellow} A     &          \cellcolor{yellow} A   &     \cellcolor{green} D    &     \cellcolor{yellow} A   &      \cellcolor{yellow} A  &       \cellcolor{yellow} A     &      \cellcolor{yellow} A     &   \cellcolor{green} D   &    \cellcolor{yellow} A  &     \cellcolor{yellow} A &  \cellcolor{yellow} A   &  \cellcolor{green} D    &     \cellcolor{yellow} A &    \cellcolor{yellow} A  &   \cellcolor{yellow} A                        \\ \cline{3-24} 

 &  & \multicolumn{1}{c|}{Total-Diff-Predicate-Based Write Skew} & 48    &   \cellcolor{yellow} A &      \cellcolor{yellow} A        &       \cellcolor{yellow} A      &      \cellcolor{yellow} A   &   \cellcolor{green} D      &         \cellcolor{yellow} A     &          \cellcolor{yellow} A   &     \cellcolor{green} D    &     \cellcolor{yellow} A   &      \cellcolor{yellow} A  &       \cellcolor{yellow} A     &      \cellcolor{yellow} A     &   \cellcolor{green} D   &    \cellcolor{yellow} A  &     \cellcolor{yellow} A &  \cellcolor{yellow} A   &  \cellcolor{green} D    &     \cellcolor{yellow} A &    \cellcolor{yellow} A  &   \cellcolor{yellow} A                        \\ \cline{3-24}

 &  & \multicolumn{1}{c|}{Write Skew(Read-only Transaction Anomaly)} & 49   &   \cellcolor{yellow} A &      \cellcolor{yellow} A        &       \cellcolor{yellow} A      &      \cellcolor{yellow} A   &   \cellcolor{green} D      &         \cellcolor{yellow} A     &          \cellcolor{yellow} A   &     \cellcolor{green} D    &     \cellcolor{yellow} A   &      \cellcolor{yellow} A  &       \cellcolor{green} D     &      \cellcolor{yellow} A     &   \cellcolor{green} D   &    \cellcolor{green} D  &     \cellcolor{yellow} A &  \cellcolor{yellow} A   &  \cellcolor{green} D    &     \cellcolor{yellow} A &    \cellcolor{yellow} A  &   \cellcolor{yellow} A                       \\ \cline{2-24}

 &   \multirow{3}{*}{\rotatebox[origin=c]{270}{Step IAT}}   & \multicolumn{1}{c|}{Step IAT(Primary Colors) (other$\ge$3)} & 50 &  \cellcolor{yellow} A &      \cellcolor{yellow} A        &       \cellcolor{yellow} A      &      \cellcolor{yellow} A   &   \cellcolor{green} D      &         \cellcolor{yellow} A     &          \cellcolor{yellow} A   &     \cellcolor{green} D    &     \cellcolor{yellow} A   &      \cellcolor{yellow} A  &       \cellcolor{yellow} A     &      \cellcolor{yellow} A     &   \cellcolor{green} D   &    \cellcolor{green} D  &     \cellcolor{green} D &  \cellcolor{green} D   &  \cellcolor{green} D    &     \cellcolor{green} D &    \cellcolor{yellow} A  &   \cellcolor{yellow} A      \\ \cline{3-24}

 &  & \multicolumn{1}{c|}{Step IAT(Sawtooth)} & 51   &   \cellcolor{yellow} A &      \cellcolor{yellow} A        &       \cellcolor{yellow} A      &      \cellcolor{yellow} A   &   \cellcolor{green} D      &         \cellcolor{yellow} A     &          \cellcolor{yellow} A   &     \cellcolor{green} D    &     \cellcolor{yellow} A   &      \cellcolor{yellow} A  &       \cellcolor{green} D     &      \cellcolor{yellow} A     &   \cellcolor{green} D   &    \cellcolor{green} D  &     \cellcolor{yellow} A &  \cellcolor{yellow} A   &  \cellcolor{green} D    &     \cellcolor{yellow} A &    \cellcolor{yellow} A  &   \cellcolor{yellow} A                        \\ \cline{3-24}

 &  & \multicolumn{1}{c|}{Step IAT(Predicate-Based Sawtooth)} & 52   &   \cellcolor{yellow} A &      \cellcolor{yellow} A        &       \cellcolor{yellow} A      &      \cellcolor{yellow} A   &   \cellcolor{green} D      &         \cellcolor{yellow} A     &          \cellcolor{yellow} A   &     \cellcolor{green} D    &     \cellcolor{yellow} A   &      \cellcolor{yellow} A  &       \cellcolor{yellow} A     &      \cellcolor{yellow} A     &   \cellcolor{green} D   &    \cellcolor{yellow} A  &     \cellcolor{yellow} A &  \cellcolor{yellow} A   &  \cellcolor{green} D    &     \cellcolor{yellow} A &    \cellcolor{yellow} A  &   \cellcolor{yellow} A                        \\ \hline
\bottomrule
\end{tabular}


==> tables/workload_description.tex <==
\begin{tabular}{c|c|c|c|c}
\toprule
\hline
 Benchmark&
 No &
  Workload &
  u/r/w/i &
  Skew 
  \\ \hline


\multirow{4}{*}{\textbf{YCSB}} & y1 & Main write & 0.9/0.1/0.9/0 & 0.5  \\ \cline{2-4} 

 & y2& Main read & 0.1/0.9/0.1/0 & 0.5  \\ \cline{2-4} 

 & y3& Low contention & 0.5/0.5/0.5/0 & 0.0  \\ \cline{2-4} 

 & y4& High contention & 0.5/0.5/0.5/0 & 0.9  \\ \hline 

\multirow{4}{*}{\textbf{TPCC}}  & t1& Payment & 1/0.2/0.6/0.2 & - \\ \cline{2-4}  

 & t2& Neworder & 1/0.2/0.6/0.2 & -  \\ \cline{2-4} 

 & t3& Mix & 1/0.2/0.6/0.2 & - \\ \hline 

\bottomrule


\end{tabular}
